Applications of Deep Learning to the Design of Enhanced Wireless Communication Systems

Innovation in the physical layer of communication systems has traditionally been achieved by breaking down the transceivers into sets of processing blocks, each optimized independently based on mathematical models. Conversely, deep learning (DL)-based systems are able to handle increasingly complex tasks for which no tractable models are available. This thesis aims at comparing different approaches to unlock the full potential of DL in the physical layer. First, we describe a neural network (NN)-based block strategy, where an NN is optimized to replace a block in a communication system. We apply this strategy to introduce a multi-user multiple-input multiple-output (MU-MIMO) detector that builds on top of an existing DL-based architecture. Second, we detail an end-to-end strategy, in which the transmitter and receiver are modeled as an autoencoder. This approach is illustrated with the design of waveforms that achieve high throughputs while satisfying peak-to-average power ratio (PAPR) and adjacent channel leakage ratio (ACLR) constraints. Lastly, we propose a hybrid strategy, where multiple DL components are inserted into a traditional architecture but are trained to optimize the end-to-end performance. To demonstrate its benefits, we propose a DL-enhanced MU-MIMO receiver that both enable lower bit error rates (BERs) compared to a conventional receiver and remains scalable to any number of users. Each approach has its own strengths and shortcomings. While the first one is the easiest to implement, its individual block optimization does not ensure the overall system optimality. On the other hand, systems designed with the second approach are computationally complex but allow for new opportunities such as pilotless transmissions. Finally, the combined flexibility and end-to-end performance gains of the third approach motivate its use for short-term practical implementations.

==> Background/figs/gradient_descent.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\pgfplotsset{
    width=.66\textwidth,
    height=0.6\textwidth
}

\begin{axis}[
  legend cell align={left},
  legend style={
    fill opacity=0.8,
    draw opacity=1,
    text opacity=1,
    at={(0.97,0.03)},
    anchor=south east,
    draw=white!80!black
  },
tick align=outside,
tick pos=left,
xtick={-4, ..., 4},
x grid style={white!69.0196078431373!black},
xlabel={$x$},
xmajorgrids,
xmin=-4.5, xmax=4.5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ytick={-4, -2, 0, 2, 4, 6, 8, 10},
minor y tick num = 1,
yminorgrids,
ymajorgrids,
ymin=-4.5, ymax=10.1,
ytick style={color=black}
]
\addplot [semithick, color0]
table {%
-5.5 15.125
-5.27551020408163 13.9155039566847
-5.05102040816327 12.7564035818409
-4.8265306122449 11.6476988754686
-4.60204081632653 10.5893898375677
-4.37755102040816 9.58147646813828
-4.1530612244898 8.62395876718034
-3.92857142857143 7.71683673469388
-3.70408163265306 6.86011037067888
-3.47959183673469 6.05377967513536
-3.25510204081633 5.29784464806331
-3.03061224489796 4.59230528946272
-2.80612244897959 3.93716159933361
-2.58163265306122 3.33241357767597
-2.35714285714286 2.7780612244898
-2.13265306122449 2.27410453977509
-1.90816326530612 1.82054352353186
-1.68367346938776 1.4173781757601
-1.45918367346939 1.06460849645981
-1.23469387755102 0.762234485630987
-1.01020408163265 0.510256143273636
-0.785714285714286 0.308673469387755
-0.561224489795919 0.157486463973345
-0.336734693877551 0.0566951270304039
-0.112244897959184 0.0062994585589338
0.112244897959184 0.0062994585589338
0.336734693877551 0.0566951270304039
0.561224489795919 0.157486463973345
0.785714285714286 0.308673469387755
1.01020408163265 0.510256143273636
1.23469387755102 0.762234485630987
1.45918367346939 1.06460849645981
1.68367346938776 1.4173781757601
1.90816326530612 1.82054352353186
2.13265306122449 2.27410453977509
2.35714285714286 2.77806122448979
2.58163265306122 3.33241357767597
2.80612244897959 3.93716159933361
3.03061224489796 4.59230528946272
3.25510204081633 5.29784464806331
3.47959183673469 6.05377967513536
3.70408163265306 6.86011037067888
3.92857142857143 7.71683673469388
4.1530612244898 8.62395876718034
4.37755102040816 9.58147646813827
4.60204081632653 10.5893898375677
4.8265306122449 11.6476988754686
5.05102040816327 12.7564035818409
5.27551020408163 13.9155039566847
5.5 15.125
};
\addlegendentry{$L(x) = \frac{1}{2}x^2$}
\addplot [semithick, color1, dashed]
table {%
-5.5 -5.5
-5.27551020408163 -5.27551020408163
-5.05102040816327 -5.05102040816327
-4.8265306122449 -4.8265306122449
-4.60204081632653 -4.60204081632653
-4.37755102040816 -4.37755102040816
-4.1530612244898 -4.1530612244898
-3.92857142857143 -3.92857142857143
-3.70408163265306 -3.70408163265306
-3.47959183673469 -3.47959183673469
-3.25510204081633 -3.25510204081633
-3.03061224489796 -3.03061224489796
-2.80612244897959 -2.80612244897959
-2.58163265306122 -2.58163265306122
-2.35714285714286 -2.35714285714286
-2.13265306122449 -2.13265306122449
-1.90816326530612 -1.90816326530612
-1.68367346938776 -1.68367346938776
-1.45918367346939 -1.45918367346939
-1.23469387755102 -1.23469387755102
-1.01020408163265 -1.01020408163265
-0.785714285714286 -0.785714285714286
-0.561224489795919 -0.561224489795919
-0.336734693877551 -0.336734693877551
-0.112244897959184 -0.112244897959184
0.112244897959184 0.112244897959184
0.336734693877551 0.336734693877551
0.561224489795919 0.561224489795919
0.785714285714286 0.785714285714286
1.01020408163265 1.01020408163265
1.23469387755102 1.23469387755102
1.45918367346939 1.45918367346939
1.68367346938776 1.68367346938776
1.90816326530612 1.90816326530612
2.13265306122449 2.13265306122449
2.35714285714286 2.35714285714286
2.58163265306122 2.58163265306122
2.80612244897959 2.80612244897959
3.03061224489796 3.03061224489796
3.25510204081633 3.25510204081633
3.47959183673469 3.47959183673469
3.70408163265306 3.70408163265306
3.92857142857143 3.92857142857143
4.1530612244898 4.1530612244898
4.37755102040816 4.37755102040816
4.60204081632653 4.60204081632653
4.8265306122449 4.8265306122449
5.05102040816327 5.05102040816327
5.27551020408163 5.27551020408163
5.5 5.5
};
\addlegendentry{$L'(x) = x$}
\addplot [semithick, black, forget plot]
table {%
-5.5 0
-5.27551020408163 0
-5.05102040816327 0
-4.8265306122449 0
-4.60204081632653 0
-4.37755102040816 0
-4.1530612244898 0
-3.92857142857143 0
-3.70408163265306 0
-3.47959183673469 0
-3.25510204081633 0
-3.03061224489796 0
-2.80612244897959 0
-2.58163265306122 0
-2.35714285714286 0
-2.13265306122449 0
-1.90816326530612 0
-1.68367346938776 0
-1.45918367346939 0
-1.23469387755102 0
-1.01020408163265 0
-0.785714285714286 0
-0.561224489795919 0
-0.336734693877551 0
-0.112244897959184 0
0.112244897959184 0
0.336734693877551 0
0.561224489795919 0
0.785714285714286 0
1.01020408163265 0
1.23469387755102 0
1.45918367346939 0
1.68367346938776 0
1.90816326530612 0
2.13265306122449 0
2.35714285714286 0
2.58163265306122 0
2.80612244897959 0
3.03061224489796 0
3.25510204081633 0
3.47959183673469 0
3.70408163265306 0
3.92857142857143 0
4.1530612244898 0
4.37755102040816 0
4.60204081632653 0
4.8265306122449 0
5.05102040816327 0
5.27551020408163 0
5.5 0
};
\addplot [semithick, black, forget plot]
table {%
0 -16.5
0 -15.8265306122449
0 -15.1530612244898
0 -14.4795918367347
0 -13.8061224489796
0 -13.1326530612245
0 -12.4591836734694
0 -11.7857142857143
0 -11.1122448979592
0 -10.4387755102041
0 -9.76530612244898
0 -9.09183673469388
0 -8.41836734693878
0 -7.74489795918367
0 -7.07142857142857
0 -6.39795918367347
0 -5.72448979591837
0 -5.05102040816327
0 -4.37755102040816
0 -3.70408163265306
0 -3.03061224489796
0 -2.35714285714286
0 -1.68367346938776
0 -1.01020408163265
0 -0.336734693877552
0 0.336734693877552
0 1.01020408163265
0 1.68367346938776
0 2.35714285714286
0 3.03061224489796
0 3.70408163265306
0 4.37755102040816
0 5.05102040816327
0 5.72448979591837
0 6.39795918367347
0 7.07142857142857
0 7.74489795918367
0 8.41836734693877
0 9.09183673469388
0 9.76530612244898
0 10.4387755102041
0 11.1122448979592
0 11.7857142857143
0 12.4591836734694
0 13.1326530612245
0 13.8061224489796
0 14.4795918367347
0 15.1530612244898
0 15.8265306122449
0 16.5
};
\end{axis}

\end{tikzpicture}


==> Background/figs_fr/act_func.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\pgfplotsset{
    width=.44\textwidth,
    height=0.4\textwidth
}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={x},
xmajorgrids,
xmin=-6, xmax=6,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={y},
ymajorgrids,
ymin=-1.25, ymax=6,
ytick style={color=black}
]
\addplot [semithick, color0]
table {%
-6 0
-5.88 0
-5.76 0
-5.64 0
-5.52 0
-5.4 0
-5.28 0
-5.16 0
-5.04 0
-4.92 0
-4.8 0
-4.68 0
-4.56 0
-4.44 0
-4.32 0
-4.2 0
-4.08 0
-3.96 0
-3.84 0
-3.72 0
-3.6 0
-3.48 0
-3.36 0
-3.24 0
-3.12 0
-3 0
-2.88 0
-2.76 0
-2.64 0
-2.52 0
-2.4 0
-2.28 0
-2.16 0
-2.04 0
-1.92 0
-1.8 0
-1.68 0
-1.56 0
-1.44 0
-1.32 0
-1.2 0
-1.08 0
-0.96 0
-0.84 0
-0.720000000000001 0
-0.600000000000001 0
-0.48 0
-0.36 0
-0.24 0
-0.12 0
0 0
0.12 0.12
0.24 0.24
0.359999999999999 0.359999999999999
0.48 0.48
0.6 0.6
0.72 0.72
0.84 0.84
0.96 0.96
1.08 1.08
1.2 1.2
1.32 1.32
1.44 1.44
1.56 1.56
1.68 1.68
1.8 1.8
1.92 1.92
2.04 2.04
2.16 2.16
2.28 2.28
2.4 2.4
2.52 2.52
2.64 2.64
2.76 2.76
2.88 2.88
3 3
3.12 3.12
3.24 3.24
3.36 3.36
3.48 3.48
3.6 3.6
3.72 3.72
3.84 3.84
3.96 3.96
4.08 4.08
4.2 4.2
4.32 4.32
4.44 4.44
4.56 4.56
4.68 4.68
4.8 4.8
4.92 4.92
5.04 5.04
5.16 5.16
5.28 5.28
5.4 5.4
5.52 5.52
5.64 5.64
5.76 5.76
5.88 5.88
6 6
};
\addlegendentry{ReLU}
\addplot [semithick, color1, dashed]
table {%
-6 -0.997521247823334
-5.88 -0.997205214724963
-5.76 -0.996848888401556
-5.64 -0.996447131593779
-5.52 -0.99599415205791
-5.4 -0.995483419057387
-5.28 -0.994907569207301
-5.16 -0.994258300314346
-5.04 -0.993526251681711
-4.92 -0.992700869153211
-4.8 -0.99177025295098
-4.68 -0.990720986112935
-4.56 -0.989537941056573
-4.44 -0.988204061480248
-4.32 -0.986700116457556
-4.2 -0.985004423179522
-4.08 -0.983092534347295
-3.96 -0.980936885708388
-3.84 -0.97850639865491
-3.72 -0.975766032154309
-3.6 -0.972676277552707
-3.48 -0.969192588967249
-3.36 -0.965264741055261
-3.24 -0.960836104901013
-3.12 -0.955842831580307
-3 -0.950212931632136
-2.88 -0.943865237165866
-2.76 -0.936708231640359
-2.64 -0.928638730443614
-2.52 -0.919540393250468
-2.4 -0.909282046710588
-2.28 -0.897715793284463
-2.16 -0.884674878961938
-2.04 -0.869971289121574
-1.92 -0.85339303786965
-1.8 -0.834701111778413
-1.68 -0.81362602396059
-1.56 -0.789863928799235
-1.44 -0.763072241317878
-1.32 -0.73286469803415
-1.2 -0.698805788087798
-1.08 -0.660404474355061
-0.96 -0.617107114024888
-0.84 -0.56828947657092
-0.720000000000001 -0.513247744040029
-0.600000000000001 -0.451188363905974
-0.48 -0.381216608193859
-0.36 -0.302323673928969
-0.24 -0.213372138933447
-0.12 -0.113079563282843
0 0
0.12 0.12
0.24 0.24
0.359999999999999 0.359999999999999
0.48 0.48
0.6 0.6
0.72 0.72
0.84 0.84
0.96 0.96
1.08 1.08
1.2 1.2
1.32 1.32
1.44 1.44
1.56 1.56
1.68 1.68
1.8 1.8
1.92 1.92
2.04 2.04
2.16 2.16
2.28 2.28
2.4 2.4
2.52 2.52
2.64 2.64
2.76 2.76
2.88 2.88
3 3
3.12 3.12
3.24 3.24
3.36 3.36
3.48 3.48
3.6 3.6
3.72 3.72
3.84 3.84
3.96 3.96
4.08 4.08
4.2 4.2
4.32 4.32
4.44 4.44
4.56 4.56
4.68 4.68
4.8 4.8
4.92 4.92
5.04 5.04
5.16 5.16
5.28 5.28
5.4 5.4
5.52 5.52
5.64 5.64
5.76 5.76
5.88 5.88
6 6
};
\addlegendentry{ELU}
\end{axis}

\end{tikzpicture}


==> Background/figs_fr/gradient_descent.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\pgfplotsset{
    width=.66\textwidth,
    height=0.6\textwidth
}

\begin{axis}[
  legend cell align={left},
  legend style={
    fill opacity=0.8,
    draw opacity=1,
    text opacity=1,
    at={(0.97,0.03)},
    anchor=south east,
    draw=white!80!black
  },
tick align=outside,
tick pos=left,
xtick={-4, ..., 4},
x grid style={white!69.0196078431373!black},
xlabel={$x$},
xmajorgrids,
xmin=-4.5, xmax=4.5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ytick={-4, -2, 0, 2, 4, 6, 8, 10},
minor y tick num = 1,
yminorgrids,
ymajorgrids,
ymin=-4.5, ymax=10.1,
ytick style={color=black}
]
\addplot [semithick, color0]
table {%
-5.5 15.125
-5.27551020408163 13.9155039566847
-5.05102040816327 12.7564035818409
-4.8265306122449 11.6476988754686
-4.60204081632653 10.5893898375677
-4.37755102040816 9.58147646813828
-4.1530612244898 8.62395876718034
-3.92857142857143 7.71683673469388
-3.70408163265306 6.86011037067888
-3.47959183673469 6.05377967513536
-3.25510204081633 5.29784464806331
-3.03061224489796 4.59230528946272
-2.80612244897959 3.93716159933361
-2.58163265306122 3.33241357767597
-2.35714285714286 2.7780612244898
-2.13265306122449 2.27410453977509
-1.90816326530612 1.82054352353186
-1.68367346938776 1.4173781757601
-1.45918367346939 1.06460849645981
-1.23469387755102 0.762234485630987
-1.01020408163265 0.510256143273636
-0.785714285714286 0.308673469387755
-0.561224489795919 0.157486463973345
-0.336734693877551 0.0566951270304039
-0.112244897959184 0.0062994585589338
0.112244897959184 0.0062994585589338
0.336734693877551 0.0566951270304039
0.561224489795919 0.157486463973345
0.785714285714286 0.308673469387755
1.01020408163265 0.510256143273636
1.23469387755102 0.762234485630987
1.45918367346939 1.06460849645981
1.68367346938776 1.4173781757601
1.90816326530612 1.82054352353186
2.13265306122449 2.27410453977509
2.35714285714286 2.77806122448979
2.58163265306122 3.33241357767597
2.80612244897959 3.93716159933361
3.03061224489796 4.59230528946272
3.25510204081633 5.29784464806331
3.47959183673469 6.05377967513536
3.70408163265306 6.86011037067888
3.92857142857143 7.71683673469388
4.1530612244898 8.62395876718034
4.37755102040816 9.58147646813827
4.60204081632653 10.5893898375677
4.8265306122449 11.6476988754686
5.05102040816327 12.7564035818409
5.27551020408163 13.9155039566847
5.5 15.125
};
\addlegendentry{$L(x) = \frac{1}{2}x^2$}
\addplot [semithick, color1, dashed]
table {%
-5.5 -5.5
-5.27551020408163 -5.27551020408163
-5.05102040816327 -5.05102040816327
-4.8265306122449 -4.8265306122449
-4.60204081632653 -4.60204081632653
-4.37755102040816 -4.37755102040816
-4.1530612244898 -4.1530612244898
-3.92857142857143 -3.92857142857143
-3.70408163265306 -3.70408163265306
-3.47959183673469 -3.47959183673469
-3.25510204081633 -3.25510204081633
-3.03061224489796 -3.03061224489796
-2.80612244897959 -2.80612244897959
-2.58163265306122 -2.58163265306122
-2.35714285714286 -2.35714285714286
-2.13265306122449 -2.13265306122449
-1.90816326530612 -1.90816326530612
-1.68367346938776 -1.68367346938776
-1.45918367346939 -1.45918367346939
-1.23469387755102 -1.23469387755102
-1.01020408163265 -1.01020408163265
-0.785714285714286 -0.785714285714286
-0.561224489795919 -0.561224489795919
-0.336734693877551 -0.336734693877551
-0.112244897959184 -0.112244897959184
0.112244897959184 0.112244897959184
0.336734693877551 0.336734693877551
0.561224489795919 0.561224489795919
0.785714285714286 0.785714285714286
1.01020408163265 1.01020408163265
1.23469387755102 1.23469387755102
1.45918367346939 1.45918367346939
1.68367346938776 1.68367346938776
1.90816326530612 1.90816326530612
2.13265306122449 2.13265306122449
2.35714285714286 2.35714285714286
2.58163265306122 2.58163265306122
2.80612244897959 2.80612244897959
3.03061224489796 3.03061224489796
3.25510204081633 3.25510204081633
3.47959183673469 3.47959183673469
3.70408163265306 3.70408163265306
3.92857142857143 3.92857142857143
4.1530612244898 4.1530612244898
4.37755102040816 4.37755102040816
4.60204081632653 4.60204081632653
4.8265306122449 4.8265306122449
5.05102040816327 5.05102040816327
5.27551020408163 5.27551020408163
5.5 5.5
};
\addlegendentry{$L'(x) = x$}
\addplot [semithick, black, forget plot]
table {%
-5.5 0
-5.27551020408163 0
-5.05102040816327 0
-4.8265306122449 0
-4.60204081632653 0
-4.37755102040816 0
-4.1530612244898 0
-3.92857142857143 0
-3.70408163265306 0
-3.47959183673469 0
-3.25510204081633 0
-3.03061224489796 0
-2.80612244897959 0
-2.58163265306122 0
-2.35714285714286 0
-2.13265306122449 0
-1.90816326530612 0
-1.68367346938776 0
-1.45918367346939 0
-1.23469387755102 0
-1.01020408163265 0
-0.785714285714286 0
-0.561224489795919 0
-0.336734693877551 0
-0.112244897959184 0
0.112244897959184 0
0.336734693877551 0
0.561224489795919 0
0.785714285714286 0
1.01020408163265 0
1.23469387755102 0
1.45918367346939 0
1.68367346938776 0
1.90816326530612 0
2.13265306122449 0
2.35714285714286 0
2.58163265306122 0
2.80612244897959 0
3.03061224489796 0
3.25510204081633 0
3.47959183673469 0
3.70408163265306 0
3.92857142857143 0
4.1530612244898 0
4.37755102040816 0
4.60204081632653 0
4.8265306122449 0
5.05102040816327 0
5.27551020408163 0
5.5 0
};
\addplot [semithick, black, forget plot]
table {%
0 -16.5
0 -15.8265306122449
0 -15.1530612244898
0 -14.4795918367347
0 -13.8061224489796
0 -13.1326530612245
0 -12.4591836734694
0 -11.7857142857143
0 -11.1122448979592
0 -10.4387755102041
0 -9.76530612244898
0 -9.09183673469388
0 -8.41836734693878
0 -7.74489795918367
0 -7.07142857142857
0 -6.39795918367347
0 -5.72448979591837
0 -5.05102040816327
0 -4.37755102040816
0 -3.70408163265306
0 -3.03061224489796
0 -2.35714285714286
0 -1.68367346938776
0 -1.01020408163265
0 -0.336734693877552
0 0.336734693877552
0 1.01020408163265
0 1.68367346938776
0 2.35714285714286
0 3.03061224489796
0 3.70408163265306
0 4.37755102040816
0 5.05102040816327
0 5.72448979591837
0 6.39795918367347
0 7.07142857142857
0 7.74489795918367
0 8.41836734693877
0 9.09183673469388
0 9.76530612244898
0 10.4387755102041
0 11.1122448979592
0 11.7857142857143
0 12.4591836734694
0 13.1326530612245
0 13.8061224489796
0 14.4795918367347
0 15.1530612244898
0 15.8265306122449
0 16.5
};
\end{axis}

\end{tikzpicture}


==> Backmatter/list_of_symbols_old.tex <==
\chapter*{List of Symbols}


\begin{center}
    \begin{tabular}{ | m{5em} | m{10cm}|  m{5em} | }
      \hline
      $\Am^{(t)}$ & matrix used in the iterative detection algorithms \\ 
      \hline
      ! $\bv^{(t)}$ & bias vector used in the iterative detection algorithms & $\cv^{(t)}$  \\ 
      \hline
      ! $b$ & b th bit (bit index)& $o$ \\
      \hline
      ! $\mathscr{b}$ & actual bit value & $b$\\
      \hline
      ! $B$ & number of bits/channel uses & $O$ \\
      \hline
      $\Bm$, $\bv$, $b$ & matrix of bits \\
      \hline
      $B_S$ & batch size \\
      \hline
      $\Cm$ & Normalization precoding downlink matrix chapter 2 \\
      \hline
      ! $\cv, c$ & FBS carrying the peak-reduction signal & $r_{m,n\in \mathcal{R}}$\\ 
      \hline
      $ ! \Cm$ & Channel covariance matrix & $\Sigmam$ \\ 
      \hline
      $\mathcal{C}$ & Constellation \\ 
      \hline
      $C$ & Achievable rate \\ 
      \hline
      ! $c$ & Constellation points & - \\ 
      \hline
      $d_{m,n\in \mathcal{D}}$ & data signal \\
      \hline
      ! $\Dm$ & Diagonal matrix from eigenvalue decomposition h=UDU & $\mathbf{\Lambda}$\\ 
      \hline
      ! $\Dm$ & Post-equaliztion diagonal matrix & $\Pm$\\ 
      \hline
      $\mathcal{D}$ & set of RE carrying data\\ 
      \hline
      $\mathcal{D}, D$ & Set of $D$ subcarriers carrying data \\ 
      \hline
      $\Em$ & Channel estimation error spatial covariance \\ 
      \hline
      $E_{...}$ & Energies \\ 
      \hline
      $\Fm$ & Inverse Fourier Transform \\ 
      \hline
      $\Gm$ & Equivalent downlink channel \\ 
      \hline
      $\Hm$ & Channel coefficients \\
      \hline
      $\Jm$ & precomputed energy matrix \\
      \hline
      $\Km$ & precomputed energy matrix \\
      \hline
      ! $K$ & Bit per channel uses & $O$ \\
      \hline
      $k$ & user index \\
      \hline
      $\Lm$ & Eigenvalue decomposition h=UDU \\
      \hline
      $l$ & BS antenna index \\
      \hline
      $\mathcal{M}, M, m$ & Subset and umber of OFDM symbols\\
      \hline
      $\nv$ & Noise \\
      \hline
      $n$ & subcarrier index \\
      \hline
      $\mathcal{N}, N, n$ & Subset and number of subcarrier chapter 3 \\
      \hline
      ! $N_r$ & Number of receiving antennas & $ N_l$\\
      \hline
      ! $N_m$ & Number of receiving antennas & $N_l$ \\
      \hline
      ! $N_u$ & Number of single-antennas users & $N_k$, $k$ \\
      \hline
      $N_k$, $k$ & Number of single-antennas users \\
      \hline
      $! N_t$ & Number of OFDM symbols& $N_m, M$ \\
      \hline
      $ ! N_f$ & Number of OFDM subcarriers& $N_n, N$ \\
      \hline
      $N_{P_f}$, $N_{P_t}$ & Number of pilots\\
      \hline
      $! \Nm$ & Normalization precoding downlink matrix chapter 2 & $\Cm$\\
      \hline
      $\Nm$ & Noise Tensor Chapter 3\\
      \hline
      $\mathcal{N}$ & Set of subcarriers\\
      \hline

    \end{tabular}
\end{center}

\begin{center}
    \begin{tabular}{ | m{5em} | m{10cm}| m{5em} | }
       


      \hline
      $o$ & Equivalent downlink noise chapter 2 & $ \xi$\\
      \hline
      ! $\widehat{P}$, $\widetilde{P}$ & Predicted probability &  $\widehat{P}$\\
      \hline
      $\mathcal{P}^{(k)}$ & Pilot pattern \\
      \hline
      $\Pm$ & Post-equalization diagonal matrix \\ 
      \hline
      $\qv$ & downlink noise vector\\ 
      \hline
      $q$ & Number of bits per channel uses\\
      \hline
      $\Qm$, $\Qm_{\Am}$, $\Qm_{\Bm}$ & QR-decomposition \\ 
      \hline
      $r_{m,n\in \mathcal{R}}$ & peak-reduction signal \\
      \hline
      $\Rm$, $\Rm_{\Am}$ & QR-decomposition \\ 
      \hline
      $! \Rm$ & Chapter 2 downlink received signal & $ \Om$\\ 
      \hline
      $\mathcal{R}, R$ &Set of subcarriers used for TR scheme\\ 
      \hline
      $\Sm$ & Tensor of unprecoded downlink symbols\\ 
      \hline
      ! $S$ & batch size & $B_S$\\
      \hline 
      $S_m(f)$ & Baseband spectrum\\
      \hline 
      $s_m(t)$ & time-domain signal\\
      \hline 
      $\Tm$ & Tensor of precoded downlink symbols \\ 
      \hline
      $T$ & Duration of an OFDM symbol \\ 
      \hline
      ! $\uv, u$ & FBS carrying the data signal chap. 3 & $d_{m,n\in \mathcal{D}}$  \\ 
      \hline
      $\Um$ & Eigenvalue decomposition h=UDU & $\Lm$\\ 
      \hline
      $\Um$ & Chapter 2 downlink received signal \\
      \hline
      $\Vm^{(k)}$  & estimatd error variances for user $k$ \\ 
      \hline
      $! \Vm$  & precomputed energy matrix & $\Jm$\\ 
      \hline
      $\Wm$  & MMSE matrix  \\ 
      \hline
      $! \Wm$  & Precoputed energy matrix & $\Km$  \\ 
      \hline
      $\widetilde{\xv}$ & symbol after MMSE  & $\widehat{\xv}$\\ 
      \hline
      $\widehat{\xv}$  & symbols from $\CC$ selected after $\widetilde{\xv}$ & $\doublehat{\xv}$ \\ 
      \hline
      $\xv^*$  & $\xv$ after QR decomposition & $\bar{\xv}$  \\ 
      \hline
      ! $\mathcal{X}$  & constellation of $\xv$ & $\mathcal{C}$ \\ 
      \hline
      $\yv^*$  & $\yv$ after QR decomposition & $\bar{\yv}$ \\ 
      \hline
      ! $\zv^{(t)}$  & intermediary vector used in the iterative detection algorithms & $\boldsymbol{\kappa}^{(t)}$ \\ 
      \hline
      ! $\zv$  & additive noise term in chapter 2 & $\zeta$ \\ 
      \hline
      $\zv$  & oversampled time-domain signal chapter 3 \\ 
      \hline
      $\thetav$, $\psiv$ & Trainable parameters\\ 
      \hline
      $\tau^{(t)}$ & estimated variance used in the iterative detection algorithms \\ 
      \hline
      ! $\alpha(t)$ & power ratio chapter 3 & $\nu(t)$\\ 
      \hline
      $\alpha, \beta, \gamma$ & exponential decay model\\ 
      \hline
      $\tau$ & variance of the equivalent downlink noise chapter 2\\ 
      \hline
      $\sigma$ & noise variance \\ 
      \hline
      $\rho$ & post-equalization uplink noise variance chapter 2\\ 
      \hline
      $\eta$ &  code rate \\
      \hline
      ! $\eta$ &  denoising function& $\chi$ \\
      \hline
      $\epsilon$ &  PAPR threshold \\
      \hline
      $\mathbf{\Theta}$ & Matrix to be optimized in the iterative detection algorithm \\ 
      \hline
      $\Sigmam$ & Channel covariance matrix \\ 
      \hline
      $\Omegam$ & Covariance matrix for the main channel chapter 2\\ 
      \hline
      $\Psim$ & Covariance matrix for the interfering channels chap. 2 \\ 
      \hline
            
    \end{tabular}
    \end{center}



==> Chapter1/abstract.tex <==
\begin{abstract}

Optimal symbol detection for \gls{MIMO} systems is known to be an NP-hard problem. 
Conventional heuristic algorithms are either too complex to be practical or suffer from poor performance.
Recently, several approaches tried to address those challenges by implementing the detector as a deep neural network. 
However, they either still achieve unsatisfying performance on practical spatially correlated channels, or are computationally demanding since they require retraining for each channel realization. 
In this work, we address both issues by training an additional \gls{NN}, referred to as the hypernetwork, which takes as input the channel matrix and generates the weights of the neural \gls{NN}-based detector.
Results show that the proposed approach achieves near state-of-the-art performance without the need for re-training.

\begin{IEEEkeywords}
MIMO Detection, Deep Learning, Hypernetworks, spatial channel correlation
\end{IEEEkeywords}

\end{abstract}



==> Chapter2/abstract.tex <==
\begin{abstract}

%Future communications systems are expected to meet even stricter requirements to satisfy the needs arising from emerging services.
An attractive research direction for future communication systems is the design of new waveforms that can both support high throughputs and present advantageous signal characteristics.
Although most modern systems use \gls{OFDM} for its efficient equalization, this waveform suffers from multiple limitations such as a high \gls{ACLR} and high \gls{PAPR}.
In this paper, we propose a learning-based method to design \gls{OFDM}-based waveforms that satisfy selected constraints while maximizing an achievable information rate. 
To that aim, we model the transmitter and the receiver as \glspl{CNN} that respectively implement a high-dimensional modulation scheme and perform the detection of the transmitted bits.
This leads to an optimization problem that is solved using the augmented Lagrangian method.
%The proposed approach is applied to the design of \gls{OFDM} waveforms that both enable pilotless transmissions and meet specific \gls{ACLR} and \gls{PAPR} targets values.
Evaluation results show that the end-to-end system is able to satisfy target \gls{PAPR} and \gls{ACLR} constraints and allows significant throughput gains compared to a \gls{TR} baseline.
An additional advantage is that no dedicated pilots are needed.

\begin{IEEEkeywords}
Deep learning, end-to-end learning, neural networks, OFDM, waveform, \gls{ACLR}, \gls{PAPR} 
\end{IEEEkeywords}

\end{abstract}



==> Chapter2/figs/CCDF_2.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={$|s(t)|^2$ [\si{dB}]},
xmajorgrids,
xmin=0, xmax=9,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={CCDF},
ymajorgrids,
ymin=2e-05, ymax=0.680933265155766,
ymode=log,
ytick style={color=black}
]
\addplot [semithick, black, mark=square, mark size=3, mark options={solid,fill opacity=0}]
table {%
-0.08820085 0.4336185714285714
0.25675178 0.4044919047619048
0.6017044 0.3749447619047619
0.94665706 0.3453609523809524
1.2916096 0.3158228571428571
1.6365623 0.28686047619047617
1.9815149 0.25822428571428574
2.3264675 0.2302204761904762
2.67142 0.20330619047619047
3.016373 0.17744904761904762
3.3613255 0.1528657142857143
3.706278 0.1298561904761905
4.051231 0.10853238095238095
4.3961835 0.08890952380952381
4.741136 0.07093333333333333
5.0860887 0.054555238095238094
5.4310412 0.039754285714285714
5.775994 0.02687095238095238
6.1209464 0.01630190476190476
6.465899 0.008869047619047618
6.8108516 0.004346666666666667
7.1558046 0.001819047619047619
7.500757 0.0006385714285714286
7.84571 0.00021428571428571427
8.190662 5.6666666666666664e-05
8.535615 1.5714285714285715e-05
};
\addlegendentry{Baseline with 2 \glspl{PRT}}

\addplot [semithick, color0, mark=o, mark size=3, mark options={solid,fill opacity=0}]
table {%
-0.0046317433 0.39614533333333335
0.3829095 0.3622365714285714
0.7704508 0.3281958095238095
1.157992 0.2941921904761905
1.5455333 0.26081866666666664
1.9330745 0.22781142857142858
2.3206158 0.19607276190476192
2.708157 0.16539066666666666
3.0956984 0.13631580952380953
3.4832397 0.10925009523809524
3.8707807 0.08410971428571429
4.2583222 0.061540761904761904
4.6458635 0.041320190476190476
5.0334044 0.024225714285714284
5.4209456 0.010878095238095239
5.808487 0.002855809523809524
6.196028 0.00031714285714285715
6.5835695 1.1238095238095239e-05
};
\addlegendentry{E2E system, $\gamma_{\text{peak}}=6$~\si{dB}}

\end{axis}

\end{tikzpicture}


==> Chapter2/figs_fr/CCDF_2.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},log basis y={10},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={$|s(t)|^2$ [\si{dB}]},
xmajorgrids,
xmin=0, xmax=9,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={CCDF},
ymajorgrids,
ymin=2e-05, ymax=0.680933265155766,
ymode=log,
ytick style={color=black}
]
\addplot [semithick, black, mark=square, mark size=3, mark options={solid,fill opacity=0}]
table {%
-0.08820085 0.4336185714285714
0.25675178 0.4044919047619048
0.6017044 0.3749447619047619
0.94665706 0.3453609523809524
1.2916096 0.3158228571428571
1.6365623 0.28686047619047617
1.9815149 0.25822428571428574
2.3264675 0.2302204761904762
2.67142 0.20330619047619047
3.016373 0.17744904761904762
3.3613255 0.1528657142857143
3.706278 0.1298561904761905
4.051231 0.10853238095238095
4.3961835 0.08890952380952381
4.741136 0.07093333333333333
5.0860887 0.054555238095238094
5.4310412 0.039754285714285714
5.775994 0.02687095238095238
6.1209464 0.01630190476190476
6.465899 0.008869047619047618
6.8108516 0.004346666666666667
7.1558046 0.001819047619047619
7.500757 0.0006385714285714286
7.84571 0.00021428571428571427
8.190662 5.6666666666666664e-05
8.535615 1.5714285714285715e-05
};
\addlegendentry{Baseline with 2 \glspl{PRT}}

\addplot [semithick, color0, mark=o, mark size=3, mark options={solid,fill opacity=0}]
table {%
-0.0046317433 0.39614533333333335
0.3829095 0.3622365714285714
0.7704508 0.3281958095238095
1.157992 0.2941921904761905
1.5455333 0.26081866666666664
1.9330745 0.22781142857142858
2.3206158 0.19607276190476192
2.708157 0.16539066666666666
3.0956984 0.13631580952380953
3.4832397 0.10925009523809524
3.8707807 0.08410971428571429
4.2583222 0.061540761904761904
4.6458635 0.041320190476190476
5.0334044 0.024225714285714284
5.4209456 0.010878095238095239
5.808487 0.002855809523809524
6.196028 0.00031714285714285715
6.5835695 1.1238095238095239e-05
};
\addlegendentry{E2E system, $\gamma_{\text{peak}}=6$~\si{dB}}

\end{axis}

\end{tikzpicture}


==> Chapter2/figs_fr/results_in_band.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\pgfplotsset{
    width=.4\textwidth,
    height=0.35\textwidth
}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={$\frac{T+T^{\text{CP}}}{T}$},
xmajorgrids,
xmin=0.995, xmax=1.105,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={$E_{I_m}$},
scaled y ticks=false,
yticklabel=\pgfkeys{/pgf/number format/.cd,fixed,precision=3,zerofill}\pgfmathprintnumber{\tick},
ymajorgrids,
ymin=24.8068725948848, ymax=24.8139566514653,
ytick style={color=black}
]
\addplot [semithick, color0, mark=+, mark size=3, mark options={solid}]
table {%
1 24.8071945974566
1.01 24.8074462917281
1.02 24.8079299281401
1.03 24.8086259535118
1.04 24.8093693671574
1.05 24.8100782735769
1.06 24.8107878318214
1.07 24.8115202041498
1.08 24.8122389328379
1.09 24.8129317426784
1.1 24.8136346488935
};
\end{axis}

\end{tikzpicture}


==> Chapter3/abstract.tex <==
\begin{abstract}

\Gls{ML} starts to be widely used to enhance the performance of \gls{MU-MIMO} receivers. 
However, it is still unclear if such methods are truly competitive with respect to conventional methods in realistic scenarios and under practical constraints. 
In addition to enabling accurate signal reconstruction on realistic channel models, \gls{MU-MIMO} receive algorithms must allow for easy adaptation to a varying number of users without the need for retraining. 
In contrast to existing work, we propose an \gls{ML}-enhanced \gls{MU-MIMO} receiver that builds on top of a conventional \gls{LMMSE} architecture. 
It preserves the interpretability and scalability of the \gls{LMMSE} receiver, while improving its accuracy in two ways. 
First, \glspl{CNN} are used to compute an approximation of the second-order statistics of the channel estimation error which are required for accurate equalization. 
Second, a \gls{CNN}-based demapper jointly processes a large number of \gls{OFDM} symbols and subcarriers, which allows it to compute better \glspl{LLR} by compensating for channel aging.
The resulting architecture can be used in the up-~and downlink and is trained in an end-to-end manner, removing the need for hard-to-get perfect \gls{CSI} during the training phase. 
Simulation results demonstrate consistent performance improvements over the baseline which are especially pronounced in high mobility scenarios. 


\begin{IEEEkeywords}
Multi-user MIMO detection, OFDM, channel estimation, deep learning, neural networks
\end{IEEEkeywords}

\end{abstract}



==> Cover/cover.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{frontpage}
\begin{center}
\includegraphics[height=2.5cm]{./Figures/Logos/3_logos}
\end{center}


\vspace{-.2cm}
{\scriptsize N$^{\circ}$ d'ordre NNT : \@ordernumber}
\vspace{0.5cm}

\begin{center}
{\fontlmss{bx} \Large \textbf{TH\MakeUppercase{è}SE de DOCTORAT DE L'\MakeUppercase{\@universite}}} \\
\vspace{.1cm}
{\large opérée au sein de} \\
\vspace{.1cm}
{\fontlmss{bx} \Large \@companyfr} 
{\large \, et \,} 
{\fontlmss{bx} \Large \@institutionfr} \\
\vspace{.5cm}

{\fontlmss{b} \large \textbf{\MakeUppercase{é}cole Doctorale }}{\large N$^{\circ}$ \@DSnumber}\\
{\fontlmss{b} \large \textbf{\@EDnom}}\\

\vspace{.5cm}
{\fontlmss{b} \large \textbf{Spécialité / discipline de doctorat : }} \\
{\fontlmss{b} \large \@specialite}

\vspace{.5cm}
{\large Soutenue publiquement le 28 janvier 2022, par :} \\ 
\vspace{.1cm}
{\fontlmss{bx} \Large\@author}

\vspace{.5cm}
\definecolor{rule}{rgb}{0.5,0.5,0.5}
{\color{rule} \rule{\textwidth}{0.7pt}}\\
\vspace{.25cm}
\fontlmss{bx} \Huge{\@titrefr}\\
\vspace{-0.1cm}
{\color{rule} \rule{\textwidth}{0.7pt}}\\
\end{center}
\vspace{.5cm}

\begin{center}
    
\hskip.3ex{\small Devant le jury composé de :} \\

\small



\begin{tabular}{hllll}
& \textbf{Rapporteurs:} & \\ 
%&\getpresident{namefr}  & \getpresident{labelfr}\\
%&\getpresident{name} & \getpresident{gradefr} & \getpresident{institution} & \getpresident{labelfr}\\
\getreviewersfr 
& \textbf{Examinateurs:} & \\
\getexaminersfr
& \textbf{Directeur de th\`{e}se:} & \\
&\getadvisor{name} &\getadvisor{gradefr}  & \getadvisor{labelfr}\\
%&\getadvisor{name} & \getadvisor{gradefr} & \getadvisor{institution} & \getadvisor{labelfr}\\
&\textbf{Co-encadrants de thèse:}& \\
\getcoadvisorsfr
&Ait Aoudia, Fayçal & Chargé de Recherche & Nvidia, France\\
%& \textbf{Membre invit\'{e}:} & \\
%\getguestsfr
\end{tabular}
\end{center}
\vspace{1.0cm}
\end{frontpage}

==> Frontmatter/Bio/bio.tex <==
% !TEX encoding = UTF-8 Unicode

\chapter*{Publications}

\section*{Journals}

\begin{enumerate}[label={[\arabic*]}]
\item ``\emph{When Does Output Feedback Enlarge the Capacity of the Interference Channel?}''. Victor Quintero, Samir M. Perlaza, I\~naki Esnaola, and Jean-Marie Gorce. IEEE Transactions on Communications, vol. 66 no. 2, pp. 615-628, Feb., 2018.
\item ``\emph{Approximate Capacity Region of the Two-User Gaussian Interference Channel with Noisy Channel-Output Feedback}''. Victor Quintero, Samir M. Perlaza, I\~naki Esnaola, and Jean-Marie Gorce. This work will appear in the IEEE Transactions on Information Theory. Submitted on Nov. 10, 2016; revised on Sep. 23, 2017; and accepted on Mar. 4, 2018. %This work is under second round review in the IEEE Transactions on Information Theory.  Submitted on Nov. 10, 2016 and revised on Sep. 23, 2017.
%https://hal.archives-ouvertes.fr/hal-01397118/document
%https://hal.archives-ouvertes.fr/hal-01432525/document
%\item ``\emph{Approximate Nash Region of the Two-User Gaussian Interference Channel with Noisy Channel-Output Feedback}''. Victor Quintero, Samir M. Perlaza, Jean-Marie Gorce, and H. Vincent Poor. \\
%This work will be submitted to IEEE Transactions on Information Theory.
\end{enumerate}

\section*{Conferences}

\begin{enumerate}[label={[\arabic*]}]
\item ``\emph{Noisy Channel-Output Feedback Capacity of the Linear Deterministic Interference Channel}''. Victor Quintero, Samir M. Perlaza, and  Jean-Marie Gorce. IEEE Information Theory Workshop (ITW), Jeju, Korea, Oct., 2015. 
%https://hal.archives-ouvertes.fr/hal-01207339/document
\item ``\emph{Approximate Capacity of the Gaussian Interference Channel with Noisy Channel-Output Feedback}''. Victor Quintero, Samir M. Perlaza, I\~naki Esnaola, and Jean-Marie Gorce. IEEE Information Theory Workshop (ITW), Cambridge, UK, Sep., 2016. 
%https://hal.archives-ouvertes.fr/hal-01293921/document
\item ``\emph{Nash Region of the Linear Deterministic Interference Channel with Noisy Output Feedback}''. Victor Quintero, Samir M. Perlaza, Jean-Marie Gorce, and H. Vincent Poor. IEEE Intl. Symposium on Information Theory (ISIT), Aachen, Germany, Jun., 2017. 
%https://hal.archives-ouvertes.fr/hal-01520799/document
\end{enumerate}

\section*{INRIA Technical Reports}

\begin{enumerate}[label={[\arabic*]}]
\item ``\emph{Noisy Channel-Output Feedback Capacity of the Linear Deterministic Interference Channel}''. Victor Quintero, Samir M. Perlaza, and  Jean-Marie Gorce.
Technical Report, INRIA, No. 456, Lyon, France, Jan., 2015. 
%https://hal.archives-ouvertes.fr/hal-01117154/document
\item ``\emph{Approximate Capacity of the Two-User Gaussian Interference Channel with Noisy Channel-Output Feedback}''. Victor Quintero, Samir M. Perlaza, I\~naki Esnaola, and Jean-Marie Gorce. Technical Report, INRIA, No. 8861, Lyon, France, Mar., 2016. 
%https://hal.archives-ouvertes.fr/hal-01315887/document
\item ``\emph{When Does Channel-Output Feedback Enlarge the Capacity Region of the Interference Channel?}''. Victor Quintero, Samir M. Perlaza, I\~naki Esnaola, and Jean-Marie Gorce. Technical Report, INRIA, No. 8862, Lyon, France, Mar., 2016. 
%https://hal.archives-ouvertes.fr/hal-01281717/document
\item ``\emph{Decentralized Interference Channels with Noisy Output Feedback}''. Victor Quintero, Samir M. Perlaza, Jean-Marie Gorce, and H. Vincent Poor.
Technical Report, INRIA, No. RR-9011, Lyon, France, Jan., 2017. 
%https://hal.archives-ouvertes.fr/hal-01462248/document
\end{enumerate}

\section*{Other Publications}

\begin{enumerate}[label={[\arabic*]}]
\item ``\emph{On the Benefits of Channel-Output Feedback in 5G}''. Victor Quintero, Samir M. Perlaza, and  Jean-Marie Gorce. GDR-ISIS meeting: 5G \& Beyond: Promises and Challenges, Paris, Oct., 2014. (Invited talk).
\item ``\emph{Noisy Channel-Output Feedback Capacity of the Linear Deterministic Interference Channel}''. Victor Quintero, Samir M. Perlaza, and  Jean-Marie Gorce.
European School of Information Theory (ESIT), Zandvoort, The Netherlands, Apr., 2015. (Poster).
%http://perso.citi.insa-lyon.fr/vquinter/Posters/ESIT-Poster.pdf
\item ``\emph{Capacit\'e du Canal Lin\'eaire D\'eterministe \`a Interf\'erences avec Voies de Retour Bruit\'ees}''. Victor Quintero, Samir M. Perlaza, and  Jean-Marie Gorce.
Colloque GRETSI, Lyon, France, Sep., 2015.
%https://hal.archives-ouvertes.fr/hal-01219393/document
\item ``\emph{Does the Channel-Output Feedback improve the performance of the Two-User Linear Deterministic Interference Channel?}''.
Victor Quintero, Samir M. Perlaza,  I\~naki Esnaola, and  Jean-Marie Gorce. INRIA-GDR-ISIS meeting: Recent Advances in Network Information Theory and Coding Theory, Villeurbanne, France, Nov., 2015. (Poster). 
%http://perso.citi.insa-lyon.fr/vquinter/Posters/GDR-Poster.pdf
\item ``\emph{When Does Channel-Output Feedback Increase the Capacity Region of the Two-User Linear Deterministic Interference Channel?}''. Victor Quintero, Samir M. Perlaza,  I\~naki Esnaola, and  Jean-Marie Gorce. 11th International Conference on Cognitive Radio Oriented Wireless Networks (CROWNCOM), Grenoble, France, May, 2016.
%https://hal.archives-ouvertes.fr/hal-01240328/document
\item ``\emph{On the Efficiency of Nash Equilibria in the Interference Channel with Noisy Feedback}''. Victor Quintero, Samir M. Perlaza, and Jean-Marie Gorce.
European Wireless Conference. Workshop COCOA - COmpetitive and COoperative Approaches for 5G networks, Dresden, Germany, May, 2017. (Invited Paper). 
%https://hal.archives-ouvertes.fr/hal-01492979/document
\item ``\emph{R\'egion d'$\eta$-\'Equilibre de Nash du Canal Lin\'eaire D\'eterministe \`a Interf\'erences avec R\'etroalimentation D\'egrad\'ee}''. Victor Quintero, Samir M. Perlaza, and  Jean-Marie Gorce. 
Colloque GRETSI, Juan-les-Pins, France, Sep., 2017.
\end{enumerate}


==> Frontmatter/FrenchPart/frenchpart.tex <==
% !TEX root = /Users/Victor/Google Drive/VQ-IC/Final Manuscript/Manuscript/manuscript.tex

\chapter{Synth\`{e}se des Contributions}\label{ChPresentationinFrench}
%
\chapterletter{C}{ette} th\`{e}se a pour objet d'\'{e}tude le GIC-NOF asym\'{e}trique \`{a} deux utilisateurs. L'analyse est r\'{e}alis\'{e}e en tenant compte de deux sc\'{e}narios :  (1) centralis\'{e}, dans lequel la totalit\'{e} du r\'{e}seau est contr\^{o}l\'{e}e par une entit\'{e} centrale qui configure les deux paires \'{e}metteur-r\'{e}cepteur; et (2) d\'{e}centralis\'{e}, dans lequel chaque paire \'{e}metteur-r\'{e}cepteur configure de fa\c{c}on autonome ses param\`{e}tres de transmission-r\'{e}ception. L'analyse dans ces deux sc\'{e}narios permet d'approximer la r\'{e}gion de capacit\'{e} ainsi que la r\'{e}gion d'$\eta$-\'{e}quilibre de Nash  du GIC-NOF \`{a} deux utilisateurs. Ces r\'{e}sultats permettent \'{e}galement d'identifier les conditions dans lesquelles une voie de retour peut agrandir la r\'{e}gion de capacit\'{e} et la r\'{e}gion d'\'{e}quilibre.

Voici les principales contributions de cette th\`{e}se : 

\begin{itemize}
\item  Une description compl\`{e}te de la r\'{e}gion de capacit\'{e} du LDIC-NOF \`{a} deux utilisateurs \cite{QPEG-TIT-2016, Quintero-ITW-2015}. Cette contribution g\'{e}n\'{e}ralise les r\'{e}sultats pour les cas du LDIC sans voie de retour \cite{Bresler-ETT-2008}, avec voie de retour parfaite (LDIC-POF) \cite{Suh-TIT-2011}, avec voie de retour d\'{e}grad\'{e}e par un bruit additif (LDIC-NOF)  dans des conditions sym\'{e}triques \cite{SyQuoc-TIT-2015}, et les cas incluant une voie de retour des r\'{e}cepteurs vers leurs \'{e}metteurs appair\'{e}s \cite{Sahai-TIT-2013}. 
\item  Une r\'{e}gion atteignable et une r\'{e}gion d'impossibilit\'{e} du LDIC-NOF \`{a} deux utilisateurs \cite{Quintero-ITW-2016, QPEG-TIT-2016}. Ces deux r\'{e}gions encadrent la r\'{e}gion de capacit\'{e} du GIC-NOF \`{a} deux utilisateurs avec un \'{e}cart maximal de $4.4$ bits. La r\'{e}gion atteignable est obtenue \`{a} l'aide d'un argument de codage al\'{e}atoire combinant le fractionnement de message, un codage de superposition de bloc Markov et un d\'{e}codage \`{a} rebours, comme sugg\'{e}r\'{e} pr\'{e}c\'{e}demment en \cite{Suh-TIT-2011, Tuninetti-ISIT-2007, Yang-Tuninetti-TIT-2011}. La r\'{e}gion d'impossibilit\'{e} est obtenue en utilisant des bornes sup\'{e}rieures existantes dans le cas du CGI \`{a} deux utilisateurs avec POF (GIC-POF) \cite{Suh-TIT-2011} ainsi qu'un ensemble de nouvelles bornes sup\'{e}rieures obtenues \`{a} l'aide de mod\`{e}les assist\'{e}s par g\'{e}nies. Cette contribution g\'{e}n\'{e}ralise les r\'{e}sultats obtenus \`{a} partir des cas sans voie de retour (CGI) \cite{Etkin-TIT-2008}, avec POF (GIC-POF) \cite{Suh-TIT-2011}, et avec NOF (GIC-NOF) dans des conditions sym\'{e}triques \cite{SyQuoc-TIT-2015}.  
\item  Une description compl\`{e}te de la r\'{e}gion d'$\eta$-\'{e}quilibre de Nash du LDIC-NOF \`{a} deux utilisateurs \cite{Quintero-ISIT-2017-1}.  Cette contribution g\'{e}n\'{e}ralise les r\'{e}sultats obtenus \`{a} partir des cas du canal lin\'{e}aire d\'{e}terministe \`{a} interf\'{e}rence   (LDIC) sans voie de retour \cite{Berry-ISIT-2008}, avec POF (GIC-POF) \cite{Perlaza-TIT-2015}, et avec NOF (GIC-NOF) dans des conditions sym\'{e}triques \cite{Perlaza-ISIT-2014a}.
\item  Une r\'{e}gion d'$\eta$-\'{e}quilibre de Nash atteignable et une r\'{e}gion de des\'{e}quilibre avec $\eta \geqslant 1$ pour le GIC-NOF \`{a} deux utilisateurs \cite{Quintero-INRIA-RR-2017}. La r\'{e}gion d'$\eta$-\'{e}quilibre de Nash atteignable est obtenue en effectuant une modification du sch\'{e}ma de codage utilis\'{e} dans la partie centralis\'{e}e. Cette modification implique l'introduction d'un caract\`{e}re al\'{e}atoire commun dans le sch\'{e}ma de codage comme sugg\'{e}r\'{e} par \cite{Berry-TIT-2011} et \cite{Perlaza-TIT-2015}, ce qui permet aux deux paires d'\'{e}metteur-r\'{e}cepteur de limiter l'am\'{e}lioration de d\'{e}bit de chacune lorsque l'une d'elles s'\'{e}carte de l'\'{e}quilibre. La r\'{e}gion de des\'{e}quilibre est obtenue avec $\eta \geqslant 1$ en utilisant les connaissances obtenues \`{a} partir de l'analyse du mod\`{e}le lin\'{e}aire d\'{e}terministe. 
\item  Identification des sc\'{e}narios dans lesquels l'utilisation d'une voie de retour agrandit la r\'{e}gion de capacit\'{e} et la r\'{e}gion d'$\eta$-\'{e}quilibre de Nash \cite{QPEG-TC-2016}.
 \end{itemize}

\section{Canaux \`{a} Interf\'{e}rence Centralis\'{e}s}\label{Chapter5afr}

Consid\'{e}rons  le IC-NOF continu \`{a} deux utilisateurs represent\'{e} par la Figure \ref{Fig:C-IC-NOFfr}.
%
L'\'{e}metteur $i$, $i \in \lbrace 1,2 \rbrace$, souhaite communiquer au r\'{e}cepteur $i$ un message $W_i$. Ce message est repr\'{e}sent\'{e} par une variable al\'{e}atoire ind\'{e}pendante et uniform\'{e}ment distribu\'{e}e prenant des valeurs d'indices dans $\mathcal{W}_i=\lbrace 1,2, \ldots, 2^{NR_i}\rbrace$, durant $N\in\mathds{N}$ utilisations du canal, $R_i \in \mathds{R}_{+}$ indiquant le taux de transmission de l'\'{e}metteur-r\'{e}cepteur $i$ en bits par utilisation du canal.
%
\`{A} cet \'{e}gard, l'\'{e}metteur $i$ envoie le mot-code ${\vec{X}_{i}=\left(X_{i,1}, X_{i,2}, \ldots, X_{i,N}\right)^\sfT \in \mathcal{C}_i \subseteq \mathds{R}^N}$, $\mathcal{C}_i$ \'{e}tant le dictionnaire de l'\'{e}metteur. 

Pour une utilisation du canal donn\'{e} $n \in\lbrace 1,2, \ldots, N\rbrace$, les \'{e}metteurs $1$ et $2$ envoient les symboles $X_{1,n}\in\mathds{R}$ et $X_{2,n}\in\mathds{R}$, respectivement, g\'{e}n\`{e}rent les sorties de canal $\overrightarrow{Y}_{1,n} \in \mathds{R}$, $\overrightarrow{Y}_{2,n} \in \mathds{R}$, $\overleftarrow{Y}_{1,n} \in \mathds{R}$, et $\overleftarrow{Y}_{2,n} \in \mathds{R}$ conform\'{e}ment \`{ a} la fonction de densit\'{e} de probabilit\'{e} conditionnelle  $\pdff_{\overrightarrow{Y}_1,\overrightarrow{Y}_2,\overleftarrow{Y}_1,\overleftarrow{Y}_2|X_{1}, X_{2}}\Big(\overrightarrow{y}_1$, $\overrightarrow{y}_2$, $\overleftarrow{y}_1$, $\overleftarrow{y}_2|x_{1}, x_{2}\Big)$, pour tout $\left(\overrightarrow{y}_1,\overrightarrow{y}_2,\overleftarrow{y}_1,\overleftarrow{y}_2, x_{1}, x_{2} \right) \in \mathds{R}^6$.

L'\'{e}metteur $i$ g\'{e}n\`{e}re le symbole $X_{i,n} \in \mathds{R}$ en prenant en compte l'indice de message $W_i$ et tous les r\'{e}sultats pr\'{e}c\'{e}dents de la voie de retour $i$, \`{a} savoir, $\Big(\overleftarrow{Y}_{i,1}$, $\overleftarrow{Y}_{i,2}$, $\ldots$, $\overleftarrow{Y}_{i,n-1}\Big)$. 
%
L'\'{e}metteur $i$ observe $\overleftarrow{Y}_{i,n}$ \`{a} la fin de la $n$-i\`eme utilisation du canal.
%
L'\'{e}metteur $i$ est d\'{e}fini par l'ensemble des fonctions d\'{e}terministes $\left \lbrace f_{i,1}, f_{i,2}, \ldots, f_{i,N} \right \rbrace$, avec $f_{i,1} : \mathcal{W}_i \rightarrow \mathds{R}$ et pour $n \in \lbrace 2, 3, \ldots, N\rbrace$, $f_{i,n} : \mathcal{W}_i \times \mathds{R}^{n-1} \rightarrow \mathds{R}$, de sorte que
%
\begin{subequations}
\label{EqencodCICNOFfr}
\begin{IEEEeqnarray}{lcl}
\label{Eqencodi1CICNOFfr}
X_{i,1}&=&f_{i,1}\left(W_i\right)  \mbox{ et }  \\
\label{EqencoditCICNOFfr}
X_{i,n}&=&f_{i,n}\left(W_i, \overleftarrow{Y}_{i,1}, \overleftarrow{Y}_{i,2}, \ldots,\overleftarrow{Y}_{i,n-1}\right) \textrm{ pour tout } n>1.
\end{IEEEeqnarray}
\end{subequations}

\`{A} la fin de la transmission, le r\'{e}cepteur $i$ utilise toutes les sorties de canal $\Big(\overrightarrow{Y}_{i,1}, \overrightarrow{Y}_{i,2}, \ldots, \overrightarrow{Y}_{i,N}\Big)^\sfT$ pour obtenir une estimation de l'indice de message $W_i$, not\'{e}e $\widehat{W}_i$. 

Ainsi, la cha\^{i}ne de Markov suivante existe : 
% 
\begin{equation}
\label{EqMarkovChainDMfr}
\Big(W_i, \overleftarrow{\vec{Y}}_{i,(1;n-1)}\Big) \rightarrow X_{i,n} \rightarrow \overrightarrow{Y}_{i,n}. 
 \end{equation}

Soit $T\in \mathds{N}$ fix\'{e}. Supposons que, durant une communication, soient transmis $T$ blocs, chaque bloc consistant en $N$ utilisations du canal. Le r\'{e}cepteur $i$ est d\'{e}fini par la fonction d\'{e}terministe ${\psi_i :  \mathds{R}^{N T} \rightarrow \mathcal{W}_i^{T}}$.
%
\`{A} la fin de la communication, le r\'{e}cepteur $i$ utilise le vecteur $\Big(\overrightarrow{Y}_{i,1}$, $\overrightarrow{Y}_{i,2}$, $\ldots$, $\overrightarrow{Y}_{i,NT}\Big)^\sfT$ pour obtenir 
%
\begin{IEEEeqnarray}{rcl}
\label{EqdecoderCICNOFfr}
\left(\widehat{W}_i^{(1)}, \widehat{W}_i^{(2)}, \ldots, \widehat{W}_i^{(T)}\right) &=& \psi_i \left(\overrightarrow{Y}_{i,1}, \overrightarrow{Y}_{i,2}, \ldots, \overrightarrow{Y}_{i,NT}\right), \quad
\end{IEEEeqnarray} 
%
o\`{u} $\widehat{W}_i^{(t)}$ est une estimation de l'indice de message $W_i^{(t)}$ envoy\'{e} au cours du bloc $t \in \lbrace 1, 2, \ldots, T \rbrace$.

La probabilit\'{e} d'erreur de d\'{e}codage dans le IC continu \`{a} deux utilisateurs durant le bloc $t$, not\'{e}e $P_{\mathrm{e}}^{(t)}(N)$, est donn\'{e}e par   
%
\begin{IEEEeqnarray}{rcl}
\label{EqDecErrorProbfr}
P_{\mathrm{e}}^{(t)}(N) &=&   \max   \Bigg(\Pr{ \widehat{W_1}^{(t)}  \neq   W_1^{(t)}  } , \Pr{ \widehat{W_2}^{(t)}   \neq   W_2^{(t)} }\Bigg). 
\end{IEEEeqnarray}

La d\'{e}finition d'une paire de d\'{e}bit atteignable $(R_1,R_2) \in \mathds{R}_+^{2}$ figure ci-dessous. 
%
\begin{definition-fr}[Paires de d\'{e}bit atteignables]\label{DefAchievableRatePairsfr}
Une paire de d\'{e}bit $(R_1,R_2) \in \mathds{R}_+^{2}$ est atteignable s'il existe des ensembles des fonctions d'encodage $\left \lbrace f_1^{(1)}, f_1^{(2)}, \ldots,f_1^{(N)} \right \rbrace$ et $\left \lbrace f_2^{(1)}, f_2^{(2)}, \ldots, f_2^{(N)}\right \rbrace$, et des fonctions de d\'{e}codage $\psi_1$ et $\psi_2$, telles que la probabilit\'{e} d'erreur $P_{e}^{(t)}(N)$ peut \^{e}tre arbitrairement r\'{e}duite lorsque le nombre d'utilisations du canal $N$ tend vers l'infini pour tous les blocs $t \in \lbrace 1, 2,  \ldots, T \rbrace$.
\end{definition-fr}

\begin{figure}[t!]
\centerline{\epsfig{figure=Figures/C-IC-NOF-FR.pdf,width=0.8\textwidth}}
\caption{Canal \`{a} interf\'{e}rence  continu \`{a} deux utilisateurs avec voie de retour d\'{e}grad\'{e}e par un bruit additif.}
\label{Fig:C-IC-NOFfr}
\end{figure}

Dans un syst\`{e}me centralis\'{e}, un contr\^{o}leur central d\'{e}termine les configurations de toutes les paires d'\'{e}metteur-r\'{e}cepteur. Le contr\^{o}leur central a une vision globale du r\'{e}seau et permet de s\'{e}lectionner des configurations optimales \'{e}tant donn\'{e} une m\'{e}trique, par exemple, la somme des d\'{e}bits, l'efficacit\'{e} \'{e}nerg\'{e}tique, etc. Les limites fondamentales dans un syst\`{e}me centralis\'{e} sont caract\'{e}ris\'{e}es par la r\'{e}gion de capacit\'{e}.

\begin{definition-fr}[R\'{e}gion de capacit\'{e} d'un IC \`{a} deux utilisateurs]\label{DefCapacityRegion2ICfr}
La r\'{e}gion de capacit\'{e} d'un IC \`{a} deux utilisateurs est la fermeture de l'ensemble de toutes les paires possibles de d\'{e}bit atteignables $(R_1,R_2) \in \mathds{R}_+^{2}$.
\end{definition-fr}

\subsection{Canal Gaussien \`{a} Interf\'{e}rence} \label{SectCGICNOFfr}

Le canal Gaussien \`{a} interf\'{e}rence (GIC) repr\'{e}sente un cas particulier du IC-NOF d\'{e}crit ci-dessus dans la perspective des r\'{e}seaux centralis\'{e}s. 
%
Consid\'{e}rons  le GIC-NOF \`{a} deux utilisateurs d\'{e}crit par la Figure~\ref{Fig:G-IC-NOFfr}. 
%
Le coefficient de canal de l'\'{e}metteur $j$ au r\'{e}cepteur $i$ est not\'{e}  $h_{ij}$; le coefficient de canal \`{a} partir de l'\'{e}metteur $i$ au r\'{e}cepteur $i$ est not\'{e} $\overrightarrow{h}_{ii}$; et le coefficient de canal de la sortie de canal $i$ l'\'{e}metteur $i$ est not\'{e}  $\overleftarrow{h}_{ii}$. Tous les coefficients de canal sont suppos\'{e}s \^{e}tre des nombres r\'{e}els non n\'{e}gatifs.
%
A la $n$-i\`{e}me utilisation du canal, 
%
\begin{IEEEeqnarray}{lcl}
\label{Eqsignalyiffr}
\overrightarrow{Y}_{i,n}&=& \overrightarrow{h}_{ii}X_{i,n} + h_{ij}X_{j,n}+\overrightarrow{Z}_{i,n},
\end{IEEEeqnarray}
%
et
\begin{IEEEeqnarray}{rcl}
\label{Eqsignalyibfr}
\overleftarrow{Y}_{i,n}  &=& 
\begin{cases}
 \overleftarrow{Z}_{i,n} &  \textrm{pour } n \! \in \lbrace \! 1, \! 2,  \ldots, d \rbrace  \\ 
\overleftarrow{h}_{ii}\overrightarrow{Y}_{i,n-d} \! + \! \overleftarrow{Z}_{i,n} \!  &  \textrm{pour } n \! \in \lbrace  d \! + \! 1, \! d \! + \! 2, \ldots, \! N \rbrace
 \end{cases}, \quad
\end{IEEEeqnarray}
%
o\`{u} $\overrightarrow{Z}_{i,n}$ et $\overleftarrow{Z}_{i,n}$ sont des variables al\'{e}atoires Gaussiennes standard et o\`{u} $d>0$ est le d\'{e}lai de la voie de retour, fini, mesur\'{e} en utilisations du canal.
% 
Sans perte de g\'{e}n\'{e}ralit\'{e}, le d\'{e}lai de la voie de retour est suppos\'{e} fix\'{e} et \'{e}gal \`{a} une utilisation du canal, c'est \`{a} dire, $d=1$. 
%
Le vecteur d'entr\'{e}e $\vec{X}_{i}$, dont les composantes sont r\'{e}elles, est soumis \`{a} une contrainte de puissance moyenne :
%
\begin{equation}
\label{Eqconstpowfr}
\frac{1}{N}\sum_{n=1}^{N}\mathbb{E}\left[X_{i,n}^2\right] \leq 1,
\end{equation}
%
l'esp\'{e}rance \'{e}tant calcul\'{e}e d'apr\`{e}s la distribution conjointe des messages $W_1$, $W_2$, et les termes de bruits, \`{a} savoir $\overrightarrow{Z}_{1}$, $\overrightarrow{Z}_{2}$, $\overleftarrow{Z}_{1}$, et $\overleftarrow{Z}_{2}$. La d\'{e}pendance de $X_{i,n}$ avec $W_1$, $W_2$, et les r\'{e}alisations de bruit observ\'{e}es pr\'{e}c\'{e}demment sont dues \`{a} l'effet de la voie de retour comme l'indiquent \eqref{EqencodCICNOFfr} et \eqref{Eqsignalyibfr}. 
%
\begin{figure}[t!]
 \centerline{\epsfig{figure=Figures/G-IC-NOF-FR.pdf,width=0.7\textwidth}}
  \caption{Canal Gaussien \`{a} interf\'{e}rence avec voie de retour d\'{e}grad\'{e}e par un bruit additif \`{a} la $n$-i\`eme utilisation du canal.}
  \label{Fig:G-IC-NOFfr}
\end{figure}



Le GIC-NOF \`{a} deux utilisateurs repr\'{e}sent\'{e} par la Figure~\ref{Fig:G-IC-NOFfr} peut \^{e}tre d\'{e}crit par six param\`{e}tres :  $\overrightarrow{\SNR}_i$, $\overleftarrow{\SNR}_i$, et $\INR_{ij}$, avec $i \in \{1,2\}$ et $j \in \{1,2\} \backslash \{i\}$, d\'{e}finis comme suit :
%
\begin{subequations}
\label{EqGICNOFparametersfr}
\begin{IEEEeqnarray}{rcl}
\label{EqSNWIRwdfr}
\overrightarrow{\SNR}_i &=& \overrightarrow{h}_{ii}^2, \\
\label{EqINRijfr}
\INR_{ij}&=& h_{ij}^2, \textrm{ et } \\
\label{EqSNRibwdfr}
\overleftarrow{\SNR}_i&=&\overleftarrow{h}_{ii}^2\left(\overrightarrow{h}_{ii}^2 + 2\overrightarrow{h}_{ii}h_{ij}+h_{ij}^2+1\right). 
\end{IEEEeqnarray}
\end{subequations}
%
Lorsque $\INR_{ij} \leqslant 1$, la paire d'\'{e}metteur-r\'{e}cepteur $i$ est alt\'{e}r\'{e}e principalement par le bruit au lieu de l'interf\'{e}rence. Dans ce cas, le traitement de l'interf\'{e}rence comme un bruit est optimal et la voie de retour n'apporte pas d'am\'{e}lioration significative du d\'{e}bit. C'est la raison pour laquelle l'analyse d\'{e}velopp\'{e}e dans cette th\`{e}se traite exclusivement le cas dans lequel $\INR_{ij} > 1$ pour tout $i \in \lbrace1, 2\rbrace$ et $j \in \lbrace 1, 2 \rbrace \setminus \lbrace i \rbrace$. 

\subsection{Canal Lin\'{e}aire D\'{e}terministe \`{a} Interf\'{e}rence }  \label{SectCLDICNOFfr}

On consid\`{e}re le canal lin\'{e}aire d\'eterministe \`{a} interf\'{e}rence   avec r\'etroalimentation d\'egrad\'ee par un bruit additif (LDIC-NOF) repr\'{e}sent\'{e} sur la Figure \ref{FigLDIC-NOFfr}. 
%
Pour tout $i \in \lbrace 1, 2 \rbrace$ et $j\in \lbrace 1, 2 \rbrace\setminus\lbrace i \rbrace$, le nombre de tubes pour les bits entre l'\'emetteur $i$ et son r\'ecepteur associ\'{e} (r\'ecepteur $i$) est not\'{e} par $\overrightarrow{n}_{ii}$; le nombre de voies pour les bits entre l'\'emetteur $i$ et l'autre r\'ecepteur (r\'ecepteur $j$)  est not\'{e} par $n_{ji}$; enfin le nombre de tubes pour les bits entre le r\'ecepteur $i$ et son \'emetteur correspondant est not\'{e} par  $\overleftarrow{n}_{ii}$. Ces six param\`{e}tres sont des entiers positifs et d\'ecrivent le LDIC-NOF repr\'esent\'e sur la Figure \ref{FigLDIC-NOFfr}.

A l'\'emetteur $i$, durant la $n$-i\`eme utilisation du canal, o\`u $n \in \lbrace 1, 2,  \ldots, N \rbrace$, le symbole en entr\'ee, not\'e $\vec{X}_{i,n}$ est un vecteur binaire de longueur $q$, c'est-\`a-dire $\vec{X}_{i,n} = \Big(X_{i,n}^{(1)}$, $X_{i,n}^{(2)}, \ldots$, $X_{i,n}^{(q)}\Big)^{\sfT} \in \mathcal{X}_i$, avec $\mathcal{X}_i = \lbrace 0, 1 \rbrace^{q}$,  $q=\ds\max \Big(\overrightarrow{n}_{11}$, $\overrightarrow{n}_{22}$, $n_{12}$, $n_{21}\Big)$, et $N \in \mathds{N}$ est la longueur de bloc. 
%
Au r\'ecepteur $i$, durant la $n$-i\`eme utilisation du canal, o\`u $n \in \lbrace 1$, $2,  \ldots$, $\max\left(N_1,N_2\right) \rbrace$, le symbole \`{a} la sortie du canal $i$, not\'e $\overrightarrow{\vec{Y}}_{i,n}$, est \'{e}galement un vecteur binaire de longueur $q$, c'est-\`a-dire $\overrightarrow{\vec{Y}}_{i,n} = \Big(\overrightarrow{Y}_{i,n}^{(1)}$, $\overrightarrow{Y}_{i,n}^{(2)}, \ldots$, $\overrightarrow{Y}_{i,n}^{(q)}\Big)^{\sfT}$. 
%
Soit $\vec{S}$ une matrice $q\times q$ \`{a} d\'{e}calage.

\begin{figure}[t!]
 \centerline{\epsfig{figure=Figures/IC-NOF-LDM-FR.pdf,width=0.7\textwidth}}
\caption{Canal lin\'{e}aire d\'{e}terministe \`{a} interf\'{e}rence \`{a} deux utilisateurs avec voie de retour d\'{e}grad\'{e}e par un bruit additif \`{a} la  $n$-i\`eme utilisation du canal.} 
  \label{FigLDIC-NOFfr}
\end{figure}

Les entr\'{e}es-sorties de ce canal durant la $n$-i\`eme utilisation du canal sont li\'{e}es par les relations suivantes : 
%
\begin{IEEEeqnarray}{lcl}
\label{EqLDICsignalsfr}
\overrightarrow{\vec{Y}}_{i,n}&=& \vec{S}^{q - \overrightarrow{n}_{ii}} \vec{X}_{i,n} + \vec{S}^{q - n_{ij}} \vec{X}_{j,n},
\end{IEEEeqnarray}
%
pour tout $i \in \lbrace 1, 2 \rbrace$ et $j\in \lbrace 1, 2 \rbrace\setminus\lbrace i \rbrace$.
%o\`{u} ${\vec{X}_{i,n} = \left(0, 0, \ldots, 0\right)^{\sfT}}$ quelque soit $n > N_i$.

Le signal d\'egrad\'e par un bruit additif dans la voie de retour est disponible \`{a} l'\'{e}metteur $i$ \`{a} la fin de la $n$-i\`eme utilisation du canal est : 
%%
\begin{IEEEeqnarray}{lcl}\label{EqLDICsignalscfr}
\left(\left(0, \ldots, 0\right), \vec{\overleftarrow{Y}}_{i,n}^{\sfT} \right)^{\sfT} &=& \vec{S}^{\left(\max(\overrightarrow{n}_{ii},n_{ij})-\overleftarrow{n}_{ii}\right)^+} \, \vec{\overrightarrow{Y}}_{i,n-d}, \quad
\end{IEEEeqnarray}
%
o\`{u} $d \in \mathds{N}$ est un d\'{e}lai limit\'{e}. On notera que les additions et les multiplications sont en binaire.
%
La dimension du vecteur $\left(0,  \ldots,  0\right)$ dans \eqref{EqLDICsignalscfr} est $q  -  \min \big(\overleftarrow{n}_{ii}, \max(\overrightarrow{n}_{ii}, n_{ij}) \big)$ et le vecteur \hspace{3mm}$\vec{\overleftarrow{Y}}_{i,n}$ repr\'{e}sente les \hspace{3mm}$\min \big(\overleftarrow{n}_{ii}, \max(\overrightarrow{n}_{ii},n_{ij}) \big)$ bits moins significatifs de $\vec{S}^{\left(\max(\overrightarrow{n}_{ii},n_{ij})-\overleftarrow{n}_{ii}\right)^+} \vec{\overrightarrow{Y}}_{i,n-d}$.

Sans perte de g\'{e}n\'{e}ralit\'{e}, le d\'{e}lai de la voie de retour est suppos\'e correspondre \`a une seule utilisation du canal.

\section{Canaux \`{a} Interf\'{e}rence D\'{e}centralis\'{e}s}\label{Chapter5bfr}

Dans un syst\`{e}me d\'{e}centralis\'{e}, il n'existe pas de contr\^{o}leur central, et chaque paire d'\'{e}metteur-r\'{e}cepteur est responsable de la s\'{e}lection de sa propre configuration d'\'{e}mission-r\'{e}ception pour maximiser son d\'{e}bit de transmission de donn\'{e}es.
%
La configuration de transmission-r\'eception, not\'{e}e $s_i$, avec $i \in \lbrace 1,2 \rbrace$,  peut \^etre caract\'{e}ris\'{e} par la longueur de bloc $N_i$, le nombre de bits par bloc $M_i$, l'alphabet d'entr\'ee $\mathcal{X}_i$, le dictionnaire, les fonctions d'encodage $f_{i}^{(1)}$, $f_{i}^{(2)}, \ldots$, $f_{i}^{(N_i)}$, les fonctions de decodage $\psi_i^{(N)}$, etc. 
%
Le but de l'\'emetteur $i$ est de choisir en toute autonomie sa configuration de transmission-r\'eception, pour maximiser son taux de transmission atteignable $R_i$. 
%
Il convient de noter que le taux de transmission atteignable par l'\'emetteur-r\'ecepteur $i$ d\'{e}pend des configurations $s_1$ et $s_2$ en raison de l'interf\'{e}rence mutuelle. Ceci est r\'{e}v\'{e}lateur de l'interaction comp\'{e}titive entre les deux liens de communication du canal \`{a} interf\'{e}rence d\'ecentralis\'e. 

Les mod\`{e}les de syst\`{e}mes pour le IC-NOF continu d\'{e}centralis\'{e} \`{a} deux utilisateurs, le D-GIC-NOF \`{a} deux utilisateurs et le D-LDIC-NOF \`{a} deux utilisateurs sont en g\'{e}n\'{e}ral les m\^{e}mes que pour le cas centralis\'{e}. Les principales diff\'{e}rences sont les suivantes : 

\begin{itemize}
\item Chaque \'{e}metteur-r\'{e}cepteur d\'{e}finit le nombre d'utilisations du canal par bloc, \`{a} savoir les utilisations du canal $N_1$ et $N_2$. 
\item La transmission d'un bloc est constitu\'{e}e de $N$ utilisations du canal, o\`{u} $N=\max\left(N_1,N_2\right)$. Alors, $X_{i,n}=0$ pour tout $n>N_i$. 
\item L'encodeur $i$ g\'{e}n\`{e}re le symbole $x_{i,n}$ en tenant compte non seulement de l'indice de message $W_i \in \mathcal{W}_i=\lbrace 1,2, \ldots, 2^{N_iR_i}\rbrace$ et de toutes les sorties pr\'{e}c\'{e}dentes de la voie de retour $i$, \`{a} savoir, $\Big(\overleftarrow{y}_{i,1}$, $\overleftarrow{y}_{i,2}$, $\ldots$, $\overleftarrow{y}_{i,n-1}\Big)$, mais aussi de l'indice de message al\'{e}atoire $\Omega_i \in \mathds{N}$. L'indice $\Omega_i$ est un indice suppl\'{e}mentaire g\'{e}n\'{e}r\'{e} de fa\c{c}on al\'{e}atoire suppos\'{e} \^{e}tre connu \`{a} l'\'{e}metteur $i$ et au r\'{e}cepteur $i$, mais inconnu \`{a} l'\'{e}metteur $j$ et au r\'{e}cepteur $j$ (caract\`{e}re al\'{e}atoire commun). 
\item \`{A} la fin de la transmission, le d\'{e}codeur $i$ utilise toutes les sorties de canal, \`{a} savoir, $\Big(\overrightarrow{y}_{i,1}$, $\overrightarrow{y}_{i,2}, \ldots$, $\overrightarrow{y}_{i,N}\Big)$ et l'indice de message al\'{e}atoire $\Omega_i$ pour estimer l'indice de message $W_i$, indiqu\'{e}e par $\widehat{W}_i$. 
\item La cha\^{i}ne de Markov suivante existe : 
%
\begin{equation}
\label{EqMarkovChainDMGDfr}
\Big(W_i, \Omega_i, \overleftarrow{\vec{Y}}_{i,(1;n-1)}\Big) \rightarrow X_{i,n} \rightarrow \overrightarrow{Y}_{i,n}. 
 \end{equation}
\item Le calcul de la probabilit\'{e} d'erreur est effectu\'{e} pour chacune des paires \'{e}metteur-r\'{e}cepteur. 
%
Soit $W_i^{(t)}$ indiqu\'{e} comme $c_{i,1}^{(t)} \, c_{i,2}^{(t)} \, \ldots \, c_{i,M_i}^{(t)}$ sous forme binaire.  Soit aussi $\widehat{W}_i^{(t)}$ indiqu\'{e} comme $\widehat{c}_{i,1}^{(t)} \, \widehat{c}_{i,2}^{(t)} \, \ldots \, \widehat{c}_{i,M_i}^{(t)}$ sous forme binaire. La probabilit\'{e} d'erreur moyenne de bit au niveau du d\'{e}codeur $i$ compte tenu des configurations $s_1$ et $s_2$, not\'{e}e $p_{i}(s_1,s_2)$, est alors donn\'{e}e par
%
\begin{IEEEeqnarray}{rcl}
\label{EqbitErrorProbGDfr}   
p_{i}(s_1,s_2)   &=& \frac{1}{M_i} \ds\sum_{\ell = 1}^{M_i} \ind{\widehat{c}_{i,\ell}^{(t)} \neq {c}_{i,\ell}^{(t)} }. 
\end{IEEEeqnarray}
%
 \end{itemize}

Les limites fondamentales dans un syst\`{e}me IC-NOF d\'{e}centralis\'{e} \`{a} deux utilisateurs sont d\'{e}finies par la r\'{e}gion d'$\eta$-\'{e}quilibre de Nash $\Nldicnof$.

\begin{definition-fr}[R\'{e}gion d'$\eta$-\'{E}quilibre de Nash d'un IC \`{a} Deux Utilisateurs]\label{DefNashRegion2ICfr}
La r\'{e}gion d'$\eta$-\'{e}quilibre de Nash $\Nldicnof$ d'un IC \`{a} deux utilisateurs est la fermeture de l'ensemble de toutes les paires possibles de d\'{e}bit atteignables $(R_1,R_2) \in \mathds{R}_+^{2}$ qui sont stables dans le sens d'un $\eta$-\'{e}quilibre de Nash. Plus pr\'{e}cis\'{e}ment, \'{e}tant donn\'{e} un sch\'{e}ma de codage atteignant l'\'{e}quilibre de Nash, il n'existe pas de sch\'{e}ma de codage alternatif pour une ou l'autre des paires \'{e}metteur-r\'{e}cepteur augmentant leurs d\'{e}bits individuels de plus de $\eta$ bits par utilisation du canal.
\end{definition-fr}

\subsection{Formulation du Jeu}\label{SecGameFormulationfr}

L'int\'{e}raction comp\'{e}titive des deux paires \'emetteur-r\'ecepteur dans le canal \`{a} interf\'{e}rence  d\'ecentralis\'e peut \^etre mod\'elis\'ee par un jeu sous forme normale suivant : 
%
\begin{equation}\label{EqGamefr}
\GameNF.
\end{equation}
%
L'ensemble $\mathcal{K} = \lbrace 1, 2 \rbrace$ est l'ensemble des joueurs, c'est-\`a-dire, l'ensemble des paires \'emetteur-r\'ecepteur. Les ensembles $\mathcal{A}_1$ et $\mathcal{A}_2$ sont les ensembles d'actions des  joueurs  $1$ et $2$, respectivement. Une action du joueur $i \in \mathcal{K}$, not\'{e}e par $s_i \in \mathcal{A}_i$, correspond \`a sa configuration de transmission-r\'eception comme indiqu\'e pr\'ec\'edemment. 
%
La fonction d'utilit\'e du joueur $i$ est $u_i : \mathcal{A}_1 \times \mathcal{A}_2 \rightarrow \mathds{R}_+$, et est d\'efinie  comme le taux de transmission de l'\'emetteur $i$,
\begin{equation}
\label{EqUtilityfr}
u_i(s_1,s_2) = \left\lbrace
\begin{array}{lcl}
R_i=\frac{M_i}{N_i} & \mbox{if} &  p_{i}(s_1,s_2)  < \epsilon \\
0 & &  \mbox{otherwise}
\end{array},
\right.
\end{equation}
o\`{u} $\epsilon > 0$ est un nombre arbitrairement petit.
%
Ce jeu sous forme normale fut propos\'{e} en premier lieu par  \cite{Yates-ISIT-2008} et \cite{Berry-ISIT-2008}.

Une classe de configurations de transmission-r\'eception $\vec{s}^* = (s_1^*, s_2^*) \in \mathcal{A}_1 \times \mathcal{A}_2$, particuli\`erement importantes dans l'analyse de ce jeu est d\'esign\'ee comme l'ensemble d'$\eta$-\'{e}quilibre de Nash. Cette classe de configurations satisfait la d\'efinition suivante:
%
\begin{definition-fr}[$\eta$-\'equilibre de Nash] \label{DefEtaNEfr} %\emph{
Dans le jeu \quad $\mathcal{G} = \big(\mathcal{K}$, $\left\lbrace\mathcal{A}_k \right\rbrace_{k \in \mathcal{K}}$, $\left\lbrace u_{k}\right\rbrace_{ k \in \mathcal{K}}\big)$, un profil d'actions $(s_1^*, s_2^*)$ est un $\eta$-\'equilibre de Nash si pour tout $i \in \mathcal{K}$ et pour tout $s_i \in \mathcal{A}_i$, il existe un $\eta > 0$ tels que
\begin{equation}\label{EqNashEquilibriumfr}
u_i (s_i , s_j^*) \leqslant u_i (s_i^*, s_j^*) + \eta.
\end{equation}
%}
\end{definition-fr}

Soit $(s_1^*, s_2^*)$ un profil d'actions d'un $\eta$-\'equilibre de Nash. Il s'en suit qu'aucun des \'emetteurs ne peut augmenter son taux de transmission de plus de $\eta$ bits par utilisation du canal en changeant sa configuration de transmission-r\'eception tout en conservant la probabilit\'e d'erreur binaire moyenne arbitrairement proche de z\'ero. 
%
Il convient de noter que si $\eta$ est  suffisamment \'elev\'e, il suit de la D\'efinition  \ref{DefEtaNEfr}, que toute paire de configurations peut \^etre un $\eta$-\'{e}quilibre de Nash. D'autre part, pour $\eta=0$, la d\'efinition classique de l'\'{e}quilibre de Nash est obtenue \cite{Nash-PNAS-1950}. Dans ce cas, si une paire de configurations est un \'equilibre de Nash ($\eta=0$), alors chaque configuration individuelle est optimale \'{e}tant donn\'{e}e \`a la configuration de l'autre paire \'emetteur-r\'ecepteur. Par cons\'equent, l'objet est de d\'ecrire l'ensemble de toutes les paires de taux de transmission $(R_1,R_2)$ $\eta$-\'{e}quilibre de Nash du jeu d\'efinit par \eqref{EqGamefr} avec la plus petite valeur possible de $\eta$ pour lequel il existe au moins une configuration d'\'equilibre.

L'ensemble des paires de taux de transmission atteignables dans un $\eta$-\'{e}quilibre de Nash est connu comme la r\'{e}gion d'$\eta$-\'{e}quilibre de Nash.
%
\begin{definition-fr}[La R\'{e}gion d'$\eta$-\'{E}quilibre de Nash] \label{DefNERegionfr} 
%\emph{
Soit $\eta > 0$ fix\'e. Une paire de taux de transmission atteignables $(R_1,R_2)$ appartient \`a la r\'{e}gion d'$\eta$-\'{e}quilibre de Nash du jeu $\mathcal{G} = \big(\mathcal{K}$, $\left\lbrace\mathcal{A}_k \right\rbrace_{k \in \mathcal{K}}$,  $\left\lbrace
u_{k}\right\rbrace_{k \in \mathcal{K}}\big)$ s'il existe une paire $(s_1^*, s_2^*) \in \mathcal{A}_1 \times \mathcal{A}_2$  qui  est  telle que 
\begin{eqnarray}
u_1 (s_1^* , s_2^*)  =  R_1 & \mbox{ et } & u_2 (s_1^* , s_2^*)  =  R_2. 
\end{eqnarray}
%}
\end{definition-fr}

\section{Connexions entre Canaux Lin\'{e}aires D\'{e}terministes \`{a} Interf\'{e}rence  et Canaux Gaussiens \`{a} Interf\'{e}rence}\label{ChapterConnectionsGLDMfr}

La r\'{e}gion de capacit\'{e} du GIC-NOF \`{a} deux utilisateurs avec les param\`{e}tres  $\overrightarrow{\SNR}_{1}$, $\overrightarrow{\SNR}_{2}$, $\INR_{12}$, $\INR_{21}$, $\overleftarrow{\SNR}_{1}$ et $\overleftarrow{\SNR}_{2}$
 peut-\^{e}tre d\'{e}crite approximativement par la r\'{e}gion de capacit\'{e} d'un LDIC-NOF avec des param\`{e}tres $\overrightarrow{n}_{ii} = \left \lfloor \frac{1}{2}\log(\overrightarrow{\SNR}_{i}) \right \rfloor$; $n_{ij}= \left \lfloor \frac{1}{2}\log(\INR_{ij}) \right \rfloor$; ${\overleftarrow{n}_{ii}= \left \lfloor \frac{1}{2}\log(\overleftarrow{\SNR}_{i}) \right \rfloor}$, avec $i \in \lbrace 1, 2 \rbrace$ et $j \in \lbrace 1, 2 \rbrace\setminus\lbrace i \rbrace$. 

\section{Principaux R\'{e}sultats du Canal Lin\'{e}aire D\'{e}terministe \`{a} Interf\'{e}rence  Centralis\'{e}}\label{Chapter6fr}

Cette section pr\'{e}sente les principaux r\'{e}sultats sur le LDIC-NOF centralis\'{e} \`{a} deux utilisateurs d\'{e}crit en Section~\ref{SectCLDICNOFfr}.  

\subsection {Region de Capacit\'{e}} \label{SectCapLDICNOFfr}

Notons $\Cldicnof(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}, n_{21}$, $ \overleftarrow{n}_{11} , \overleftarrow{n}_{22})$ la r\'{e}gion de capacit\'{e} du LDIC-NOF \`{a} deux utilisateurs avec les param\`{e}tres $\overrightarrow{n}_{11}$, $\overrightarrow{n}_{22}$, $n_{12}$, $n_{21}$, $\overleftarrow{n}_{11}$, et $\overleftarrow{n}_{22}$, caract\'{e}ris\'{e}e par le Th\'{e}or\`{e}me~\ref{TheoremANFBLDMCapfr}. 

%theorem style=margin apart,left=10mm, right=10mm
\begin{thm-fr}[, label=TheoremANFBLDMCapfr]{Region de capacit\'{e}}{} 
La r\'{e}gion de capacit\'{e} $\Cldicnof(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}, n_{21}, \overleftarrow{n}_{11} , \overleftarrow{n}_{22})$ du LDIC-NOF \`{a} deux utilisateurs est l'ensemble des paires de d\'{e}bit $(R_1,R_2) \in \mathds{R}_{+}^2$ qui pour tout $i \in \lbrace 1, 2 \rbrace$, avec $j\in\lbrace 1, 2 \rbrace\setminus\lbrace i \rbrace$ : 
%
\begin{subequations}
\begin{IEEEeqnarray}{rcl}
\label{EqRiV2fr}
R_{i}& \leqslant & \min\left(\max\left(\overrightarrow{n}_{ii},n_{ji}\right),\max\left(\overrightarrow{n}_{ii},n_{ij}\right)\right), \\
\label{EqRi-2-V2fr}
R_i& \leqslant &\min\left(\max\left(\overrightarrow{n}_{ii},n_{ji}\right),\max\left(\overrightarrow{n}_{ii},\overleftarrow{n}_{jj}-\left(\overrightarrow{n}_{jj}-n_{ji}\right)^+\right)\right), \\
\nonumber
R_1+R_2  &\leqslant& \min \left(\max\left(\overrightarrow{n}_{22},n_{12}\right)+\left(\overrightarrow{n}_{11}-n_{12}\right)^+, \max\left(\overrightarrow{n}_{11},n_{21}\right)+\left(\overrightarrow{n}_{22}-n_{21}\right)^+\right), \\
\label{EqRi+Rj-1-V2fr}
\nonumber
R_1+R_2 &\leqslant& \max\Big(\left(\overrightarrow{n}_{11}-{n}_{12} \right)^+, n_{21}, \overrightarrow{n}_{11}-\left(\max\left(\overrightarrow{n}_{11},n_{12}\right)-\overleftarrow{n}_{11}\right)^+\Big)\\
 \label{EqRi+Rj-2-V2fr}  
 & &+\max\Big(\left(\overrightarrow{n}_{22}-{n}_{21} \right)^+, n_{12}, \overrightarrow{n}_{22}-\left(\max\left(\overrightarrow{n}_{22},n_{21}\right)-\overleftarrow{n}_{22}\right)^+\Big), \\
%\end{IEEEeqnarray}
%%%
%\begin{IEEEeqnarray}{rcl}
\nonumber
2R_i+R_j  &\leqslant& \max\left(\overrightarrow{n}_{ii},{n}_{ji} \right) \! + \! \left(\overrightarrow{n}_{ii} \! - \! {n}_{ij} \right)^+ \! \\
\label{Eq2Ri+Rj-V2fr}
& & + \! \max\Big(\! \left(\overrightarrow{n}_{jj} \! - \! {n}_{ji} \right)^+, n_{ij}, \overrightarrow{n}_{jj} \! - \! \left(\max\left(\overrightarrow{n}_{jj},{n}_{ji} \right)-\overleftarrow{n}_{jj}\right)^+ \! \Big). \qquad
\end{IEEEeqnarray}
\end{subequations}
\end{thm-fr} 

\subsection {Cas o\`{u} la Voie de Retour Agrandit la R\'{e}gion de Capacit\'{e}} \label{SectThLDICNOFfr}

Soit $\alpha_i \in \mathds{Q}$, avec $i \in \lbrace 1, 2 \rbrace$ et ${j \in \lbrace 1, 2\rbrace\setminus\lbrace i \rbrace}$ d\'{e}fini comme
\begin{equation}
\label{DefAlphaLDMfr}
\alpha_i = \frac{n_{ij}}{\overrightarrow{n}_{ii}}.
\end{equation}
%
Pour chaque paire d'\'{e}metteur-r\'{e}cepteur $i$, il existe cinq r\'{e}gimes d'interf\'{e}rence (IR) possibles, comme sugg\'{e}r\'{e} en \cite{Etkin-TIT-2008} :  le IR tr\`{e}s faible (VWIR), \`{a} savoir, $ \alpha_i \leqslant \frac{1}{2}$, le IR faible (WIR), \`{a} savoir, $ \frac{1}{2} < \alpha_i \leqslant \frac{2}{3}$, le IR mod\'{e}r\'{e} (MIR), \`{a} savoir,  $ \frac{2}{3} < \alpha_i < 1$, le IR fort (SIR), \`{a} savoir, $ 1 \leqslant \alpha_i \leqslant 2$ et le IR tr\`{e}s fort (VSIR), \`{a} savoir, $ \alpha_i > 2 $. 
%
Les sc\'{e}narios dans lesquels le signal souhait\'{e} est plus fort que l'interf\'{e}rence ($ \alpha_i < 1$), notamment les VWIR, WIR, et MIR, sont cit\'{e}s comme les r\'{e}gimes \`{a} faible interf\'{e}rence (LIR). A l'inverse, les sc\'{e}narios dans lesquels le signal souhait\'{e} est plus faible ou \'{e}gal \`{a} l'interf\'{e}rence ($ \alpha_i \geqslant 1$), \`{a} savoir le SIR et le VSIR, sont consid\'{e}r\'{e}s comme des r\'{e}gimes \`{a} hautes interf\'{e}rence (HIR).


Les r\'{e}sultats de cette section sont pr\'{e}sent\'{e}s au moyen d'un ensemble d'\'{e}v\'{e}nements (variables bool\'{e}ennes) d\'{e}termin\'{e}s par les param\`{e}tres $\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}$, et $n_{21}$. \'{E}tant donn\'{e} un quadruplet d\'{e}termin\'{e} $(\overrightarrow{n}_{11}$, $\overrightarrow{n}_{22}$, $n_{12}$, $n_{21})$, les \'{e}v\'{e}nements sont d\'{e}finis ci-dessous : 
%
\begin{IEEEeqnarray}{lc}
\label{Event1fr}
E_1 :  	\qquad	& 	\alpha_1 <1 \land \alpha_2  <  1, \\
\label{Event2fr}
E_{2,i} :  \qquad	& 	\alpha_i  \leqslant  \frac{1}{2} \land 1 \leqslant	\alpha_j\leqslant  2, \\
\label{Event3fr}
E_{3,i} :   \qquad	&  	\alpha_i  \leqslant  \frac{1}{2} \land \alpha_j  > 2,  \\
\label{Event4fr}
E_{4,i} :  \qquad 	& \frac{1}{2}  <	\alpha_i \leqslant \frac{2}{3} \land \alpha_j	 \geqslant  1, 
\end{IEEEeqnarray}
%%%
\begin{IEEEeqnarray}{lc}
\label{Event5fr}
E_{5,i} :  \qquad	& \frac{2}{3} < \alpha_i < 1 \land \alpha_j \geqslant  1, \\
\label{Event6fr}
E_{6,i} :   \qquad	&\frac{1}{2} < \alpha_i \leqslant	 1 \land \alpha_j > 1,    \\ 
\label{Event7fr}
E_{7,i} :  \qquad	& \alpha_i	 \geqslant	1 \land  \alpha_j \leqslant 1,  \\
\label{Event8fr}
E_{8,i} :   \qquad	 &	\overrightarrow{n}_{ii} >  n_{ji}, \\
\label{Event9fr}
E_{9} :   \qquad	&	\overrightarrow{n}_{11}+\overrightarrow{n}_{22}	 >  n_{12}+n_{21}, \\
\label{Event10fr}
E_{10,i} :   \qquad	&	\overrightarrow{n}_{ii}+\overrightarrow{n}_{jj}  >  n_{ij}+2n_{ji}, \\
\label{Event11fr}
E_{11,i}:  \qquad	&	\overrightarrow{n}_{ii}+\overrightarrow{n}_{jj}	 <  n_{ij}.
\end{IEEEeqnarray}


Dans le cas de $E_{8,i} : \overrightarrow{n}_{ii} >  n_{ji}$, la notation $\widetilde{E}_{8,i}$ indique $\overrightarrow{n}_{ii} <  n_{ji}$; la notation $\overline{E}_{8,i}$ indique $\overrightarrow{n}_{ii} \leqslant  n_{ji}$ (compl\'{e}ment logique); et la notation $\check{E}_{8,i}$ indique $\overrightarrow{n}_{ii} \geqslant  n_{ji}$. Dans le cas $E_{1} :  \alpha_1 <1 \land \alpha_2  <  1$, la notation $\widetilde{E}_{1}$ indique $\alpha_1 > 1 \land \alpha_2  > 1$; et la notation $\overline{E}_{1}$ indique $\alpha_1 \geqslant 1 \land \alpha_2  \geqslant  1$. Dans le cas $E_{9} :  \overrightarrow{n}_{11}+\overrightarrow{n}_{22}	 >  n_{12}+n_{21}$, la notation $\overline{E}_{9}$ indique $\overrightarrow{n}_{11}+\overrightarrow{n}_{22} \leqslant  n_{12}+n_{21}$. 


En combinant les \'{e}v\'{e}nements \eqref{Event1fr}-\eqref{Event11fr}, cinq sc\'{e}narios principaux sont identifi\'{e}s : 
%
\begin{IEEEeqnarray}{lll}
\label{S1ifr}
S_{1,i} & :  \,& \left(E_1 \land E_{8,i}\right) \! \lor \! \left(E_{2,i} \land E_{8,i}\right) \! \lor \! \left(E_{3,i} \! \land \! E_{8,i} \! \land \! E_{9}\right) \! \lor \! \left(E_{4,i} \! \land \! E_{8,i} \! \land \! E_{9}\right) \! \lor \! \left(E_{5,i} \! \land \! E_{8,i} \! \land \! E_{9}\right), \qquad\\
\label{S2ifr}
S_{2,i} & :  \,& \left(E_{3,i} \land \widetilde{E}_{8,j}  \land \overline{E}_{9}\right) \lor \left(E_{6,i} \land \widetilde{E}_{8,j}  \land \overline{E}_{9}\right) \lor \left(\widetilde{E}_1 \land \widetilde{E}_{8,j}\right), \\
\nonumber
S_{3,i} & :  \,& \left(E_{1} \land \overline{E}_{8,i}\right) \lor \left(E_{2,i} \land \overline{E}_{8,i}\right) \lor \left(E_{3,i} \land \check{E}_{8,j} \land \overline{E}_{8,i}\right) \lor \left(E_{4,i} \land \check{E}_{8,j} \land \overline{E}_{8,i}\right)   \\
\label{S3ifr}
 & &  \lor \left(E_{5,i} \land \check{E}_{8,j} \land \overline{E}_{8,i}\right) \lor \left(\overline{E}_1 \land \check{E}_{8,j} \right) \lor \left(E_{7,i} \right), \\
\label{S4ifr}
S_{4} & :  \,& E_{1} \land E_{8,1} \land E_{8,2} \land E_{10,1} \land E_{10,2}, \\
\label{S5ifr}
S_{5} & :  \,& \overline{E}_{1} \land E_{11,1} \land E_{11,2}.
\end{IEEEeqnarray}
%
Pour tout $i \in \lbrace 1, 2 \rbrace$, les \'{e}v\'{e}nements $S_{1,i}$, $S_{2,i} $,  $S_{3,i}$, $S_4$ et $S_5$  montrent les propri\'{e}t\'{e}s \'{e}num\'{e}r\'{e}es par les corollaires suivants.
%
\begin{corollary-fr} \label{LemmaProperSetfr} \emph{
Pour tout $(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}, n_{21}) \in \mathds{N}^{4}$, \'{e}tant donn\'{e} un $i \in \lbrace 1, 2 \rbrace$ d\'{e}termin\'{e}, seul un des \'{e}v\'{e}nements $S_{1,i}$, $S_{2,i}$ et $S_{3,i}$ est vrai.
}
\end{corollary-fr}
%
\begin{corollary-fr} \label{LemmaProperSet2fr} \emph{
Pour tout $(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}, n_{21}) \in \mathds{N}^{4}$, lorsque l'un des \'{e}v\'{e}nements $S_{4}$ ou $S_{5}$ est vrai, l'autre est n\'{e}cessairement faux.
}
\end{corollary-fr}

\indent
Notez que le Corollaire \ref{LemmaProperSet2fr} n'exclut pas le cas dans lequel les deux $S_{4}$ et $S_{5}$ sont simultan\'{e}ment faux.

\begin{corollary-fr} \label{LemmaProperSet3fr} \emph{
Pour tout $(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}, n_{21}) \in \mathds{N}^{4}$, si $S_{4}$ est vrai, alors $S_{1,1}$ et $S_{1,2}$ sont tous deux vrais; et si $S_{5}$ est vrai, alors $S_{2,1}$ et $S_{2,2}$ sont tous deux vrais.
}
\end{corollary-fr}


\subsubsection{M\'{e}trique de l'Am\'{e}lioration de D\'{e}bit}\label{SectionRateImprovementMetricsfr}

\'{E}tant donn\'{e} un quadruplet $\left(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}, n_{21} \right)$, soit ${\Cldicnof(\overleftarrow{n}_{11} , \overleftarrow{n}_{22}) }$ la r\'{e}gion de capacit\'{e} d'un LDIC-NOF avec les param\`{e}tres $\overleftarrow{n}_{11}$ et $\overleftarrow{n}_{22}$.
%
L'am\'{e}lioration maximum des d\'{e}bits individuels $R_1$ et $R_2$, not\'{e}e respectivement par $\Delta_1(\overleftarrow{n}_{11}, \overleftarrow{n}_{22})$ et $\Delta_2(\overleftarrow{n}_{11}, \overleftarrow{n}_{22})$, due \`{a} l'effet de la voie de retour est : 
%
\begin{IEEEeqnarray}{lcl}
\nonumber
\Delta_{1}(\overleftarrow{n}_{11} , \overleftarrow{n}_{22} )  &=& \! \max_{0< R_{2} < R_{2}^*}  \Bigg \lbrace \! \sup \Big \lbrace R_{1} : (R_1, R_2) \in \Cldicnof(\overleftarrow{n}_{11}, \overleftarrow{n}_{22}) \Big \rbrace \!  -  \!  \sup \Big \lbrace R_1^{\dagger} : (R_1^{\dagger}, R_2)  \in \Cldicnof(0,0)  \Big \rbrace \Bigg \rbrace \\
\label{EqDelta1fr} 
\textrm{ et } \\
\nonumber
\Delta_{2}(\overleftarrow{n}_{11} , \overleftarrow{n}_{22} )  &=& \! \max_{0< R_{1} < R_{1}^*}  \Bigg \lbrace \! \sup  \Big \lbrace R_{2} : (R_1, R_2) \in \Cldicnof(\overleftarrow{n}_{11}, \overleftarrow{n}_{22}) \Big \rbrace  \! - \! \sup \Big \lbrace R_2^{\dagger} : (R_1,R_2^{\dagger})  \in \Cldicnof(0,0) \Big \rbrace  \Bigg \rbrace, \\
\label{EqDelta2fr} 
\end{IEEEeqnarray}
%
avec 
\begin{IEEEeqnarray}{lcl}
\label{EqDelta1astfr}
R_{1}^*  &=&  \sup  \Big \lbrace r_{1} : (r_1, r_2) \in \Cldicnof(0, 0)  \Big \rbrace  \textrm{ et }\\
\label{EqDelta2astfr}
R_{2}^*  &=&  \sup  \Big \lbrace r_{2} : (r_1, r_2) \in \Cldicnof(0, 0) \Big \rbrace.
\end{IEEEeqnarray}
%
Notons que pour tout $i\in \lbrace 1,2 \rbrace$, $\Delta_{i}(\overleftarrow{n}_{11} , \overleftarrow{n}_{22}) > 0$ si et seulement s'il est possible d'atteindre une paire de d\'{e}bits $(R_1,R_2) \in \mathds{R}_+^{2}$ avec une voie de retour telle que $R_i$ est sup\'{e}rieur au d\'{e}bit maximum atteignable par l'\'{e}metteur-r\'{e}cepteur $i$ sans voie de retour lorsque le d\'{e}bit de la paire \'{e}metteur-r\'{e}cepteur $j$ est fix\'{e} \`{a} $R_j$. \'{E}tant donn\'{e} les param\`{e}tres d\'{e}termin\'{e}s $\overleftarrow{n}_{11}$ et $\overleftarrow{n}_{22}$, l'assertion \emph{``le d\'{e}bit $R_i$ est am\'{e}lior\'{e} \`{a} l'aide de la voie de retour''} sert \`{a} indiquer que $\Delta_{i}(\overleftarrow{n}_{11} , \overleftarrow{n}_{22}) > 0$.

L'am\'{e}lioration maximum du d\'{e}bit somme $\Sigma(\overleftarrow{n}_{11} , \overleftarrow{n}_{22})$ concernant le cas sans voie de retour est : 
%
\begin{IEEEeqnarray}{lcl}
\nonumber
\Sigma(\overleftarrow{n}_{11}, \overleftarrow{n}_{22} )  &=& \sup \Big \lbrace R_{1}+R_{2} : (R_1, R_2) \in \Cldicnof(\overleftarrow{n}_{11}, \overleftarrow{n}_{22}) \Big \rbrace - \sup \Big \lbrace R_1^{\dagger}+R_2^{\dagger} : (R_1^{\dagger}, R_2^{\dagger})  \in \Cldicnof(0,0) \Big \rbrace.\\
\label{EqDeltaSumfr}
\end{IEEEeqnarray}
%
Notons que $\Sigma(\overleftarrow{n}_{11}, \overleftarrow{n}_{22} ) >0$ si et seulement s'il existe une paire de d\'{e}bits avec voie de retour dont la somme est sup\'{e}rieure au d\'{e}bit somme maximum atteignable sans voie de retour. \'{E}tant donn\'{e} les param\`{e}tres d\'{e}termin\'{e}s $\overleftarrow{n}_{11}$ et $\overleftarrow{n}_{22}$, l'assertion \emph{``le d\'{e}bit somme est am\'{e}lior\'{e} \`{a} l'aide de la voie de retour''} sert \`{a} impliquer que  $\Sigma(\overleftarrow{n}_{11}, \overleftarrow{n}_{22} ) >0$.


Lorsque la voie de retour est exclusivement utilis\'{e}e par la paire d'\'{e}metteur-r\'{e}cepteur $i$, \`{a} savoir, $\overleftarrow{n}_{ii}>0$ et $\overleftarrow{n}_{jj}=0$, l'am\'{e}lioration maximum du d\'{e}bit individuel de l'\'{e}metteur-r\'{e}cepteur $k$, avec $k \in \{1,2\}$, et l'am\'{e}lioration maximum du d\'{e}bit somme sont indiqu\'{e}es par $\Delta_{k}(\overleftarrow{n}_{ii})$ et $\Sigma(\overleftarrow{n}_{ii})$, respectivement. Par cons\'{e}quent, cette notation $\Delta_{k}(\overleftarrow{n}_{ii})$ remplace soit $\Delta_{k}(\overleftarrow{n}_{11},0)$ ou $\Delta_{k}(0, \overleftarrow{n}_{22})$, lorsque $i=1$ ou $i=2$, respectivement.  Il en va de m\^{e}me pour la notation $\Sigma(\overleftarrow{n}_{ii})$ qui remplace $\Sigma(\overleftarrow{n}_{11},0)$ ou $\Sigma(0, \overleftarrow{n}_{22})$, lorsque $i=1$ ou $i=2$, respectivement.

\subsubsection{Agrandissement de la R\'{e}gion de Capacit\'{e}} \label{SectEnlargeCfr}

Compte tenu des param\`{e}tres fix\'{e}s $(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}$,  $n_{21})$, $i \in \lbrace 1, 2 \rbrace$, et $j \in \lbrace 1, 2 \rbrace\setminus\lbrace i \rbrace$, la r\'{e}gion de capacit\'{e} d'un LDIC-NOF \`{a} deux utilisateurs, lorsque la voie de retour est disponible uniquement au niveau de la paire \'{e}metteur-r\'{e}cepteur $i$, \`{a} savoir, $\overleftarrow{n}_{ii} > 0$ et $\overleftarrow{n}_{jj} = 0$, est not\'{e} $\Cldicnof\left(\overleftarrow{n}_{ii}\right)$ au lieu de $\Cldicnof\left(\overleftarrow{n}_{11},0\right)$ ou $\Cldicnof\left(0,\overleftarrow{n}_{22}\right)$, quand $i = 1$ ou $i = 2$, respectivement.
 %
\`{A} la suite de cette notation, le Th\'{e}or\`{e}me \ref{TheoremLD-IC-NOF-Th1fr} identifie les valeurs exactes de $\overleftarrow{n}_{ii}$ pour lesquelles l'inclusion stricte de $\Cldicnof\left(0, 0\right) \subset \Cldicnof\left(\overleftarrow{n}_{ii}\right)$ vaut pour tout $i \in \lbrace 1,2 \rbrace$.
%
%theorem style=margin apart,left=10mm, right=10mm
\begin{thm-fr}[, label=TheoremLD-IC-NOF-Th1fr]{Agrandissement de la R\'{e}gion de Capacit\'{e}}{}
Soit $\left(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}, n_{21} \right) \in \mathds{N}^4$ un quadruplet fixe. Soit aussi $i \in \lbrace 1, 2 \rbrace$, $j \in \lbrace 1, 2 \rbrace\setminus\lbrace i \rbrace$ et $\overleftarrow{n}_{ii}^{*} \in \mathds{N}$ des nombres entiers fixes, avec
\begin{equation}
\label{Threshold1fr}
\overleftarrow{n}_{ii}^*=\left\{\begin{array}{ll}
\max\left(n_{ji},\left(\overrightarrow{n}_{ii}-n_{ij}\right)^+\right) & \text{ si } S_{1,i} \textrm{ est vrai}\\ 
\overrightarrow{n}_{jj}+\left(\overrightarrow{n}_{ii}-n_{ij}\right)^+ & \text{ si } S_{2,i}\textrm{ est vrai}
\end{array}.\right.
\end{equation}
%
Supposons que $S_{3,i}\textrm{ est vrai}$. Alors, pour tout $\overleftarrow{n}_{ii} \in \mathds{N}$, $\Cldicnof\Big(0, 0\Big)=\Cldicnof\Big(\overleftarrow{n}_{ii}\Big)$. 
%
Supposons aussi que $S_{1,i}\textrm{ est vrai}$ ou $S_{2,i}\textrm{ est vrai}$. Alors, pour tout $\overleftarrow{n}_{ii}\leqslant \overleftarrow{n}_{ii}^{*}$, $\Cldicnof\Big(0, 0\Big)=\Cldicnof\Big(\overleftarrow{n}_{ii}\Big)$ et pour tout $\overleftarrow{n}_{ii} > \overleftarrow{n}_{ii}^{*}$,   
$\Cldicnof\Big(0, 0\Big) \subset \Cldicnof\Big(\overleftarrow{n}_{ii}\Big)$.
%
\end{thm-fr} 
%



Le Th\'{e}or\`{e}me \ref{TheoremLD-IC-NOF-Th1fr} indique qu'\'{e}tant donn\'{e} l'\'{e}v\'{e}nement $S_{3,i}$ en \eqref{S3ifr}, l'impl\'{e}mentation de la voie de retour \`{a} la paire \'{e}metteur-r\'{e}cepteur  $i$, avec tout $\overleftarrow{n}_{ii} > 0$ et $\overleftarrow{n}_{jj} = 0$, n'agrandit pas la r\'{e}gion de capacit\'{e}. 
%
\'{E}tant donn\'{e} les \'{e}v\'{e}nements $S_{1,i}$ en \eqref{S1ifr} et $S_{2,i}$ en \eqref{S2ifr}, la r\'{e}gion de capacit\'{e} peut \^{e}tre agrandie lorsque $\overleftarrow{n}_{ii} > \overleftarrow{n}_{ii}^{*}$. 
%
Il importe de souligner que dans les cas dans lesquels la voie de retour agrandit la r\'{e}gion de capacit\'{e} du LDIC-NOF \`{a} deux utilisateurs, \'{e}tant donn\'{e} les \'{e}v\'{e}nements $S_{1,1}$, $S_{2,1}$, $S_{1,2}$ ou $S_{2,2}$, pour tout $i \in \lbrace 1,2 \rbrace$ et $j \in \lbrace 1, 2 \rbrace\setminus\lbrace i \rbrace$, ce qui suit est toujours vrai :  
\begin{equation}
\label{EqNiistarIneqfr}
\overleftarrow{n}_{ii}^{*} > (\overrightarrow{n}_{ii} - n_{ij})^{+}.
\end{equation}
%
En effet, l'in\'{e}galit\'{e} \eqref{EqNiistarIneqfr} d\'{e}voile une condition n\'{e}cessaire mais non suffisante pour agrandir la r\'{e}gion de capacit\'{e} \`{a} l'aide de la voie de retour. Cette condition indique que pour au moins un $i \in \lbrace 1,2 \rbrace$, avec  $j \in \lbrace 1,2 \rbrace\setminus \lbrace i \rbrace$,  l'\'{e}metteur $i$ puisse d\'{e}coder un sous-ensemble de bits d'information envoy\'{e}s par l'\'{e}metteur $j$ \`{a} chaque utilisation du canal.

Il est \'{e}galement int\'{e}ressant d'observer que, le seuil $\overleftarrow{n}_{ii}^{*}$ au-del\`{a} duquel la voie de retour est utile est diff\'{e}rent \'{e}tant donn\'{e} l'\'{e}v\'{e}nement $S_{1,i}$ en \eqref{S1ifr} et l'\'{e}v\'{e}nement $S_{2,i}$ en \eqref{S2ifr}. 
%
En g\'{e}n\'{e}ral, lorsque $S_{1,i}$ est vrai, l'agrandissement de la r\'{e}gion de capacit\'{e} est due au fait que la voie de retour permet d'utiliser \emph{l'interf\'{e}rence comme information secondaire} \cite{Shannon-IBM-1958}. 
%
Si $S_{2,i}$ en \eqref{S2ifr} est vrai, l'agrandissement de la r\'{e}gion de capacit\'{e} survient est comme une cons\'{e}quence du fait que certains bits ne pouvant \^{e}tre transmis directement de l'\'{e}metteur $j$ au r\'{e}cepteur $j$, peuvent parvenir au r\'{e}cepteur $j$ par un chemin alternatif :  \'{e}metteur $j$ - r\'{e}cepteur $i$ - \'{e}metteur $i$ - r\'{e}cepteur $j$.  
%


\subsubsection{Am\'{e}lioration du D\'{e}bit Individuel $R_i$ \`{a} l'Aide de la Voie de Retour dans le Lien $i$}
%
\'{E}tant donn\'{e} les param\`{e}tres fix\'{e}s $(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}$,  $n_{21})$, et $i \in \lbrace 1, 2 \rbrace$, l'impl\'{e}mentation de la voie de retour \`{a} la paire \'{e}metteur-r\'{e}cepteur  $i$ augmente le d\'{e}bit individuel $R_i$, \`{a} savoir, $\Delta_i(\overleftarrow{n}_{ii})>0$ pour certaines valeurs de $\overleftarrow{n}_{ii}$.
%
Le Th\'{e}or\`{e}me \ref{TheoremLD-IC-NOF-Th2fr} identifie les valeurs exactes de $\overleftarrow{n}_{ii}$ pour lesquelles $\Delta_i(\overleftarrow{n}_{ii})>0$.
%
%theorem style=margin apart,left=10mm, right=10mm
\begin{thm-fr}[, label=TheoremLD-IC-NOF-Th2fr]{Am\'{e}lioration de $R_i$ \`{a} l'Aide de la Voie de Retour dans le Lien $i$}{}
Soit $\left(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}, n_{21} \right) \in \mathds{N}^4$ un quadruplet fixe. Soit aussi $i \in \lbrace 1, 2 \rbrace$, $j \in \lbrace 1, 2 \rbrace\setminus\lbrace i \rbrace$ et $\overleftarrow{n}_{ii}^{\dagger} \in \mathds{N}$ des nombres entiers fixes, avec
%
\begin{equation}
\label{Eq:th2fr}
\overleftarrow{n}_{ii}^{\dagger}=\max\left(n_{ji},\left(\overrightarrow{n}_{ii}-n_{ij}\right)^+\right).
\end{equation}
%
Supposons que $S_{2,i}\textrm{ est vrai}$ ou $S_{3,i}\textrm{ est vrai}$. Alors, pour tout $\overleftarrow{n}_{ii} \in \mathds{N}$, $\Delta_{i}(\overleftarrow{n}_{ii})=0$.
%
Supposons que $S_{1,i}\textrm{ est vrai}$. Alors, si $\overleftarrow{n}_{ii} \leqslant \overleftarrow{n}_{ii}^{\dagger}$, cela signifie que $\Delta_{i}(\overleftarrow{n}_{ii})=0$;  et sinon $\overleftarrow{n}_{ii} > \overleftarrow{n}_{ii}^{\dagger}$, cela signifie que $\Delta_{i}(\overleftarrow{n}_{ii})>0$.
\end{thm-fr} 
%


Le Th\'{e}or\`{e}me  \ref{TheoremLD-IC-NOF-Th2fr} souligne qu'\'{e}tant donn\'{e} les \'{e}v\'{e}nements $S_{2,i}$ en \eqref{S2ifr} et $S_{3,i}$ en \eqref{S3ifr}, le d\'{e}bit individuel $R_i$ ne peut \^{e}tre am\'{e}lior\'{e} \`{a} l'aide de la voie de retour \`{a} la paire \'{e}metteur-r\'{e}cepteur  $i$, \`{a} savoir,  $\Delta_{i}(\overleftarrow{n}_{ii})=0$.
%
\'{E}tant donn\'{e} l'\'{e}v\'{e}nement  $S_{1,i}$ en \eqref{S1ifr}, le d\'{e}bit individuel $R_i$ peut \^{e}tre am\'{e}lior\'{e}, \`{a} savoir, $\Delta_{i}\Big(\overleftarrow{n}_{ii}\Big)>0$, si $\overleftarrow{n}_{ii} > \max\left(n_{ji},\left(\overrightarrow{n}_{ii}-n_{ij}\right)^+\right)$. 

 \subsubsection{Am\'{e}lioration du D\'{e}bit Individuel $R_j$ \`{a} l'Aide de la Voie de Retour dans le Lien $i$}

\'{E}tant donn\'{e} les param\`{e}tres fix\'{e}s $(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}$,  $n_{21})$, $i \in \lbrace 1, 2 \rbrace$, et $j \in \lbrace 1, 2 \rbrace\setminus\lbrace i \rbrace$, l'impl\'{e}mentation de la voie de retour \`{a} la paire \'{e}metteur-r\'{e}cepteur  $i$ augmente le d\'{e}bit individuel $R_j$, \`{a} savoir, $\Delta_j(\overleftarrow{n}_{ii})>0$ pour certaines valeurs de $\overleftarrow{n}_{ii}$.  
%
Le Th\'{e}or\`{e}me \ref{TheoremLD-IC-NOF-Th5fr} identifie les valeurs exactes de $\overleftarrow{n}_{ii}$ pour lesquelles $\Delta_j(\overleftarrow{n}_{ii})>0$.

%theorem style=margin apart,left=10mm, right=10mm
\begin{thm-fr}[, label=TheoremLD-IC-NOF-Th5fr]{Am\'{e}lioration de $R_j$ \`{a} l'Aide de la Voie de Retour dans le Lien $i$}{}
Soit $\left(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}, n_{21} \right) \in \mathds{N}^4$ un quadruplet fixe. Soit aussi $i \in \lbrace 1, 2 \rbrace$, $j \in \lbrace 1, 2 \rbrace\setminus\lbrace i \rbrace$ et $\overleftarrow{n}_{ii}^{*} \in \mathds{N}$ en \eqref{Threshold1fr}, des nombres entiers fixes.
%
Supposons que ${S_{3,i}\textrm{ est vrai}}$. Alors, pour tout $\overleftarrow{n}_{ii} \in \mathds{N}$, $\Delta_{j}(\overleftarrow{n}_{ii})=0$.
%
Supposons que ${S_{1,i}\textrm{ est vrai}}$ ou ${S_{2,i}\textrm{ est vrai}}$. Alors, si ${\overleftarrow{n}_{ii} \leqslant \overleftarrow{n}_{ii}^{*}}$, cela signifie que $\Delta_{j}(\overleftarrow{n}_{ii})=0$;  et sinon $\overleftarrow{n}_{ii} > \overleftarrow{n}_{ii}^{*}$, cela signifie que $\Delta_{j}(\overleftarrow{n}_{ii})>0$.
\end{thm-fr} 
%


Le Th\'{e}or\`{e}me \ref{TheoremLD-IC-NOF-Th5fr} indique qu'\'{e}tant donn\'{e} l'\'{e}v\'{e}nement $S_{3,i}$ en \eqref{S3ifr}, l'impl\'{e}mentation de la voie de retour \`{a} la paire \'{e}metteur-r\'{e}cepteur $i$ n'apporte aucune am\'{e}lioration au d\'{e}bit $R_j$. 
%
\'{E}tant donn\'{e} les \'{e}v\'{e}nements $S_{1,i}$ en \eqref{S1ifr} et $S_{2,i}$ en \eqref{S2ifr}, le d\'{e}bit individuel $R_j$ peut \^{e}tre am\'{e}lior\'{e}, \`{a} savoir, ${\Delta_{j}(\overleftarrow{n}_{ii})>0}$ pour tout $\overleftarrow{n}_{ii} > \overleftarrow{n}_{ii}^{*}$. 
%


\subsubsection{Am\'{e}lioration du D\'{e}bit Somme}

\'{E}tant donn\'{e} les param\`{e}tres fix\'{e}s $(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}$,  $n_{21})$, et $i \in \lbrace 1, 2 \rbrace$,  l'impl\'{e}mentation de la voie de retour \`{a} la paire \'{e}metteur-r\'{e}cepteur  $i$ augmente le d\'{e}bit somme, \`{a} savoir, $\Sigma(\overleftarrow{n}_{ii})>0$ pour certaines valeurs de $\overleftarrow{n}_{ii}$.
%
Le Th\'{e}or\`{e}me \ref{TheoremLD-IC-NOF-Th6fr} identifie les valeurs exactes de $\overleftarrow{n}_{ii}$ pour lesquelles $\Sigma(\overleftarrow{n}_{ii})>0$.


%theorem style=margin apart,left=10mm, right=10mm
\begin{thm-fr}[, label=TheoremLD-IC-NOF-Th6fr]{Am\'{e}lioration de la Somme des Capacit\'{e}s}{}
Soit $\left(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}, n_{21} \right) \in \mathds{N}^4$ un quadruplet fixe. Soit aussi $i \in \lbrace 1, 2 \rbrace$, $j \in \lbrace 1, 2 \rbrace\setminus\lbrace i \rbrace$ et $\overleftarrow{n}_{ii}^{+} \in \mathds{N}$ des nombres entiers fixes, avec
%
\begin{equation}
\overleftarrow{n}_{ii}^{+}=\left\{\begin{array}{ll}
\max\left(n_{ji},\left(\overrightarrow{n}_{ii}-n_{ij}\right)^+\right) & \text{ si } S_{4}\textrm{ est vrai}\\ 
\overrightarrow{n}_{jj}+\left(\overrightarrow{n}_{ii}-n_{ij}\right)^+ & \text{ si } S_{5}\textrm{ est vrai}  \\
\end{array}. \right.
\label{Eq:th6fr}
\end{equation}
%
Supposons que $S_{4}$ et $S_{5}$ soient faux. Alors, $\Sigma(\overleftarrow{n}_{ii})=0$ pour tout $\overleftarrow{n}_{ii} \in \mathds{N}$. 
%
Supposons que $S_{4}\textrm{ est vrai}$ ou $S_{5}\textrm{ est vrai}$. Alors, si ${\overleftarrow{n}_{ii} \leqslant \overleftarrow{n}_{ii}^{+}}$, cela signifie que $\Sigma(\overleftarrow{n}_{ii})=0$; et sinon $\overleftarrow{n}_{ii} > \overleftarrow{n}_{ii}^{+}$, cela signifie que  $\Sigma(\overleftarrow{n}_{ii})>0$.
\end{thm-fr} 
%
Le Th\'{e}or\`{e}me \ref{TheoremLD-IC-NOF-Th6fr} introduit une condition n\'{e}cessaire mais non suffisante pour l'am\'{e}lioration du d\'{e}bit somme par l'impl\'{e}mentation de la voie de retour \`{a} la paire \'{e}metteur-r\'{e}cepteur  $i$. 

\textbf{Remarque $1$ : } \emph{Une condition n\'{e}cessaire mais non suffisante pour observer  $\Sigma(\overleftarrow{n}_{ii})>0$ est de satisfaire \`{a} l'une des conditions suivantes :  
$(a)$ les deux paires \'{e}metteur-transmetteur sont en LIR (\'{E}v\'{e}nement $E_1$); ou 
$(b)$ les deux paires \'{e}metteur-transmetteur sont en HIR (\'{E}v\'{e}nement $\overline{E}_1$).  
}

Enfin, il r\'{e}sulte du Corollaire~\ref{LemmaProperSet3fr} que si $S_4$ ou $S_5$ est vrai, avec $i \in \lbrace 1,2 \rbrace$ et  $\overleftarrow{n}_{ii} > \overleftarrow{n}_{ii}^+$, outre $\Sigma (\overleftarrow{n}_{ii} ) > 0$, cela signifie aussi que $\Delta_1(\overleftarrow{n}_{ii} ) > 0$ et $\Delta_2(\overleftarrow{n}_{ii} ) > 0$. 

\subsection{Degr\'{e}s de Libert\'{e} G\'{e}n\'{e}ralis\'{e}s}

Cette section se concentre sur l'analyse du nombre de degr\'{e}s de libert\'{e} g\'{e}n\'{e}ralis\'{e}s (GDoF) du LDIC-NOF \`{a} deux utilisateurs pour \'{e}tudier le cas dans lequel la voie de retour est impl\'{e}ment\'{e}e simultan\'{e}ment dans les deux paires \'{e}metteur-r\'{e}cepteur. 
%
L'analyse n'est de plus r\'{e}alis\'{e}e que pour le cas sym\'{e}trique, \`{a} savoir, $\overrightarrow{n}  =  \overrightarrow{n}_{11} = \overrightarrow{n}_{22}$, $m  =  n_{12} = n_{21}$, et $\overleftarrow{n}  =  \overleftarrow{n}_{11} = \overleftarrow{n}_{22}$, avec $( \overrightarrow{n}, m,  \overleftarrow{n}) \in \mathds{N}^3$. 
%
Les r\'{e}sultats du th\'{e}or\`{e}me \ref{TheoremANFBLDMCapfr} permettent une analyse plus g\'{e}n\'{e}rale du nombre de GDoF, \`{a} savoir, le cas non sym\'{e}trique. Le cas sym\'{e}trique donne toutefois certains des aper\c{c}us les plus importants concernant l'agrandissement de la r\'{e}gion de capacit\'{e} lorsque la voie de retour est utilis\'{e}e dans les deux paires d'\'{e}metteurs-r\'{e}cepteurs.

\'{E}tant donn\'{e} les param\`{e}tres $\overrightarrow{n}$, $m$ et $\overleftarrow{n}$, avec $\alpha =  \frac{m}{ \overrightarrow{n}}$ et $\beta  =  \frac{ \overleftarrow{n}}{ \overrightarrow{n}}$,
%
le nombre de GDoF, not\'{e}e $D(\alpha, \beta)$, repr\'{e}sente le rapport entre la capacit\'{e} sym\'{e}trique, \`{a} savoir, $C_\mathrm{sym}( \overrightarrow{n}, m,\overleftarrow{n}) = \sup \lbrace R :  (R,R) \in \mathcal{C}(\overrightarrow{n}, \overrightarrow{n},m, m,\overleftarrow{n}, \overleftarrow{n})\rbrace$,
%
et la capacit\'{e} individuelle sans interf\'{e}rence, \`{a} savoir,  $ \overrightarrow{n}$, lorsque $( \overrightarrow{n}, m,  \overleftarrow{n}) \rightarrow (\infty, \infty, \infty)$. Le nombre de GDoF est plus pr\'{e}cis\'{e}ment :  % des rapports constants $\alpha=\frac{m}{ \overrightarrow{n}}$ et $\beta = \frac{ \overleftarrow{n}}{ \overrightarrow{n}}$
%
\begin{equation}
\label{EqGDoFfr}
D(\alpha,\beta)=\lim_{\left(\overrightarrow{n},  m,  \overleftarrow{n}\right) \rightarrow \left(\infty, \infty, \infty \right)}\frac{C_\mathrm{sym}( \overrightarrow{n}, m,  \overleftarrow{n} ) }{\overrightarrow{n} }. 
\end{equation}

Le Th\'{e}or\`{e}me \ref{TheoremGDoF-LD-IC-NOFfr} d\'{e}termine le nombre de GDoF pour le LDIC-NOF sym\'{e}trique \`{a} deux utilisateurs. \\

%theorem style=margin apart,left=10mm, right=10mm
\begin{thm-fr}[, label=TheoremGDoF-LD-IC-NOFfr]{Le Nombre de GDoF}{}
Le nombre de GDoF pour le LDIC-NOF sym\'{e}trique \`{a} deux utilisateurs avec param\`{e}tres $\alpha$ et $\beta$ est donn\'{e} par
\begin{IEEEeqnarray}{rcl}
\nonumber
D(\alpha,\beta)&=&\min\Bigg(\max(1,\alpha),\max\left(1, \beta-\left(1-\alpha\right)^+\right), \frac{1}{2}\left(\max(1,\alpha)+\left(1-\alpha\right)^+\right), \\
\label{EqLDM-GDoF2fr}
& & \max\left(\left(1-\alpha\right)^+,\alpha,1-\left(\max(1,\alpha)-\beta\right)^+\right) \Bigg).
\end{IEEEeqnarray}
\end{thm-fr} 

\begin{figure*}[t!]
 \centerline{\epsfig{figure=Figures/LDM-GDoF-FR.pdf,width=1.0 \textwidth}}
  \caption{Degr\'{e}s de libert\'{e} g\'{e}n\'{e}ralis\'{e}s  comme fonction des param\`{e}tres $\alpha$ et $\beta$, avec $0 \leqslant \alpha \leqslant 3$ et $\beta \in \lbrace{\frac{3}{5}, \frac{4}{5}, \frac{6}{5}\rbrace}$, du LDIC-NOF sym\'{e}trique \`{a} deux utilisateurs. Le point sans voie de retour est obtenu \`{a} partir de \cite{Etkin-TIT-2008} et le point avec voie de retour parfaite est obtenu \`{a} partir de \cite{Suh-TIT-2011}.}
  \label{FigLDM-GDoFfr}
\end{figure*}

Le r\'{e}sultat du Th\'{e}or\`{e}me \ref{TheoremGDoF-LD-IC-NOFfr} peut \'{e}galement \^{e}tre obtenu \`{a} partir du Th\'{e}or\`{e}me $1$ en \cite{SyQuoc-TIT-2015}.
%
Les propri\'{e}t\'{e}s suivantes sont une cons\'{e}quence directe du Th\'{e}or\`{e}me \ref{TheoremGDoF-LD-IC-NOFfr}.

\begin{corollary-fr} 
Le nombre de  GDoF pour le LDIC-NOF sym\'{e}trique \`{a} deux utilisateurs avec param\`{e}tres $\alpha$ et $\beta$ r\'{e}pond aux propri\'{e}t\'{e}s suivantes : 
%
\begin{subequations}
\label{EqGDoFPropfr}
\begin{IEEEeqnarray}{lll}
\label{EqGDoFProp1fr}
& \forall  \alpha \in \left[0,\frac{2}{3} \right]   \textrm{ et } \beta \leqslant 1, &  \quad  \max\left(\frac{1}{2}, \beta \right) \leqslant  D(\alpha,\beta) \leqslant 1, \\
\label{EqGDoFProp1bfr}
& \forall  \alpha \in \left[0,\frac{2}{3} \right] \textrm{ et } \beta > 1,  & \quad D(\alpha,\beta) = 1 - \frac{\alpha}{2}, \\
\label{EqGDoFProp2fr}
&\forall  \alpha \in \left(\frac{2}{3}, 2 \right] \textrm{ et } \beta \in [0, \infty),  & \quad D(\alpha,0)  =  D(\alpha,\beta)  =  D(\alpha, \max(1,\alpha)),  
\end{IEEEeqnarray}
%
\begin{IEEEeqnarray}{lll}
\label{EqGDoFProp3fr}
& \forall  \alpha \in \left(2, \infty \right) \textrm{ et } \beta \geqslant 1,  & \quad 1 \leqslant  D(\alpha,\beta)  \leqslant  \min\left(\frac{\alpha}{2}, \beta \right),\\
\label{EqGDoFProp3bfr}
& \forall  \alpha \in \left(2, \infty \right) \textrm{ et } \beta < 1,  & \quad D(\alpha,\beta)=1.
\end{IEEEeqnarray}
\end{subequations}
\end{corollary-fr} 

Les propri\'{e}t\'{e}s \eqref{EqGDoFProp1fr} et \eqref{EqGDoFProp1bfr} mettent en \'{e}vidence le fait que l'existence de voies de retour dans le LDIC-NOF sym\'{e}trique \`{a} deux utilisateurs dans le VWIR et WIR n'ont aucun impact sur le nombre de GDoF si $\beta \leqslant \frac{1}{2}$, et le nombre de GDoF est \'{e}gal au cas avec une voie de retour parfaite si $\beta > 1$.
%
La propri\'{e}t\'{e} \eqref{EqGDoFProp2fr} souligne que dans le LDIC-NOF sym\'{e}trique \`{a} deux utilisateurs en MIR et SIR, le nombre de GDoF est identique dans les deux cas extr\^{e}mes :  sans voie de retour ($\beta = 0$) et avec voie de retour parfaite $\big(\beta = \max(1, \alpha)\big)$.  
%
Il r\'{e}sulte enfin qu'\`{a} partir de \eqref{EqGDoFProp3fr} et \eqref{EqGDoFProp3bfr}, pour observer une am\'{e}lioration du nombre de GDoF du LDIC-NOF sym\'{e}trique \`{a} deux utilisateurs en VSIR, la condition suivante doit \^{e}tre satisfaite :  $\beta > 1$.  Autrement dit, la capacit\'{e} dans les voies de retour doit \^{e}tre sup\'{e}rieur a la capacit\'{e} dans les liens directs. 


La Figure \ref{FigLDM-GDoFfr} montre le nombre de GDoF pour le LDIC-NOF sym\'{e}trique \`{a} deux utilisateurs pour le cas dans lequel $0 \leqslant \alpha \leqslant 3$ et $\beta \in \lbrace{\frac{3}{5}, \frac{4}{5}, \frac{6}{5}\rbrace}$. 

\section{Principaux R\'{e}sultats du Canal Gaussien \`{a} Interf\'{e}rence Centralis\'{e}}\label{ChGICNOFfr} 

Cette section pr\'{e}sente les principaux r\'{e}sultats sur le GIC-NOF centralis\'{e} d\'{e}crit en Section \ref{SectCGICNOFfr}. 
%
Ceux-ci incluent une r\'{e}gion atteignable (Th\'{e}or\`{e}me~\ref{TheoremA-G-IC-NOFfr})  et une r\'{e}gion d'impossibilit\'{e} (Th\'{e}or\`{e}me~\ref{TheoremC-G-IC-NOFfr}), not\'{e}e $\agicnof$ et $\cgicnof$ respectivement, pour le GIC-NOF \`{a} deux utilisateurs et param\`{e}tres fix\'{e}s $\overrightarrow{\SNR}_{1}$, $\overrightarrow{\SNR}_{2}$, $\INR_{12}$, $\INR_{21}$, $\overleftarrow{\SNR}_{1}$, et $\overleftarrow{\SNR}_{2}$.
%
En g\'{e}n\'{e}ral, la r\'{e}gion de capacit\'{e} d'un canal multi-utilisateurs donn\'{e} est approxim\'{e} avec un \'{e}cart constant conform\'{e}ment \`{a} la D\'{e}finition \ref{DefGapfr}.

\begin{definition-fr}[Approximation \`{a} $\xi$ unit\'{e}s pr\`{e}s]\label{DefGapfr}\emph{ \newline Un ensemble ferm\'{e} et convexe $\mathcal{T}\subset\mathds{R}_{+}^{m}$ est obtenu par approximation \`{a} $\xi$ unit\'{e}s pr\`{e}s par les ensembles $\underline{\mathcal{T}}$ et $\overline{\mathcal{T}}$ si  $\underline{\mathcal{T}} \subseteq \mathcal{T} \subseteq \overline{\mathcal{T}}$ et pour tout ${\vec{t}=(t_1, t_2, \ldots, t_m)\in \overline{\mathcal{T}}}$, $\Big(\left(t_1-\xi\right)^+$, $\left(t_2-\xi\right)^+$, $\ldots$, $\left(t_m-\xi\right)^+\Big) \in \underline{\mathcal{T}}$.}
\end{definition-fr}


Notons $\Cgicnof$ la r\'{e}gion de capacit\'{e} du GIC-NOF \`{a} deux utilisateurs. La r\'{e}gion atteignable $\agicnof$ et la r\'{e}gion d'impossibilit\'{e} $\cgicnof$ correspondent approximativement \`{a} la r\'{e}gion de capacit\'{e} $\Cgicnof$ \`{a} $4.4$ bits pr\`{e}s. (Th\'{e}or\`{e}me~\ref{TheoremGAP-G-IC-NOFfr}).

\subsection{Une R\'{e}gion Atteignable}
%
La description de la r\'{e}gion atteignable $\agicnof$ est pr\'{e}sent\'{e}e \`{a} l'aide des constantes $a_{1,i}$; des fonctions $a_{2,i} : [0,1] \rightarrow \mathds{R}_{+}$,  $a_{l,i} : [0,1]^2\rightarrow \mathds{R}_{+}$, avec $l \in \lbrace 3, \ldots, 6 \rbrace$; et $a_{7,i} : [0,1]^3\rightarrow \mathds{R}_{+}$, qui sont d\'{e}finis comme suit, pour tout $i \in \lbrace 1, 2 \rbrace$, avec $j \in \lbrace 1, 2 \rbrace \setminus \lbrace i \rbrace$ : 

\begin{subequations}
\label{Eq-afr}
\begin{IEEEeqnarray}{rcl}
\label{Eq-a1fr}
a_{1,i}  &=&  \frac{1}{2}\log \left(2+\frac{\overrightarrow{\SNR_{i}}}{\INR_{ji}}\right)-\frac{1}{2}, \\
\label{Eq-a2fr}
a_{2,i}(\rho) &=& \frac{1}{2}\log \Big(b_{1,i}(\rho)+1\Big)-\frac{1}{2}, 
\end{IEEEeqnarray}
%%%
\begin{IEEEeqnarray}{rcl}
\label{Eq-a3fr}
a_{3,i}(\rho,\mu) &=&   \frac{1}{2}\log \left( \frac{ \overleftarrow{\SNR}_i  \Big(b_{2,i}(\rho)+2\Big)+b_{1,i}(1)+1}{\overleftarrow{\SNR}_i\Big(  \left(1-\mu\right)  b_{2,i}( \rho )+2\Big)+ b_{1,i}( 1  ) + 1}  \right), \\
\label{Eq-a4fr}
a_{4,i}(\rho,\mu) &=& \frac{1}{2}\log \bigg(\Big(1-\mu\Big)b_{2,i}(\rho)+2 \bigg)-\frac{1}{2},  \\
\label{Eq-a5fr}
a_{5,i}(\rho,\mu) &=& \frac{1}{2}\log \left(2+\frac{\overrightarrow{\SNR}_{i}}{\INR_{ji}}+\Big(1-\mu\Big)b_{2,i}(\rho)\right)-\frac{1}{2}, \\
\label{Eq-a6fr}
a_{6,i}(\rho,\mu) &=& \frac{1}{2}\log \left(\frac{\overrightarrow{\SNR}_{i}}{\INR_{ji}}\bigg(\Big(1-\mu\Big)b_{2,j}(\rho)+1\bigg)+2\right)-\frac{1}{2}, \textrm { et } \\
\label{Eq-a7fr}
a_{7,i}(\rho,\mu_1,\mu_2) &=& \frac{1}{2}\log \Bigg(\frac{\overrightarrow{\SNR}_{i}}{\INR_{ji}}\bigg(\Big(1-\mu_i\Big)b_{2,j}(\rho)+1\bigg) +\Big(1-\mu_j\Big)b_{2,i}(\rho)+2\Bigg)-\frac{1}{2},
\end{IEEEeqnarray}
\end{subequations}
%
o\`{u} les fonctions $b_{l,i} : [0,1]\rightarrow \mathds{R}_{+}$, avec $(l,i) \in \lbrace1, 2 \rbrace^2$ sont d\'{e}finies comme suit :  
\begin{subequations}
\label{Eqfntsfr}
\begin{IEEEeqnarray}{rcl}
\label{Eqb1ifr}
b_{1,i}(\rho)&=&\overrightarrow{\SNR}_{i}+2\rho\sqrt{\overrightarrow{\SNR}_{i}\INR_{ij}}+\INR_{ij} \textrm{ et } \\
\label{Eqb5ifr}
b_{2,i}(\rho)&=&\Big(1-\rho\Big)\INR_{ij}-1,
\end{IEEEeqnarray}
\end{subequations}
%
avec $j \in \lbrace 1, 2 \rbrace \setminus \lbrace i \rbrace$.



Notons que les fonctions dans \eqref{Eq-afr} et \eqref{Eqfntsfr} d\'{e}pendent de $\overrightarrow{\SNR}_{1}$, $\overrightarrow{\SNR}_{2}$, $\INR_{12}$, $\INR_{21}$, $\overleftarrow{\SNR}_{1}$, et $\overleftarrow{\SNR}_{2}$. Toutefois, comme ces param\`{e}tres sont fix\'{e}s dans cette analyse, cette d\'{e}pendance n'est pas mise en \'{e}vidence dans la d\'{e}finition de ces fonctions. Enfin, en utilisant cette notation, le Th\'{e}or\`{e}me~\ref{TheoremA-G-IC-NOFfr} est pr\'{e}sent\'{e} comme suit : 

%theorem style=margin apart,left=10mm, right=10mm
\begin{thm-fr}[, label=TheoremA-G-IC-NOFfr]{R\'{e}gion Atteignable}{} % of the Two-User Gaussian Interference Channel with Noisy Channel-Output Feedback
La r\'{e}gion de capacit\'{e} $\Cgicnof$ contient la r\'{e}gion $\agicnof$ donn\'{e}e par la fermeture de l'ensemble de toutes les paires possibles de d\'{e}bit atteignables $(R_1,R_2)\in\mathds{R}_{+}^2$ satisfaisant :
%
\begin{subequations}
\label{EqRa-G-IC-NOFfr}
\begin{IEEEeqnarray}{rcl}
\nonumber
R_{1}  & \leqslant & \min\Big(a_{2,1}(\rho),a_{6,1}(\rho,\mu_1)+a_{3,2}(\rho,\mu_1), a_{1,1}+a_{3,2}(\rho,\mu_1)+a_{4,2}(\rho,\mu_1)\Big),  \\ 
\label{EqR1a-G-IC-NOFfr}\\
\nonumber
R_{2}   & \leqslant & \min\Big(a_{2,2}(\rho),a_{3,1}(\rho,\mu_2)+a_{6,2}(\rho,\mu_2), a_{3,1}(\rho,\mu_2)+a_{4,1}(\rho,\mu_2)+a_{1,2}\Big),   \\
\label{EqR2a-G-IC-NOFfr} \\
%\end{IEEEeqnarray}
%%%
%\begin{IEEEeqnarray}{rcl}
\nonumber
R_{1}+R_{2}  & \leqslant & \min\Big(a_{2,1}(\rho)+a_{1,2}, a_{1,1}+a_{2,2}(\rho), \\
\nonumber
& & a_{3,1}(\rho,\mu_2)+a_{1,1}+a_{3,2}(\rho,\mu_1)+a_{7,2}(\rho,\mu_1,\mu_2), \\
\nonumber
& & a_{3,1}(\rho,\mu_2)  +  a_{5,1}(\rho,\mu_2)+a_{3,2}(\rho,\mu_1)+a_{5,2}(\rho,\mu_1), \\
\label{EqR1+R2a-G-IC-NOFfr}
& & a_{3,1}(\rho,\mu_2)+a_{7,1}(\rho,\mu_1,\mu_2)+a_{3,2}(\rho,\mu_1)+a_{1,2}\Big), \\
%\end{IEEEeqnarray}
%%%
%\begin{IEEEeqnarray}{rcl}
\nonumber
2R_{1}+R_{2}  & \leqslant & \min\Big(a_{2,1}(\rho)+a_{1,1}+a_{3,2}(\rho,\mu_1)+a_{7,2}(\rho,\mu_1,\mu_2),  \\
\nonumber
& &  a_{3,1}(\rho,\mu_2)+a_{1,1}+a_{7,1}(\rho,\mu_1,\mu_2)+2a_{3,2}(\rho,\mu_1)+a_{5,2}(\rho,\mu_1), \\
\label{Eq2R1+R2a-G-IC-NOFfr}
& & a_{2,1}(\rho)+a_{1,1}+a_{3,2}(\rho,\mu_1)+a_{5,2}(\rho,\mu_1)\Big), 
\end{IEEEeqnarray}
%%
\begin{IEEEeqnarray}{rcl}
\nonumber
R_{1}+2R_{2}  & \leqslant & \min\Big(a_{3,1}(\rho,\mu_2)+a_{5,1}(\rho,\mu_2)+a_{2,2}(\rho)+a_{1,2}, \\
\nonumber
& & a_{3,1}(\rho,\mu_2)+a_{7,1}(\rho,\mu_1,\mu_2)+a_{2,2}(\rho)+a_{1,2}, \\
\nonumber
& &  2a_{3,1}(\rho,\mu_2)+a_{5,1}(\rho,\mu_2)+a_{3,2}(\rho,\mu_1)+a_{1,2}+a_{7,2}(\rho,\mu_1,\mu_2)\Big), \\
\label{EqR1+2R2a-G-IC-NOFfr}
\end{IEEEeqnarray}
\end{subequations}
%
avec $\left(\rho, \mu_1, \mu_2\right) \in \left[0,\left(1-\max\left(\frac{1}{\INR_{12}},\frac{1}{\INR_{21}}\right) \right)^+\right]\times[0,1]\times[0,1]$.
%}
%\end{theorem}
\end{thm-fr}

\subsection{Une R\'{e}gion d'Impossibilit\'{e}}

La description de la r\'{e}gion d'impossibilit\'{e} $\cgicnof$ est d\'{e}termin\'{e}e par deux \'{e}v\'{e}nements indiqu\'{e}s par $S_{l_{1},1}$ et $S_{l_{2},2}$, o\`{u} $(l_{1},l_{2}) \in \lbrace 1, \ldots, 5 \rbrace^2$. Les \'{e}v\'{e}nements sont d\'{e}finis comme suit pour tout $i \in \{1,2\}$ : 
 %
 \begin{subequations}
\label{EqSifr}
\begin{IEEEeqnarray}{rcl}
\label{EqS1ifr}  
 S_{1,i}& : \quad & \overrightarrow{\SNR}_{j} < \min\left(\INR_{ij},\INR_{ji}\right), \\ 
\label{EqS2ifr}
 S_{2,i}& :  \quad & \INR_{ji} \leqslant  \overrightarrow{\SNR}_{j} < \INR_{ij},\\
 \label{EqS3ifr}
 S_{3,i}& :  \quad & \INR_{ij} \leqslant \overrightarrow{\SNR}_{j} < \INR_{ji}, \\
 \label{EqS4ifr}
 S_{4,i}& :  \quad & \max\left(\INR_{ij}, \INR_{ji}\right) \leqslant \overrightarrow{\SNR}_{j} < \INR_{ij}\INR_{ji}, \qquad \\
 \label{EqS5ifr}
 S_{5,i}& :  \quad & \overrightarrow{\SNR}_{j} \geqslant  \INR_{ij}\INR_{ji}.
\end{IEEEeqnarray}
\end{subequations}
%
Notons que pour tout $i \in \lbrace 1, 2 \rbrace$, les \'{e}v\'{e}nements $S_{1,i}$, $S_{2,i} $, $S_{3,i}$, $S_{4,i}$, et $S_{5,i}$ sont mutuellement exclusifs. Cette observation indique que pour tout quadruplet $(\overrightarrow{\SNR}_{1}, \overrightarrow{\SNR}_{2}, \INR_{12}, \INR_{21})$, il existe toujours une unique paire d'\'{e}v\'{e}nements  $(S_{l_{1},1}, S_{l_{2},2})$, avec $(l_{1},l_{2}) \in \lbrace 1, \ldots, 5 \rbrace^2$, qui identifie un sc\'{e}nario unique. Notons \'{e}galement que les paires d'\'{e}v\'{e}nements $(S_{2,1}, S_{2,2})$ et $(S_{3,1}, S_{3,2})$ ne sont pas r\'{e}alisables. Compte tenu de ceci, vingt-trois sc\'{e}narios diff\'{e}rents peuvent \^{e}tre identifi\'{e}s \`{a} l'aide des \'{e}v\'{e}nements en \eqref{EqSifr}.
%
Une fois le sc\'{e}nario exact identifi\'{e}, la r\'{e}gion d'impossibilit\'{e} est d\'{e}crite \`{a} l'aide des fonctions $\kappa_{l,i} :  [0,1]\rightarrow \mathds{R}_{+}$, avec $l \in \lbrace 1, \ldots, 3\rbrace$; $\kappa_{l} :  [0,1]\rightarrow \mathds{R}_{+}$, avec $l \in \lbrace 4, 5 \rbrace$; $\kappa_{6,l} :  [0,1]\rightarrow \mathds{R}_{+}$, avec $l \in \lbrace 1, \ldots, 4\rbrace$; et $\kappa_{7,i,l} : [0,1]\rightarrow \mathds{R}_{+}$, avec $l \in \lbrace 1, 2 \rbrace$. Ces fonctions sont d\'{e}finies comme suit, pour tout $i \in \lbrace 1, 2 \rbrace$, avec $j \in \lbrace 1, 2 \rbrace\setminus\lbrace i \rbrace$ : 
%
%
\begin{subequations}
\label{Eqconvfr}
\begin{IEEEeqnarray}{rcl}
\label{Eqconv1fr}
\kappa_{1,i}(\rho)  & = & \frac{1}{2}\log \Big(b_{1,i}(\rho)+1\Big), \\
\label{Eqconv2fr}
\kappa_{2,i}(\rho)  & = & \frac{1}{2}\log \Big(1+b_{5,j}(\rho)\Big) \!+\! \frac{1}{2}\log \Bigg(1\!+\! \frac{b_{4,i}(\rho)}{1+b_{5,j}(\rho)}\Bigg),   \\
%\end{IEEEeqnarray}
%%%
%\begin{IEEEeqnarray}{rcl}
\label{Eqconv3fr}
\kappa_{3,i}(\rho)  & = & \frac{1}{2} \! \log \! \left(\frac{\bigg(b_{4,i}(\rho)+b_{5,j}(\rho)+1\bigg)\overleftarrow{\SNR}_j}{\bigg(b_{1,j}(1) \! + \! 1\bigg)\bigg(b_{4,i}(\rho) \! + 1 \! \bigg)} \! + \! 1 \! \right) +\frac{1}{2}\log\Big(b_{4,i}(\rho)+1\Big), \\
\label{Eqconv4fr}
\kappa_{4}(\rho)  & = & \frac{1}{2}\log \! \Bigg(1+\frac{b_{4,1}(\rho)}{1+b_{5,2}(\rho)}\Bigg) \! + \! \frac{1}{2}\log \! \Big(b_{1,2}(\rho)+1\Big), 
\end{IEEEeqnarray}
%%%
\begin{IEEEeqnarray}{rcl}
\label{Eqconv5fr}
\kappa_{5}(\rho)  & = & \frac{1}{2}\log \Bigg(1 \! + \! \frac{b_{4,2}(\rho)}{1 \!+ \! b_{5,1}(\rho)}\Bigg) \! + \! \frac{1}{2}\log \Big(b_{1,1}(\rho) \! + \! 1\Big), \\
%\end{IEEEeqnarray}
%%%
%\begin{IEEEeqnarray}{rcl}
\label{Eqk6fr} 
\kappa_{6}(\rho) &=& \begin{cases} \kappa_{6,1}(\rho) & \textrm{si } (S_{1,2} \lor S_{2,2} \lor S_{5,2} ) \land (S_{1,1} \lor S_{2,1} \lor S_{5,1} )\\
                                                \kappa_{6,2} (\rho) & \textrm{si }(S_{1,2} \lor S_{2,2} \lor S_{5,2} ) \land (S_{3,1} \lor S_{4,1} )\\
                                                \kappa_{6,3}(\rho) & \textrm{si } (S_{3,2} \lor S_{4,2}) \land (S_{1,1} \lor S_{2,1} \lor S_{5,1})\\
                                                \kappa_{6,4}(\rho) & \textrm{si } (S_{3,2} \lor S_{4,2} ) \land ( S_{3,1} \lor S_{4,1})
                                           \end{cases}, \qquad \qquad  \\
%\end{IEEEeqnarray}
%%
%\begin{IEEEeqnarray}{rcl}
\label{Eqk77fr}
\kappa_{7,i}(\rho) &=& \begin{cases} \kappa_{7,i,1}(\rho) & \textrm{si } (S_{1,i} \lor S_{2,i} \lor S_{5,i})\\
                                                  \kappa_{7,i,2}(\rho) & \textrm{si } (S_{3,i} \lor S_{4,i})
                                                \end{cases}, \qquad\qquad\qquad\qquad
\end{IEEEeqnarray}
\end{subequations}
%
%
o\`{u}
%
\begin{subequations}
\label{Eqconv6fr}
\begin{IEEEeqnarray}{rcl}
\label{Eqconv61fr}
\kappa_{6,1}&(&\rho) \! = \! \frac{1}{2} \! \log \! \Big(b_{1,1}(\rho) \! + \! b_{5,1}(\rho)\INR_{21}\Big) \! - \! \frac{1}{2}\log\Big(1 \! + \! \INR_{12}\Big) +\frac{1}{2}\log\left(1+\frac{b_{5,2}(\rho)\overleftarrow{\SNR}_2}{b_{1,2}(1)+1}\right)\\
\nonumber
& & +\frac{1}{2}\log\Big(b_{1,2}(\rho)+b_{5,1}(\rho)\INR_{21}\Big) -\frac{1}{2}\log\Big(1 \! + \! \INR_{21}\Big) \! + \! \frac{1}{2}\log\left(\! 1 \! + \! \frac{b_{5,1}(\rho)\overleftarrow{\SNR}_1}{b_{1,1}(1)+1}\right)+\log(2 \pi e), \\
\label{Eqconv62fr}
\kappa_{6,2}&(&\rho) \! = \!   \frac{1}{2}\log\left(b_{6,2}(\rho)+\frac{b_{5,1}(\rho)\INR_{21}}{\overrightarrow{\SNR}_2}\Big(\overrightarrow{\SNR}_2+b_{3,2}\Big)\right) - \frac{1}{2}\log\Big(1 \!+ \! \INR_{12}\Big)  \\
\nonumber
& & +\frac{1}{2}\log\left(1+\frac{b_{5,1}(\rho)\overleftarrow{\SNR}_1}{b_{1,1}(1)+1}\right) + \frac{1}{2} \! \log\Big(b_{1,1}(\rho) \! + \! b_{5,1}(\rho)\INR_{21}\Big) \! -\frac{1}{2}\log\Big(1+\INR_{21}\Big)\\
\nonumber
& & +\frac{1}{2}\log\Bigg(1+\frac{b_{5,2}(\rho)}{\overrightarrow{\SNR}_2}\left(\INR_{12}+\frac{b_{3,2} \overleftarrow{\SNR}_2}{b_{1,2}(1)+1}\right)\Bigg)-\frac{1}{2}\log\left(1+\frac{b_{5,1}(\rho)\INR_{21}}{\overrightarrow{\SNR}_2}\right)+\log(2 \pi e), \\
\label{Eqconv63fr}
\kappa_{6,3}&(&\rho) \! = \! \frac{1}{2}\log\Bigg(b_{6,1}(\rho)+\frac{b_{5,1}(\rho)\INR_{21}}{\overrightarrow{\SNR}_1}\Big(\overrightarrow{\SNR}_1+b_{3,1}\Big)\Bigg)-\frac{1}{2}\log\Big(1+\INR_{12}\Big) \\ 
\nonumber
& & +\frac{1}{2}\log\left(1+\frac{b_{5,2}(\rho)\overleftarrow{\SNR}_2}{b_{1,2}(1)+1}\right)+\frac{1}{2}\log\Big(b_{1,2}(\rho) \! + \! b_{5,1}(\rho)\INR_{21}\Big) \! - \! \frac{1}{2}\log\Big(1 \! + \! \INR_{21}\Big)\\
\nonumber
& & +\frac{1}{2}\log\Bigg(1+\frac{b_{5,1}(\rho)}{\overrightarrow{\SNR}_1}\left(\INR_{21}+\frac{b_{3,1} \overleftarrow{\SNR}_1}{b_{1,1}(1)+1}\right)\Bigg)-\frac{1}{2}\log\left(1+\frac{b_{5,1}(\rho)\INR_{21}}{\overrightarrow{\SNR}_1}\right) +\log(2 \pi e), \\
%\end{IEEEeqnarray}
%%%%%%
%\begin{IEEEeqnarray}{rcl}
\label{Eqconv64fr}
\kappa_{6,4}&(&\rho)=\frac{1}{2}\log\left(b_{6,1}(\rho)+\frac{b_{5,1}(\rho)\INR_{21}}{\overrightarrow{\SNR}_1}\Big(\overrightarrow{\SNR}_1+b_{3,1}\Big)\right)-\frac{1}{2}\log\Big(1+\INR_{12}\Big)\\
\nonumber
& & +\frac{1}{2}\log\left(1+\frac{b_{5,2}(\rho)}{\overrightarrow{\SNR}_2}\left(\INR_{12}+\frac{b_{3,2}\overleftarrow{\SNR}_2}{b_{1,2}(1)+1}\right)\right)-\frac{1}{2}\log\left(1+\frac{b_{5,1}(\rho)\INR_{21}}{\overrightarrow{\SNR}_2}\right) \\
\nonumber
& & -\frac{1}{2}\log\left(1+\frac{b_{5,1}(\rho)\INR_{21}}{\overrightarrow{\SNR}_1}\right)+\frac{1}{2}\log\left(b_{6,2}(\rho)+\frac{b_{5,1}(\rho)\INR_{21}}{\overrightarrow{\SNR}_2}\Big(\overrightarrow{\SNR}_2+b_{3,2}\Big)\right)\\
\nonumber
& & -\frac{1}{2}\log\Big(1+\INR_{21}\Big)+\frac{1}{2}\log\Bigg(1+\frac{b_{5,1}(\rho)}{\overrightarrow{\SNR}_1}\left(\INR_{21}+\frac{b_{3,1} \overleftarrow{\SNR}_1}{b_{1,1}(1)+1}\right)\Bigg)+\log(2 \pi e), 
\end{IEEEeqnarray}
\end{subequations}
%
et
%
\begin{subequations}
\label{Eqconv7ifr}
\begin{IEEEeqnarray}{rcl}
\label{Eqconv7i1fr}
\kappa_{7,i,1}&(&\rho) =\frac{1}{2}\log\Big(b_{1,i}(\rho)+1\Big)-\frac{1}{2}\log\Big(1+\INR_{ij}\Big) +\frac{1}{2}\log\left(1+\frac{b_{5,j}(\rho)\overleftarrow{\SNR}_j}{b_{1,j}(1)+1}\right)\\
\nonumber
& &  +  \frac{1}{2}\log\Big(b_{1,j}(\rho)+b_{5,i}(\rho)\INR_{ji}\Big) \! + \! \frac{1}{2}\log\Big(1 \! + \! b_{4,i}(\rho) \!+ \! b_{5,j}(\rho) \Big) \! - \! \frac{1}{2}\log\Big(1 \! + \! b_{5,j}(\rho)\Big) \! \\
\nonumber
& & +  2\log(2 \pi e), \\
%\end{IEEEeqnarray}
%%%%%
%\begin{IEEEeqnarray}{rcl}
\label{Eqconv7i2fr}
\kappa_{7,i,2}&(&\rho) = \frac{1}{2}\log\Big(b_{1,i}(\rho)+1\Big)-\frac{1}{2}\log\Big(1+\INR_{ij}\Big)-\frac{1}{2}\log\Big(1+b_{5,j}(\rho)\Big) \\
\nonumber
& & +\frac{1}{2}\log\Big(1+b_{4,i}(\rho)+b_{5,j}(\rho) \Big)+\frac{1}{2}\log\Bigg(1+\Big(1-\rho^2\Big)\frac{\INR_{ji}}{\overrightarrow{\SNR}_j}\Bigg(\INR_{ij}+\frac{b_{3,j}\overleftarrow{\SNR}_j}{b_{1,j}(1)+1}\Bigg)\Bigg)\\
\nonumber
& & -\frac{1}{2}\log\left(1+\frac{b_{5,i}(\rho)\INR_{ji}}{\overrightarrow{\SNR}_j}\right)+\frac{1}{2}\!\log\!\left(\!b_{6,j}(\rho)\!+\!\frac{b_{5,i}(\rho)\INR_{ji}}{\overrightarrow{\SNR}_j}\Big(\overrightarrow{\SNR}_j+b_{3,j}\Big)\right)+2\log(2 \pi e), \quad
\end{IEEEeqnarray}
\end{subequations}
%
o\`{u}, les fonctions $b_{l,i}$, avec $(l,i) \in \lbrace1, 2 \rbrace^2$ sont d\'{e}finies en \eqref{Eqfntsfr}; les param\`{e}tres $b_{3,i}$ sont des constantes; et les fonctions $b_{l,i} : [0,1]\rightarrow \mathds{R}_{+}$, avec $(l,i) \in \lbrace 4, 5, 6 \rbrace\times\lbrace1, 2 \rbrace$ sont d\'{e}finies comme suit, avec $j \in \lbrace 1, 2 \rbrace \setminus \lbrace i \rbrace$ : 
%
\begin{subequations}
\label{Eqfnts2fr}
\begin{IEEEeqnarray}{rcl}
\label{Eqb2ifr}
b_{3,i}&=&\overrightarrow{\SNR}_i-2\sqrt{\overrightarrow{\SNR}_i\INR_{ji}}+\INR_{ji}, \\
\label{Eqb3ifr}
b_{4,i}(\rho)&=&\Big(1-\rho^2\Big)\overrightarrow{\SNR}_{i}, \\
\label{Eqb4ifr}
b_{5,i}(\rho)&=&\Big(1-\rho^2\Big)\INR_{ij},\\
\label{Eqb6ifr}
b_{6,i}(\rho)&=&\overrightarrow{\SNR}_i \! + \! \INR_{ij} \!+ \! 2\rho\sqrt{\INR_{ij}}\left(\sqrt{\overrightarrow{\SNR}_i}-\sqrt{\INR_{ji}}\right) \! \\
\nonumber
& & + \frac{\INR_{ij}\sqrt{\INR_{ji}}}{\overrightarrow{\SNR}_i} \left(\sqrt{\INR_{ji}}-2\sqrt{\overrightarrow{\SNR}_i}\right).
\end{IEEEeqnarray}
\end{subequations}


Notons que les fonctions en \eqref{Eqconvfr}, \eqref{Eqconv6fr}, \eqref{Eqconv7ifr}, et \eqref{Eqfnts2fr} d\'{e}pendent de $\overrightarrow{\SNR}_{1}$, $\overrightarrow{\SNR}_{2}$, $\INR_{12}$, $\INR_{21}$, $\overleftarrow{\SNR}_{1}$, et $\overleftarrow{\SNR}_{2}$. Toutefois, comme ces param\`{e}tres sont fix\'{e}s dans cette analyse, cette d\'{e}pendance n'est pas mise en \'{e}vidence dans la d\'{e}finition de ces fonctions. 
%
Enfin, \`{a} l'aide de cette notation, le Th\'{e}or\`{e}me~\ref{TheoremC-G-IC-NOFfr} est pr\'{e}sent\'{e} comme suit.
%
%theorem style=margin apart,left=10mm, right=10mm
\begin{thm-fr}[, label=TheoremC-G-IC-NOFfr]{R\'{e}gion d'Impossibilit\'{e}}{} 
La r\'{e}gion de capacit\'{e} $\Cgicnof$ est contenue dans la r\'{e}gion $\cgicnof$ donn\'{e}e par la fermeture de l'ensemble de paires de  $(R_1,R_2)\in\mathds{R}_{+}^2$ qui pour tout $i \in \lbrace 1, 2 \rbrace$, avec $j\in\lbrace 1, 2 \rbrace\setminus\lbrace i \rbrace$ d\'{e}finies : 
%
\begin{subequations}\label{EqRic-G-IC-NOFfr}
\begin{IEEEeqnarray}{rcl}
\label{EqRic-12-G-IC-NOFfr}
R_{i}  & \leqslant & \min\left(\kappa_{1,i}(\rho), \kappa_{2,i}(\rho)\right), \\ 
\label{EqRic-3-G-IC-NOFfr}
R_{i}  & \leqslant & \kappa_{3,i}(\rho), \\
\label{EqR1+R2c-12-G-IC-NOFfr}
R_{1}+R_{2}  & \leqslant & \min\left(\kappa_{4}(\rho), \kappa_{5}(\rho)\right),\\
\label{EqR1+R2c-3g-G-IC-NOFfr}
R_{1}+R_{2}  & \leqslant &\kappa_{6}(\rho),\\
\label{Eq2Ri+Rjc-g-G-IC-NOFfr}
2R_i+R_j&\leqslant&  \kappa_{7,i}(\rho),
\end{IEEEeqnarray}
\end{subequations}
avec $\rho \in [0,1]$.
%}
\end{thm-fr} 
%

\subsection{\'{E}cart entre la R\'{e}gion Atteignable et la R\'{e}gion d'Impossibilit\'{e}}\label{SectGAPfr}


Le Th\'{e}or\`{e}me~~\ref{TheoremGAP-G-IC-NOFfr} d\'{e}crit l'\'{e}cart entre la r\'{e}gion atteignable $\agicnof$ et la r\'{e}gion d'impossibilit\'{e} $\cgicnof$ (D\'{e}finition \ref{DefGapfr}).

%theorem style=margin apart,left=10mm, right=10mm
\begin{thm-fr}[, label=TheoremGAP-G-IC-NOFfr]{\'{E}cart}{}
La r\'{e}gion de capacit\'{e} du GIC-NOF \`{a} deux utilisateurs est approxim\'{e}e \`{a} $4.4$ bits pr\`{e}s par la r\'{e}gion atteignable $\agicnof$ et la r\'{e}gion d'impossibilit\'{e} $\cgicnof$.
\end{thm-fr} 

\subsection{Cas o\`{u} la Voie de Retour Agrandit la R\'{e}gion de Capacit\'{e}}\label{SectFeedbackGICfr}


Cette section examine l'application des r\'{e}sultats obtenus \`{a} la Section \ref{SectEnlargeCfr} dans le GIC-NOF \`{a} deux utilisateurs. 
%
En Section \ref{ChapterConnectionsGLDMfr}, ont \'{e}t\'{e} pr\'{e}sent\'{e}es les connexions entre le LDIC-NOF \`{a} deux utilisateurs et le
GIC-NOF \`{a} deux utilisateurs. \`{A} l'aide de ces connexions, un CGI avec des param\`{e}tres fix\'{e}s $\Big(\overrightarrow{\SNR}_{1}$, $\overrightarrow{\SNR}_{2}$, $\INR_{12}$, $\INR_{21}\Big)$ est approxim\'{e} par un LDIC avec des param\`{e}tres $\overrightarrow{n}_{11} = \left \lfloor \frac{1}{2}\log(\overrightarrow{\SNR}_{1}) \right \rfloor$, $\overrightarrow{n}_{22} = \left\lfloor \frac{1}{2}\log(\overrightarrow{\SNR}_{2}) \right \rfloor$, $n_{12} = \left \lfloor \frac{1}{2}\log(\INR_{12}) \right \rfloor$ et $n_{21} = \left \lfloor \frac{1}{2}\log(\INR_{21}) \right \rfloor$. 
%
\`{A} partir de cette observation, les r\'{e}sultats des Th\'{e}or\`{e}me \ref{TheoremLD-IC-NOF-Th1fr} - Th\'{e}or\`{e}me \ref{TheoremLD-IC-NOF-Th6fr} 
peuvent servir \`{a} d\'{e}terminer les seuils de SNR de la voie de retour au-del\`{a} duquel un des d\'{e}bits individuels ou le d\'{e}bit somme est am\'{e}lior\'{e} dans le GIC-NOF original. La proc\'{e}dure consiste \`{a} utiliser les \'{e}galit\'{e}s $\overleftarrow{n}_{ii} = \left \lfloor \frac{1}{2}\log\left( \overleftarrow{\SNR}_{i}\right) \right \rfloor $, avec $i \in \lbrace 1,2 \rbrace$. Par cons\'{e}quent, les seuils correspondants dans le CGI \`{a} deux utilisateurs peuvent \^{e}tre calcul\'{e}s approximativement par : 
%
\begin{subequations}\label{EqApproxSNRfr}
\begin{IEEEeqnarray}{lcl}
\overleftarrow{\SNR}_{i}^* & = & 2^{2 \overleftarrow{n}_{ii}^*},\\
\overleftarrow{\SNR}_{i}^{\dagger} & = & 2^{2 \overleftarrow{n}_{ii}^{\dagger}}, \textrm{ et }\\
\overleftarrow{\SNR}_{i}^{+} & = & 2^{2 \overleftarrow{n}_{ii}^{+}}.
\end{IEEEeqnarray}
\end{subequations}
%
Lorsque le LDIC-NOF correspondant est tel que sa r\'{e}gion de capacit\'{e} peut \^{e}tre agrandie, \`{a} savoir, si $\overleftarrow{n}_{ii} > \overleftarrow{n}_{ii}^{*}$ (Th\'{e}or\`{e}me \ref{TheoremLD-IC-NOF-Th1fr}) pour un $i \in \lbrace 1,2 \rbrace$, on s'attend \`{a} ce que, soit la faisabilit\'{e}, soit les r\'{e}gions d'impossibilit\'{e} du GIC-NOF original s'agrandissent  lorsque $\overleftarrow{\SNR}_{i} > \overleftarrow{\SNR}_{i}^*$. 
%
De m\^{e}me, si le LDIC-NOF correspondant est tel que $\Delta_i(\overleftarrow{n}_{ii})>0$ ou $\Delta_i(\overleftarrow{n}_{jj})>0$, on s'attend \`{a} observer une am\'{e}lioration du d\'{e}bit individuel $R_i$ soit en utilisant la voie de retour \`{a} la paire \'{e}metteur-r\'{e}cepteur  $i$, avec $\overleftarrow{\SNR}_{i} > \overleftarrow{\SNR}_{i}^{\dagger}$ soit en utilisant la voie de retour \`{a} la paire \'{e}metteur-r\'{e}cepteur  $j$, avec $\overleftarrow{\SNR}_{j} > \overleftarrow{\SNR}_{j}^{*}$.
%
Lorsque le LDIC-NOF correspondant est tel que $\Sigma(\overleftarrow{n}_{ii})>0$ en utilisant la voie de retour \`{a} la paire \'{e}metteur-r\'{e}cepteur  $i$, avec $\overleftarrow{n}_{ii} > \overleftarrow{n}_{ii}^{+}$  (Th\'{e}or\`{e}me \ref{TheoremLD-IC-NOF-Th6fr}), on s'attend \`{a} observer une am\'{e}lioration au niveau du d\'{e}bit somme en utilisant la voie de retour \`{a} la paire \'{e}metteur-r\'{e}cepteur  $i$, avec $\overleftarrow{\SNR}_{i} > \overleftarrow{\SNR}_{i}^{+}$.
%
Enfin, lorsqu'on n'observe aucune am\'{e}lioration dans une m\'{e}trique donn\'{e}e dans le LDIC-NOF \`{a} deux utilisateurs, \`{a} savoir, $\Delta_1(\overleftarrow{n}_{11})=0$, $\Delta_1(\overleftarrow{n}_{22})=0$, $\Delta_2(\overleftarrow{n}_{11})=0$, $\Delta_2(\overleftarrow{n}_{22})=0$, $\Sigma(\overleftarrow{n}_{11})=0$, ou $\Sigma(\overleftarrow{n}_{22})=0$, on n'observe qu'une am\'{e}lioration n\'{e}gligeable (le cas \'{e}ch\'{e}ant) dans la m\'{e}trique correspondante du GIC-NOF \`{a} deux utilisateurs.
%

\section{Principaux R\'{e}sultats du Canal Lin\'{e}aire D\'{e}terministe \`{a} Interf\'{e}rence  D\'{e}centralis\'{e}}\label{Chapter8fr}

Cette section pr\'{e}sente les principaux r\'{e}sultats sur le D-LDIC-NOF \`{a} deux utilisateurs. Ce mod\`{e}le est d\'{e}crit dans la Section \ref{SectCLDICNOFfr} et peut \^{e}tre analys\'{e} par un jeu comme sugg\'{e}r\'{e} dans la Section \ref{SecGameFormulationfr}.
%
Notons $\Cldicnof(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}, n_{21}$, $ \overleftarrow{n}_{11} , \overleftarrow{n}_{22})$ la r\'{e}gion de capacit\'{e} du LDIC-NOF \`{a} deux utilisateurs avec les param\`{e}tres $\overrightarrow{n}_{11}$, $\overrightarrow{n}_{22}$, $n_{12}$, $n_{21}$, $\overleftarrow{n}_{11}$, et $\overleftarrow{n}_{22}$, d\'{e}crits dans le Th\'{e}or\`{e}me \ref{TheoremANFBLDMCapfr}. 

\subsection {R\'{e}gion d'$\eta$-\'{E}quilibre de Nash} \label{SectNLDICNOFfr}

Cette section pr\'{e}sente la r\'{e}gion d'$\eta$-\'{e}quilibre de Nash $\Nldicnof$ (D\'{e}finition \ref{DefNERegionfr}) du D-LDIC-NOF \`{a} deux utilisateurs.
%

La r\'{e}gion d'$\eta$-\'{e}quilibre de Nash $\Nldicnof$ du D-LDIC-NOF, \`{a} deux utilisateurs, \'{e}tant donn\'{e}  les param\`{e}tres fix\'{e}s  $\big(\overrightarrow{n}_{11}$, $\overrightarrow{n}_{22}$, $n_{12}$, $n_{21}$, $\overleftarrow{n}_{11}$,$\overleftarrow{n}_{22}\big)\in \mathds{N}^6$, est not\'{e}e,   $\Nldicnof\left(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}, n_{21}, \overleftarrow{n}_{11}, \overleftarrow{n}_{22}\right)$.  
%
La r\'{e}gion d'$\eta$-\'{e}quilibre de Nash $\Nldicnof$ est caract\'eris\'ee par deux r\'egions :  la r\'egion de capacit\'e, not\'{e}e par $\Cldicnof \big(\overrightarrow{n}_{11}$, $\overrightarrow{n}_{22}$, $n_{12}$, $n_{21}$, $\overleftarrow{n}_{11}$, $\overleftarrow{n}_{22}\big)$ et une r\'egion convexe, not\'{e}e par $\Bldicnof\big(\overrightarrow{n}_{11}$, $\overrightarrow{n}_{22}$, $n_{12}$, $n_{21}$, $\overleftarrow{n}_{11}$, $\overleftarrow{n}_{22}\big)$. 
%
Dans les sections suivantes, le sextuplet   $(\overrightarrow{n}_{11}$, $\overrightarrow{n}_{22}$, $n_{12}$, $n_{21}$, $\overleftarrow{n}_{11}$, $\overleftarrow{n}_{22})$ sera explicit\'e seulement s'il est n\'ecessaire. 

La r\'egion de capacit\'e $\Cldicnof$ du LDIC-NOF est d\'ecrite par le Th\'eor\`eme \ref{TheoremANFBLDMCapfr}. 
%
Pour tout $\eta > 0$, la r\'egion convexe $\Bldicnof$ est d\'efinie de la mani\`ere suivante : 

%
\begin{IEEEeqnarray}{lcl}
\label{EqBldicnfbfr}
\Bldicnof &=& \Big \lbrace (R_1, R_2) \in \mathds{R}_{+}^2  :  L_i  \leqslant \! R_i  \leqslant  \Uldicnfb_i,  \mbox{ pour tout } i \in \mathcal{K}=\lbrace 1, 2 \rbrace \Big \rbrace, 
\end{IEEEeqnarray}
%
%o\`{u}, 
o\`{u},
%
\begin{subequations}
\label{EqLlUidicnfbfr}
\begin{IEEEeqnarray}{lcl}
\label{EqLldicnfbfr}
L_i & = & \left(\left(\overrightarrow{n}_{ii} - n_{ij} \right)^+-\eta\right)^+ \textrm{ et } \\
\label{EqUldicnfbfr}
U_i & = & \max\left( \overrightarrow{n}_{ii}, n_{ij} \right) \\
\nonumber
& & - \Bigg(\! \min\left(\left(\overrightarrow{n}_{jj} \! - \! n_{ji} \right)^+ \! , n_{ij}\right) \! - \!  \bigg(\! \min\left(\left(\overrightarrow{n}_{jj}\! - \! n_{ij} \right)^+\!, n_{ji}\right) \! - \! \left( \max\left(\overrightarrow{n}_{jj}, n_{ji} \right) \! - \! \overleftarrow{n}_{jj} \right)^+ \bigg)^+\Bigg)^+ \! + \eta,
\end{IEEEeqnarray}
\end{subequations}
%
avec $i\in \lbrace 1, 2 \rbrace$ et $j\in \lbrace 1, 2 \rbrace\setminus \lbrace i \rbrace$.
%
Le Th\'eor\`eme \ref{TheoremMainResultLDICnFBfr} utilise la r\'egion $\Bldicnof$ dans \eqref{EqBldicnfbfr} et la r\'egion de capacit\'e $\Cldicnof$ pour d\'ecrire la r\'{e}gion d'$\eta$-\'{e}quilibre de Nash $\Nldicnof$. 

%theorem style=margin apart,left=10mm, right=10mm
\begin{thm-fr}[, label=TheoremMainResultLDICnFBfr]{R\'{e}gion d'$\eta$-\'{E}quilibre de Nash}{}
%
Soit $\eta > 0$ fix\'e. La r\'{e}gion d'$\eta$-\'{e}quilibre de Nash $\Nldicnof$ du canal lin\'{e}aire d\'eterministe \`{a} interf\'{e}rence  avec  r\'etro-alimentation d\'egrad\'ee par un bruit additif d\'ecrit par les param\`{e}tres $\overrightarrow{n}_{11}$, $\overrightarrow{n}_{22}$, $n_{12}$, $n_{21}$, $\overleftarrow{n}_{11}$ et $\overleftarrow{n}_{22}$, est
%
\begin{equation}
\label{EqNERegionldicnfbfr}
\Nldicnof = \Cldicnof \cap \Bldicnof.
\end{equation}
%
\end{thm-fr}
%

\subsection{Agrandissement de la R\'{e}gion d'$\eta$-\'{E}quilibre de Nash avec Voie de Retour}\label{SectEnlargNashLDfr}

La m\'{e}trique, les conditions et les valeurs pour les param\`{e}tres de la voie de retour au-del\`{a} desquelles la r\'{e}gion d'$\eta$-\'{e}quilibre de Nash $\Nldicnof$ du LDIC-NOF \`{a} deux utilisateurs peut \^{e}tre agrandie sont les m\^{e}mes que dans le cas centralis\'{e}, en tenant compte du fait que ceux-ci se r\'{e}f\`{e}rent \`{a} la r\'{e}gion d'$\eta$-\'{e}quilibre de Nash $\Nldicnof$ au lieu de la r\'{e}gion de capacit\'{e}.

\subsection{Efficacit\'{e} d'$\eta$-\'{E}quilibre de Nash}\label{SectEfficmetricsfr}

Cette section caract\'{e}rise l'efficacit\'{e} de l'ensemble des \'{e}quilibres dans le D-LDIC-NOF \`{a} deux utilisateurs \`{a} l'aide de deux indicateurs :  le prix de l'anarchie (PoA) et le prix de la stabilit\'{e} (PoS).

\subsubsection{D\'{e}finitions}

Les r\'{e}sultats de cette section sont pr\'{e}sent\'{e}s au moyen d'une liste d'\'{e}v\'{e}nements (variables bool\'{e}ennes) d\'{e}termin\'{e}s par les param\`{e}tres $\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}$, et $n_{21}$.  Soient $i \in \lbrace 1, 2 \rbrace$ et $j \in \lbrace 1, 2 \rbrace\setminus\lbrace i \rbrace$, et d\'{e}finissons les \'{e}v\`{e}nements suivants : 
%
\begin{subequations}
\label{EventsNashEfficiencyfr}
\begin{IEEEeqnarray}{rl}
\label{EventA1fr}
A_{1,i} : & \quad \overrightarrow{n}_{ii}-n_{ij} \geqslant n_{ji}, \\
\label{EventA2fr}
A_{2,i} : & \quad \overrightarrow{n}_{ii} \geqslant n_{ji}, \\
\label{EventB1fr}
B_{1} : &  \quad A_{1,1} \land A_{1,2},\\
\label{EventB2fr}
B_{2,i} : & \quad A_{1,i} \land \overline{A}_{1,j} \land A_{2,j}, \\
\label{EventB3fr}
B_{3,i} : &  \quad A_{1,i} \land \overline{A}_{1,j} \land \overline{A}_{2,j}, \\
\label{EventB4fr}
B_{4} : & \quad \overline{A}_{1,1} \land \overline{A}_{1,2} \land A_{2,1} \land A_{2,2},  \\
\label{EventB5fr}
B_{5,i} : & \quad \overline{A}_{1,1} \land \overline{A}_{1,2} \land \overline{A}_{2,i} \land A_{2,j}, \\
\label{EventB6fr}
B_{6} : & \quad  \overline{A}_{1,1} \land \overline{A}_{1,2} \land \overline{A}_{2,1} \land \overline{A}_{2,2}, \\  
\label{EventB7fr}
B_{7} : & \quad  A_{1,1}, \\
\label{EventB8fr}
B_{8}  : & \quad \overline{A}_{1,1} \land A_{2,1} \land A_{2,2}, \\
\label{EventB9fr}
B_{9}  : & \quad \overline{A}_{1,1} \land \overline{A}_{2,1} \land A_{2,2}, \\
\label{EventB10fr}
B_{10} : & \quad \overline{A}_{1,1} \land \overline{A}_{2,2}.
\end{IEEEeqnarray}
\end{subequations}
%
Lorsque les deux paires \'{e}metteur-r\'{e}cepteur sont en LIR, \`{a} savoir, $\overrightarrow{n}_{11}>n_{12}$ et $\overrightarrow{n}_{22} > n_{21}$, les \'{e}v\'{e}nements $B_{1}$, $B_{2,1}$, $B_{2,2}$, $B_{3,1}$, $B_{3,2}$, $B_{4}$, $B_{5,1}$, $B_{5,2}$, et $B_{6}$ satisfont la propri\'{e}t\'{e} d\'{e}clar\'{e}e par le lemme suivant.
%
\begin{lemma-fr} \label{LemmaProperSetPoA1fr}
Pour un quadruplet fixe $(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}, n_{21}) \in \mathds{N}^{4}$ avec $\overrightarrow{n}_{11}>n_{12}$ et $\overrightarrow{n}_{22} > n_{21}$, seul un des \'{e}v\'{e}nements $B_{1}$, $B_{2,1}$, $B_{2,2}$, $B_{3,1}$, $B_{3,2}$, $B_{4}$, $B_{5,1}$, $B_{5,2}$, et $B_{6}$ est vrai.
\end{lemma-fr}
%

Lorsque la paire \'{e}metteur-transmetteur $1$ est en LIR et la paire \'{e}metteur-transmetteur $2$ est en HIR, \`{a} savoir, $\overrightarrow{n}_{11}>n_{12}$ et $\overrightarrow{n}_{22} \leqslant n_{21}$, les \'{e}v\'{e}nements $B_{7}$, $B_{8}$, $B_{9}$, et $B_{10}$ satisfont la propri\'{e}t\'{e} d\'{e}clar\'{e}e par le lemme suivant.
%
\begin{lemma-fr} \label{LemmaProperSetPoA2fr}
Pour un quadruplet fixe $(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}, n_{21}) \in \mathds{N}^{4}$ avec $\overrightarrow{n}_{11}>n_{12}$ et $\overrightarrow{n}_{22} \leqslant n_{21}$, seul un des \'{e}v\'{e}nements $B_{7}$, $B_{8}$, $B_{9}$, et $B_{10}$ est vrai.
\end{lemma-fr}
%


\subsubsection{Prix de l'Anarchie}\label{SecPoA-LD-DICfr}

Soit $\mathcal{A}=\mathcal{A}_1 \times \mathcal{A}_2$ l'ensemble de toutes les paires de configuration possibles et $\mathcal{A}_{\eta-\mathrm{EN}} \subset \mathcal{A}$ l'ensemble de paires de configuration d'$\eta$-\'{e}quilibre de Nash du jeu dans \eqref{EqGamefr} (D\'{e}finition \ref{DefEtaNEfr}).
%

\begin{definition-fr}[Prix de l'Anarchie \cite{Papadimitriou-STACS-1999}] \label{DefPoAfr}
Soit $\eta > 0$. Le PoA du jeu $\gameNF$, not\'{e} $\PoA\left(\eta, \gameNF \right)$, est donn\'{e} par : 
%
\begin{IEEEeqnarray}{rcl}
\label{EqPoAfr}
\PoA\left(\eta, \gameNF \right) = \frac{\ds\max_{(s_1,s_2) \in \mathcal{A}} \ds\sum_{i = 1}^{2} R_{i}(s_1,s_2)}{\ds\min_{(s_1^*,s_2^*) \in \mathcal{A}_{\eta-\mathrm{EN}}} \ds\sum_{i = 1}^{2} R_{i}(s_1^*,s_2^*)}.
\end{IEEEeqnarray}
\end{definition-fr}

Soit $\overline\Sigma_{C}$ la solution du probl\`{e}me d'optimisation dans le num\'{e}rateur de \eqref{EqPoAfr}, qui correspond au d\'{e}bit somme maximum dans le cas centralis\'{e}. 
%
Soit aussi $\underline\Sigma_{N}$ la solution du probl\`{e}me d'optimisation dans le d\'{e}nominateur de \eqref{EqPoAfr}.

Les th\'{e}or\`{e}mes suivants explicitent l'expression du $\PoA \left( \eta, \gameNF \right)$ dans les r\'{e}gimes d'interf\'{e}rence particuliers du D-LDIC-NOF \`{a} deux utilisateurs. Dans tous les cas, on suppose que $\overleftarrow{n}_{ii} \leqslant \max \left(\overrightarrow{n}_{ii}, n_{ij} \right)$ pour tout $i \in \lbrace 1, 2 \rbrace$ et $j\in \lbrace 1, 2 \rbrace\setminus \lbrace i \rbrace$. Si $\overleftarrow{n}_{11} > \max \left(\overrightarrow{n}_{11}, n_{12} \right)$ ou $\overleftarrow{n}_{22} > \max \left(\overrightarrow{n}_{22}, n_{21} \right)$, les r\'{e}sultats sont les m\^{e}mes que ceux dans le cas  de POF, \`{a} savoir, $\overleftarrow{n}_{11} = \max \left(\overrightarrow{n}_{11}, n_{12} \right)$ ou $\overleftarrow{n}_{22} = \max \left(\overrightarrow{n}_{22}, n_{21} \right)$.

%theorem style=margin apart,left=10mm, right=10mm
\begin{thm-fr}[, label=theoremPoA1fr]{Les Deux Paires \'Emetteur-R\'ecepteur en LIR}{}
Pour tout $i \in \lbrace 1, 2 \rbrace$, $j \in \lbrace 1, 2 \rbrace\setminus\lbrace i \rbrace$ et pour tout $(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}, n_{21}, \overleftarrow{n}_{11}, \overleftarrow{n}_{22}) \in \mathds{N}^{6}$ avec $\overrightarrow{n}_{11}>n_{12}$ et $\overrightarrow{n}_{22} > n_{21}$, le $\PoA \left( \eta, \gameNF \right)$ satisfait :  
%
\begin{equation}
\label{EqPoALIRLIRfr}
\PoA \left(\eta, \gameNF \right) = \left\lbrace
\begin{array}{lcl}
\ds \frac{\overline\Sigma_{C1}}{\overrightarrow{n}_{11}-n_{12}+\overrightarrow{n}_{22}-n_{21}-2\eta} & \text{ si }& B_{1}\textrm{ est vrai}  \\ 
\ds \frac{\overline\Sigma_{C2,i}}{\overrightarrow{n}_{11}-n_{12}+\overrightarrow{n}_{22}-n_{21}-2\eta} & \text{ si }& B_{2,i}\textrm{ est vrai} \\ 
\ds \frac{\overrightarrow{n}_{ii}}{\overrightarrow{n}_{11}-n_{12}+\overrightarrow{n}_{22}-n_{21}-2\eta} & \text{ si }& B_{3,i} \lor B_{5,i} \textrm{ est vrai}  \\ 
\ds \frac{\overline\Sigma_{C3}}{\overrightarrow{n}_{11}-n_{12}+\overrightarrow{n}_{22}-n_{21}-2\eta} & \text{ si }& B_{4}\textrm{ est vrai}  \\ 
%\ds \frac{\overrightarrow{n}_{ii}}{\overrightarrow{n}_{11}-n_{12}+\overrightarrow{n}_{22}-n_{21}-2\eta} & \text{ si }& B_{5,i}\textrm{ est vrai}  \\
\ds \frac{\min(\overrightarrow{n}_{11},\overrightarrow{n}_{22})}{\overrightarrow{n}_{11}-n_{12}+\overrightarrow{n}_{22}-n_{21}-2\eta} & \text{ si }& B_{6}\textrm{ est vrai}
\end{array},
\right.
\end{equation}
%
o\`{u}, 
%
\begin{subequations}
\label{EqSumCLIRLIRfr}
\begin{IEEEeqnarray}{rcl}
\label{EqsumC1fr}
\overline{\Sigma}_{C1} &=&  \min \! \Bigg( \!  \overrightarrow{n}_{22}  +  \overrightarrow{n}_{11}  -  n_{12}, \overrightarrow{n}_{11}  +  \overrightarrow{n}_{22} - n_{21}, \\
\nonumber
& & \max \! \Big( \! \overrightarrow{n}_{11}-n_{12}, \overleftarrow{n}_{11} \Big) +\max \! \Big( \! \overrightarrow{n}_{22}-n_{21}, \overleftarrow{n}_{22} \Big), \\
\nonumber
& & 2\overrightarrow{n}_{11}-n_{12} +\max\Big(\overrightarrow{n}_{22}-n_{21}, \overleftarrow{n}_{22} \Big), 2\overrightarrow{n}_{22}-n_{21} +\max\Big(\overrightarrow{n}_{11}-n_{12}, \overleftarrow{n}_{11} \Big) \Bigg);  
\end{IEEEeqnarray}
%%%%%%
\begin{IEEEeqnarray}{rcl}
\label{EqsumC2fr}
\overline{\Sigma}_{C2,i} &=& \min \! \Bigg( \! \overrightarrow{n}_{22}+\overrightarrow{n}_{11}-n_{12}, \overrightarrow{n}_{11}+\overrightarrow{n}_{22}-n_{21}, \\
\nonumber
& & \max \! \Big( \! \overrightarrow{n}_{11}-n_{12}, \overleftarrow{n}_{11}  \Big) +\max \! \Big( \! \overrightarrow{n}_{22}-n_{21}, \overleftarrow{n}_{22} \Big), \\
\nonumber
& & 2\overrightarrow{n}_{ii}-n_{ij}+\max\Big(n_{ij}, \overleftarrow{n}_{jj} \Big), 2\overrightarrow{n}_{jj}-n_{ji}+\max\Big(\overrightarrow{n}_{ii}-n_{ij}, \overleftarrow{n}_{ii} \Big) \Bigg); \textrm{ et }  \\
%\end{IEEEeqnarray}
%%%%
%\begin{IEEEeqnarray}{rcl}
\nonumber
\overline{\Sigma}_{C3} &=& \min\Bigg( \overrightarrow{n}_{22}+\overrightarrow{n}_{11}-n_{12}, \overrightarrow{n}_{11}+\overrightarrow{n}_{22}-n_{21}, \max\Big(n_{21}, \overleftarrow{n}_{11} \Big) +\max\Big(n_{12}, \overleftarrow{n}_{22} \Big), \\
\label{EqSumC3fr}
& & 2\overrightarrow{n}_{11}-n_{12}+\max\Big(n_{12}, \overleftarrow{n}_{22} \Big), 2\overrightarrow{n}_{22}-n_{21}+\max\Big(n_{21}, \overleftarrow{n}_{11}\Big) \Bigg). 
\end{IEEEeqnarray}
\end{subequations}
\end{thm-fr}


%theorem style=margin apart ,left=10mm, right=10mm

\begin{thm-fr}[, label=theoremPoA2fr]{\'Emetteur-R\'ecepteur $1$ en LIR et \'Emetteur-R\'ecepteur $2$ en HIR}{}
Pour tout $(\overrightarrow{n}_{11}, \overrightarrow{n}_{22}, n_{12}, n_{21}, \overleftarrow{n}_{11}, \overleftarrow{n}_{22}) \in \mathds{N}^{6}$ avec $\overrightarrow{n}_{11}>n_{12}$ et $\overrightarrow{n}_{22} \leqslant n_{21}$, le $\PoA \left( \eta, \gameNF \right)$ satisfait :  
%
\begin{equation}
\label{EqPoALIRHIRfr}
\PoA \left(\eta, \gameNF \right) = \left\lbrace
\begin{array}{lcl}
\ds \frac{\overrightarrow{n}_{11}}{\overrightarrow{n}_{11} - n_{12}  -\eta} & \text{ si }& B_{7} \lor B_{8} \lor B_{10} \textrm{ est vrai}  \\ \\
%\ds \frac{\overrightarrow{n}_{11}}{\overrightarrow{n}_{11} - n_{12}  -\eta} & \text{ si }& B_{8}\textrm{ est vrai} \\
\ds \frac{\min(\overrightarrow{n}_{22}+\overrightarrow{n}_{11}-n_{12},n_{21})}{\overrightarrow{n}_{11} - n_{12}  -\eta} & \text{ si }& B_{9}\textrm{ est vrai}  
%\ds \frac{\overrightarrow{n}_{11}}{\overrightarrow{n}_{11} - n_{12}  -\eta} & \text{ si }& B_{10}\textrm{ est vrai}.
\end{array}.
\right.
\end{equation}
\end{thm-fr}


Notons que dans les cas dans lesquels la paire \'{e}metteur-r\'{e}cepteur $1$ est en LIR et la paire \'{e}metteur-r\'{e}cepteur  $2$ est en HIR, le $\PoA \left( \eta, \gameNF \right)$ ne d\'{e}pend pas des param\`{e}tres de la voie de retour. Ceci en r\'{e}sulte dans la mesure o\`{u} l'utilisation de la voie de retour dans ce sc\'{e}nario peut agrandir la r\'{e}gion de capacit\'{e} mais n'augmente  pas la capacit\'{e} du d\'{e}bit somme (Th\'{e}or\`{e}me \ref{TheoremLD-IC-NOF-Th6fr}).

Dans le cas dans lequel la paire \'{e}metteur-r\'{e}cepteur $1$ est en HIR et la paire \'{e}metteur-r\'{e}cepteur $2$ est en LIR, \`{a} savoir, $\overrightarrow{n}_{11} \leqslant n_{12}$ et $\overrightarrow{n}_{22} > n_{21}$, le $\PoA \left( \eta, \gameNF \right)$ pour le D-LDIC-NOF \`{a} deux utilisateurs est qualifi\'{e} comme dans le Th\'{e}or\`{e}me \ref{theoremPoA2fr} interchangeant les indices des param\`{e}tres.


%theorem style=margin apart,left=10mm, right=10mm
\begin{thm-fr}[, label=theoremPoA4fr]{Les Deux Paires \'Emetteur-R\'ecepteur en HIR}{}
Pour tout $(\overrightarrow{n}_{11}$, $\overrightarrow{n}_{22}$, $n_{12}$, $n_{21}$, $\overleftarrow{n}_{11}$, $\overleftarrow{n}_{22}) \in \mathds{N}^{6}$ avec $\overrightarrow{n}_{11} \leqslant n_{12}$ et $\overrightarrow{n}_{22} \leqslant n_{21}$, le $\PoA \left( \eta, \gameNF \right)$ satisfait : 
%
\begin{equation}
\label{EqPoAHIRHIRfr}
\PoA \left(\eta, \gameNF \right) = \infty.
\end{equation}
\end{thm-fr}

Le r\'{e}sultat du Th\'{e}or\`{e}me \ref{theoremPoA4fr} est d\^{u} au fait que $\Big(\big(\overrightarrow{n}_{11} - n_{12} \big)^{+}-\eta\Big)^++\Big(\big(\overrightarrow{n}_{22} - n_{21} \big)^{+}-\eta\Big)^+=0$. Autrement dit, lorsque $\overrightarrow{n}_{11} \leqslant n_{12}$ et $\overrightarrow{n}_{22} \leqslant n_{21}$, aucune des paires d'\'{e}metteur-r\'{e}cepteur n'est capable de transmettre \`{a} un d\'{e}bit strictement positif au pire $\eta$-\'{e}quilibre de Nash (le plus petit d\'{e}bit somme dans la r\'{e}gion d'$\eta$-\'{e}quilibre de Nash $\Nldicnof$). 

D'une fa\c{c}on g\'{e}n\'{e}rale, dans tout r\'{e}gime d'interf\'{e}rence dans lequel le  $\PoA \left( \eta, \gameNF \right)$ d\'{e}pend des param\`{e}tres de la voie de retour $\overleftarrow{n}_{11}$ ou $\overleftarrow{n}_{22}$, il existe une valeur de param\`{e}tre de la voie de retour $\overleftarrow{n}_{11}$ ou de param\`{e}tre de la voie de retour  $\overleftarrow{n}_{22}$ au-del\`{a} duquel le $\PoA \left( \eta, \gameNF \right)$ augmente. Ces valeurs correspondent \`{a} celles au-del\`{a} desquelles la capacit\'{e} de somme peut \^{e}tre augment\'{e}e (Th\'{e}or\`{e}me \ref{TheoremLD-IC-NOF-Th6fr}). 

\subsubsection{Prix de la Stabilit\'{e}}\label{SecPoS-LD-DICfr}

Dans cette section, l'efficacit\'{e} d'$\eta$-\'{e}quilibre de Nash du jeu $\gameNF$ en \eqref{EqGamefr} est analys\'{e}e \`{a} l'aide du PoS. 
%
\begin{definition-fr}[Prix de la Stabilit\'{e} \cite{Anshelevich-STC-2003}] \label{DefPoSfr} 
Soit $\eta > 0$. Le PoS du jeu $\gameNF$, d\'{e}not\'{e} par $\PoS\left(\eta, \gameNF \right)$, est donn\'{e} par : 
%
\begin{IEEEeqnarray}{rcl}
\label{EqPoSfr}
\PoS \left(\eta, \mathcal{G} \right) &=& \frac{\ds\max_{(s_1,s_2) \in \mathcal{A}} \ds\sum_{i = 1}^{2} R_{i}(s_1,s_2)}{\ds\max_{(s_1^*,s_2^*) \in \mathcal{A}_{\eta-\mathrm{EN}}} \ds\sum_{i = 1}^{2} R_{i}(s_1^*,s_2^*)}.
\end{IEEEeqnarray}
\end{definition-fr}
%
Soit $\overline\Sigma_{N}$  la solution du probl\`{e}me d'optimisation dans le d\'{e}nominateur de \eqref{EqPoSfr}.   

La proposition suivante caract\'{e}rise le PoS du jeu $\gameNF$ dans \eqref{EqGamefr} pour le D-LDIC-NOF \`{a} deux utilisateurs.

\begin{proposition}[PoS]\label{PropPoSfr}\emph{
Pour tout $(\overrightarrow{n}_{11}$, $\overrightarrow{n}_{22}$, $n_{12}$, $n_{21}$, $\overleftarrow{n}_{11}$, $\overleftarrow{n}_{22}) \in \mathds{N}^6$ et pour tout $\eta>0$ arbitrairement petit, le PoS dans le jeu $\gameNF$ du D-LDIC-NOF \`{a} deux utilisateurs est : 
\begin{IEEEeqnarray}{rcl}
\PoS \left( \eta, \gameNF \right) &=& 1. 
\end{IEEEeqnarray}
%
}
\end{proposition}


Notons que le fait que le prix de la stabilit\'{e} soit \'{e}gal \`{a} un, ind\'{e}pendamment des param\`{e}tres $\overrightarrow{n}_{11}$, $\overrightarrow{n}_{22}$, $n_{12}$, $n_{21}$, $\overleftarrow{n}_{11}$ et $\overleftarrow{n}_{22}$, implique que malgr\'{e} le comportement anarchique des deux paires \'{e}metteur-r\'{e}cepteur, le d\'{e}bit somme d'$\eta$-\'{e}quilibre de Nash le plus \'{e}lev\'{e} est \'{e}gal \`{a} la capacit\'{e} du d\'{e}bit somme, \`{a} savoir, $\overline{\Sigma}_{C}=\overline{\Sigma}_{N}$. Cela implique que dans tous les r\'{e}gimes d'interf\'{e}rence, il existe toujours un $\eta$-\'{e}quilibre de Nash optimal pour le d\'{e}bit somme (optimum de Pareto d'$\eta$-\'{e}quilibre de Nash). 
%
Les seuils sur les param\`{e}tres de la voie de retour au-del\`{a} desquels la somme des capacit\'{e}s et le d\'{e}bit somme maximum dans la r\'{e}gion d'$\eta$-\'{e}quilibre de Nash $\Nldicnof$ peuvent \^{e}tre am\'{e}lior\'{e}s sont obtenus d'apr\`{e}s le Th\'{e}or\`{e}me \ref{TheoremLD-IC-NOF-Th6fr}. 

\section{Principaux R\'{e}sultats du Canal Gaussien \`{a} Interf\'{e}rence D\'{e}centralis\'{e}}\label{Chapter2fr} 

Cette section pr\'{e}sente les principaux r\'{e}sultats sur le D-GIC-NOF \`{a} deux utilisateurs. Ce mod\`{e}le est d\'{e}crit dans la Section \ref{SectCGICNOFfr} et peut \^{e}tre mod\'{e}lis\'{e} par un jeu comme sugg\'{e}r\'{e} dans la Section \ref{SecGameFormulationfr}.
%
Notons $\Cgicnof$ la r\'{e}gion de capacit\'{e} du GIC-NOF \`{a} deux utilisateurs avec les param\`{e}tres fix\'{e}s $\overrightarrow{\SNR}_{1}$, $\overrightarrow{\SNR}_{2}$, $\INR_{12}$, $\INR_{21}$, $\overleftarrow{\SNR}_{1}$, et $\overleftarrow{\SNR}_{2}$.  La r\'{e}gion de capacit\'{e} atteignable $\agicnof$ et la r\'{e}gion d'impossibilit\'{e} $\cgicnof$ correspondent approximent la r\'{e}gion de capacit\'{e} $\Cgicnof$ \`{a} $4.4$ bits pr\`{e}s (Th\'{e}or\`{e}me \ref{TheoremGAP-G-IC-NOFfr}). La r\'{e}gion de capacit\'{e} atteignable  $\agicnof$ et la r\'{e}gion d'impossibilit\'{e}  $\cgicnof$ sont d\'{e}finies par le Th\'{e}or\`{e}me \ref{TheoremA-G-IC-NOFfr} et Th\'{e}or\`{e}me \ref{TheoremC-G-IC-NOFfr}, respectivement.


\subsection{R\'{e}gion d'$\eta$-\'{E}quilibre de Nash Atteignable} \label{SectMainResultsDGICNOFfr}

Soit la r\'{e}gion d'$\eta$-\'{e}quilibre de Nash (D\'{e}finition \ref{DefNERegionfr}) du D-GIC-NOF \`{a} deux utilisateurs indiqu\'{e}e par $\Ngicnof$. 
%
Cette section pr\'{e}sente une r\'{e}gion $\aNgicnof \subseteq \Ngicnof$ qui est atteignable en utilisant le syst\`{e}me Han-Kobayashi randomis\'{e} avec la voie de retour d\'{e}grad\'{e}e par un bruit additif (RHK-NOF). 
%
Le RHK-NOF s'av\`{e}re \^{e}tre une paire de configuration d'$\eta$-\'{e}quilibre de Nash avec $\eta \geqslant 1$. Autrement dit, toute d\'{e}viation unilat\'{e}rale du RHK-NOF par toute paire \'{e}metteur-r\'{e}cepteur peut entra\^{i}ner une am\'{e}lioration du d\'{e}bit individuel d'au maximum un bit par utilisation du canal. 
%
La description de la r\'{e}gion d'$\eta$-\'{e}quilibre de Nash atteignable $\aNgicnof$ est pr\'{e}sent\'{e}e \`{a} l'aide des constantes $a_{1,i}$; des fonctions $a_{2,i} : [0,1] \rightarrow \mathds{R}_{+}$,  $a_{l,i} : [0,1]^2\rightarrow \mathds{R}_{+}$, avec $l \in \lbrace 3, \ldots, 6 \rbrace$; et $a_{7,i} : [0,1]^3\rightarrow \mathds{R}_{+}$, d\'{e}fini dans \eqref{Eq-afr}, pour tout $i \in \lbrace 1, 2 \rbrace$, avec $j \in \lbrace 1, 2 \rbrace \setminus \lbrace i \rbrace$, et les fonctions $b_{l,i} : [0,1]\rightarrow \mathds{R}_{+}$, avec $(l,i) \in \lbrace1, 2 \rbrace^2$, d\'{e}fini en \eqref{Eqfntsfr}. 
%
\`{A} l'aide de cette notation, le r\'{e}sultat principal est pr\'{e}sent\'{e} par le Th\'{e}or\`{e}me~\ref{TheoremMainResultNAGICnFBfr}. 

%theorem style=margin apart,left=10mm, right=10mm
\begin{thm-fr}[, label=TheoremMainResultNAGICnFBfr]{R\'{e}gion d'$\eta$-\'{E}quilibre de Nash Atteignable}{}
Soit $\eta \geqslant 1$. La r\'{e}gion d'$\eta$-\'{e}quilibre de Nash atteignable $\aNgicnof$ est donn\'{e}e par la fermeture de toutes les paires possibles de d\'{e}bit atteignables $(R_1,R_2) \in \agicnof$ satisfaisant, pour tout  $i \in \lbrace 1,2 \rbrace$ et $j \in \lbrace1,2 \rbrace \setminus \lbrace i \rbrace$, les conditions suivantes :
\begin{subequations}
\label{EqNashGAchievableregionfr}
\begin{IEEEeqnarray}{rcl}
\label{EqNashGAchievableregion1fr}
R_i  & \geqslant &  \Big(a_{2,i}(\rho) -a_{3,i}(\rho,\mu_j)-a_{4,i}(\rho,\mu_j)-\eta\Big)^+,\\
\label{EqNashGAchievableregion2fr}
R_i &\leqslant& \min\Big( a_{2,i}(\rho)+a_{3,j}(\rho,\mu_i)+a_{5,j}(\rho,\mu_i)-a_{2,j}(\rho)+\eta,  \\
\nonumber
& &  a_{3,i}(\rho,\mu_j)+a_{7,i}(\rho,\mu_1,\mu_2)+2a_{3,j}(\rho,\mu_i)+a_{5,j}(\rho,\mu_i)-a_{2,j}(\rho)+\eta,   \\
\nonumber
& &  \! a_{2,i}(\rho) \! + \! a_{3,i}(\rho,\mu_j) \! + \!  2a_{3,j}(\rho,\mu_i) \! + \!  a_{5,j}(\rho,\mu_i) \!  + \!  a_{7,j}(\rho,\mu_1,\mu_2) \!  - \!  2a_{2,j}(\rho) + 2\eta \Big),  \\
\label{EqNashGAchievableregion3fr}
R_1+R_2 & \leqslant & a_{1,i} \!  + \!   a_{3,i}(\rho,\mu_j)\! +\! a_{7,i}(\rho,\mu_1,\mu_2)\! +\! a_{2,j}(\rho)\! +\! a_{3,j}(\rho,\mu_1)\! -\! a_{2,i}(\rho) + \eta, 
\end{IEEEeqnarray}
\end{subequations}
pour tout $\left(\rho, \mu_1, \mu_2\right) \in \left[0,\left(1-\max\left(\frac{1}{\INR_{12}},\frac{1}{\INR_{21}}\right) \right)^+\right]\times[0,1]\times[0,1]$.
\end{thm-fr}

\subsection{R\'{e}gion de Des\'{e}quilibre} \label{SectMainResultsDCGICNOFfr}

Soit la r\'{e}gion d'$\eta$-\'{e}quilibre de Nash (D\'{e}finition \ref{DefNERegionfr}) du D-GIC-NOF \`{a} deux utilisateurs indiqu\'{e}e par $\Ngicnof$.  
%
Cette section pr\'{e}sente une r\'{e}gion $\cNgicnof \supseteq \Ngicnof$ donn\'{e}e en termes de r\'{e}gion convexe $\overBgicnof$. Ici, pour le cas du D-GIC-NOF \`{a} deux utilisateurs, la r\'{e}gion convexe $\overBgicnof$ est donn\'{e}e par la fermeture des paires de d\'{e}bit non n\'{e}gatif  $(R_1,R_2)$ qui pour tout $i \in \lbrace 1, 2 \rbrace$, avec $j\in\lbrace 1, 2 \rbrace\setminus\lbrace i \rbrace$ v\'{e}rifient : 

\begin{IEEEeqnarray}{lcl}
\label{EqBiCGaussianfr}
\overBgicnof & = & \Big \lbrace (R_1,R_2)\in \mathds{R}_{+}^2 : L_i \leqslant R_i \leqslant \overline{U}_i, \mbox{ pour tout } i \in \mathcal{K}=\lbrace 1, 2 \rbrace \Big \rbrace, 
\end{IEEEeqnarray}
%
o\`{u}
%
\begin{IEEEeqnarray}{lcl}
\label{EqLiGaussianfr}
L_i & = &   \left(\frac{1}{2}\log\left( 1 + \frac{\overrightarrow{\SNR}_i}{1 + \INR_{ij}}\right)-\eta\right)^+ \mbox{ et } 
\end{IEEEeqnarray}

\begin{IEEEeqnarray}{lcl}
\nonumber
\overline{U}_i &=& \frac{1}{2} \log \left(\overrightarrow{\SNR}_i+2 \rho \sqrt{\overrightarrow{\SNR}_i \INR_{ij}}+\INR_{ij}+1 \right) \\
\nonumber
& &  -\frac{1}{2}\log\left(\frac{\overrightarrow{\SNR}_j+2\left(\rho-\rho_{X_iV_j}\sqrt{\gamma_j}\right)\sqrt{\overrightarrow{\SNR}_j\INR_{ji}} +\INR_{ji}+1}{\left(1-\gamma_j\right) \, \overrightarrow{\SNR}_j+2\left(\rho-\rho_{X_iV_j}\sqrt{\gamma_j}\right)\sqrt{\overrightarrow{\SNR}_j\INR_{ji}} +\INR_{ji}+1} \right)  \\
\nonumber
& & -\frac{1}{2}\log\left(\INR_{ji}\left(1-\rho^2\right)+1 \right)+\frac{1}{2}\log\left(\INR_{ji}\left(1-\left(\rho-\rho_{X_iV_j}\sqrt{\gamma_j}\right)^2\right)+1 \right)  \\
\nonumber
& & + \frac{1}{2}\log \Big(\overrightarrow{\SNR}_j+2 \rho \sqrt{\overrightarrow{\SNR}_j \INR_{ji}}+\INR_{ji}+1 \Big) \\
\nonumber
& & -\frac{1}{2}\! \log \! \Bigg( \overrightarrow{\SNR}_j\left(\gamma_j\!-\gamma_j^2\right)\!+2\gamma_j\left(\rho\!-\rho_{X_iV_j}\sqrt{\gamma_j} \right)\sqrt{\overrightarrow{\SNR}_j \INR_{ji}}\!+\gamma_j\INR_{ji}\left(1\!-\rho_{X_iV_j}^2\right)+\gamma_j \Bigg) \\
\nonumber
& & -\frac{1}{2}\log\left( 1-\rho_{X_iV_j}^2\right)-\frac{1}{2}\log\left(\INR_{ij}\left(1-\rho^2\right)+1\right)\\
\nonumber
&& +\frac{1}{2}\log \Bigg(\gamma_j\left(\INR_{ij}\left(1-\rho^2\right)+1\right)-\rho_{X_iV_j}^2\gamma_j\left(\INR_{ij}+1\right)+\gamma_2\INR_{ij}\left(2\rho_{X_iV_j}\rho\sqrt{\gamma_j}-\gamma_j\right)\Bigg)\\
\label{EqoverUiGaussianfr}
& & + \eta.
\end{IEEEeqnarray}
%
avec
%
\begin{equation}
\label{EqGammajfr}
\gamma_j=\left \{
\begin{array}{lcl}
\ds \min\left(\frac{\overrightarrow{\SNR}_j}{\INR_{ij}\INR_{ji}},\frac{1}{\INR_{ji}}\right)& \text{ si } &  C_{1,j} \lor \Big(C_{2,j} \land C_{3,j} \Big) \textrm{ est vrai}\\ 
\ds \min\left(\frac{1}{\INR_{ji}},\frac{\INR_{ij}}{\INR_{ji}\overrightarrow{\SNR}_j}\right) & \text{ si } & C_{4,j} \textrm{ est vrai} \\ 
\ds \min\left(1, \frac{\INR_{ij}}{\overrightarrow{\SNR}_j}\right) & \text{ si } & C_{5,j} \land  C_{6,j} \textrm{ est vrai}  \\ 
\ds \min\left(\frac{\overrightarrow{\SNR}_j}{\overleftarrow{\SNR}_{j}\INR_{ji}}, \frac{\INR_{ij}}{\overleftarrow{\SNR}_{j}\INR_{ji}}, 1\right)& \text{ si } &  C_{7,j} \lor C_{8,j} \textrm{ est vrai}\\ 
0 & & \textrm{ otherwise} 
\end {array}, \right.
\end{equation}

\begin{subequations}
\label{EventsGammajfr}
\begin{IEEEeqnarray}{ll}
\label{EventsGammaj1fr}
C_{1,j} :   \;	& 	\INR_{ji}<\overrightarrow{\SNR}_j\leqslant\INR_{ij}, \\
\label{EventsGammaj2fr}
C_{2,j} :   	& 	\max\left(\INR_{ij}, \INR_{ji},\overleftarrow{\SNR}_j \right) < \overrightarrow{\SNR}_j<\INR_{ij}\INR_{ji}, \\
\label{EventsGammaj3fr}
C_{3,j} :   	&  	\overleftarrow{\SNR}_j\leqslant\INR_{ij},  \\
\label{EventsGammaj4fr}
C_{4,j} :   	& \INR_{ji}<\INR_{ij} <\overrightarrow{\SNR}_j  \leqslant \overleftarrow{\SNR}_j, \\
\label{EventsGammaj5fr}
C_{5,j} :   	& \overrightarrow{\SNR}_j > \max \left(\INR_{ij},\INR_{ji}, \overleftarrow{\SNR}_j \right), \\
\label{EventsGammaj6fr}
C_{6,j} :   	& \overrightarrow{\SNR}_j \geqslant \max \left(\INR_{ij}\INR_{ji}, \overleftarrow{\SNR}_j\INR_{ji} \right),  \\
\label{EventsGammaj7fr}
C_{7,j} :   	& \max\left(\INR_{ij}, \INR_{ji}, \overleftarrow{\SNR}_j, \frac{\overleftarrow{\SNR}_j\INR_{ji}}{\INR_{ij}}  \right) < \overrightarrow{\SNR}_j<\overleftarrow{\SNR}_j\INR_{ji}\leqslant \frac{\overleftarrow{\SNR}_j\overrightarrow{\SNR}_j}{\INR_{ij}}, \qquad \quad \\
\label{EventsGammaj8fr}
C_{8,j} :   	& \max\left(\INR_{ij}, \INR_{ji}, \overleftarrow{\SNR}_j, \frac{\overleftarrow{\SNR}_j\INR_{ji}}{\INR_{ij}}  \right)<\overrightarrow{\SNR}_j<\INR_{ij}\INR_{ji}<\overleftarrow{\SNR}_j\INR_{ji}, 
\end{IEEEeqnarray}
\end{subequations}
%
,$\rho \in [0,1]$, et $\rho_{X_iV_j} \in [0,1)$.

Notons que $L_i$ est le d\'{e}bit obtenu par la paire d'\'{e}metteur-r\'{e}cepteur $i$ quand il sature la contrainte de puissance en \eqref{Eqconstpowfr} et traite l'interf\'{e}rence comme un bruit. Conform\'{e}ment \`{a} cette notation, la r\'{e}gion de des\'{e}quilibre du GIC-NOF \`{a} deux utilisateurs, \`{a} savoir, $\cNgicnof$, est caracteris\'{e} par le th\`{e}or\'{e}me suivant.

%theorem style=margin apart,left=10mm, right=10mm
\begin{thm-fr}[, label=TheoremMainResultNCGICnFBfr]{R\'{e}gion de Des\'{e}quilibre}{}
Soit $\eta \geqslant 1$. La r\'{e}gion de des\'{e}quilibre $\cNgicnof$ du D-GIC-NOF \`{a} deux utilisateurs est donn\'{e}e par la fermeture de toutes les paires de d\'{e}bits non n\'{e}gatifs possibles $(R_1,R_2) \in \cgicnof \cap \overBgicnof$ pour tout $\rho \in [0,1]$. 
\end{thm-fr}



==> Frontmatter/Notation/notation.tex <==
% !TEX encoding = UTF-8 Unicode
\addchap{Notation}




==> Frontmatter/Notation/notation__1_.tex <==
% !TEX encoding = UTF-8 Unicode
\addchap{Notation}

\chapterletter{T}{hroughout} this thesis, sets are denoted with uppercase calligraphic letters, e.g. $\mathcal{X}$. Random variables are denoted by uppercase letters, e.g., $X$. The realizations and the set of events from which the random variable $X$ takes values are respectively denoted by  $x$ and $\mathcal{X}$. 

For discrete random variables, the probability mass function (pmf) of $X$ over the set $\mathcal{X}$ is denoted $P_{X}$, i.e., $P_X:~\mathcal{X}~\rightarrow~(0,1]$. 
%The support of  $P_X$ is ${\mathrm{supp}\left(P_X \right) = \lbrace x \in \mathcal{X}: P_X\left( x \right) > 0 \rbrace}$. The set of all possible pmfs on $\mathcal{X}$ is $\triangle\left( \mathcal{X} \right)$,  i.e., $P_X \in \triangle\left( \mathcal{X}\right)$. 
%
Whenever a second discrete random variable $Y$ is involved, $P_{X \, Y}$ and $P_{Y|X}$ denote respectively the joint probability mass function of $(X, Y)$, i.e., $P_{X Y}:~\mathcal{X}\times\mathcal{Y}~\rightarrow~(0,1]$,  and the conditional probability mass function of $Y$ given $X$, i.e., $P_{Y|X}:~\mathcal{X}\times\mathcal{Y}~\rightarrow~(0,1]$. 

For continuos random variables, the probability density function (pdf) of $X$ over the set $\mathcal{X}$ is denoted $f_{X}$, i.e., $f_X:~\mathcal{X}~\rightarrow~(0,1]$. 
%The support of  $f_X$ is ${\mathrm{supp}\left(f_X \right) = \lbrace x \in \mathcal{X}: f_X\left( x \right) > 0 \rbrace}$. The set of all possible pdfs on $\mathcal{X}$ is $\triangle\left( \mathcal{X} \right)$,  i.e., $f_X \in \triangle\left( \mathcal{X}\right)$. 
%
Whenever a second continuos random variable $Y$ is involved, $f_{X \, Y}$ and $f_{Y|X}$ denote respectively the joint probability density function of $(X, Y)$, i.e., $f_{X Y}:~\mathcal{X}\times\mathcal{Y}~\rightarrow~(0,1]$,  and the conditional probability density function of $Y$ given $X$, i.e., $f_{Y|X}:~\mathcal{X}\times\mathcal{Y}~\rightarrow~(0,1]$. 

Let $N$ be a fixed natural number. An $N$-dimensional vector of random variables is denoted by $\vec{X} = (X_{1}, X_{2}, ..., X_{N})^\sfT$ and a corresponding realization is denoted by $\vec{x}= (x_{1}, x_{2}, ..., x_{N})^\sfT \in \mathcal{X}^{N}$.  Given $\vec{X} = (X_{1}, X_{2}, ..., X_{N})^\sfT$ and $(a,b) \in \mathds{N}^2$, with $a < b \leqslant N$,  the $(b-a+1)$-dimensional vector of random variables formed by the components $a$ to $b$ of $\vec{X}$ is denoted by ${\vec{X}_{(a:b)} = (X_a, X_{a+1}, \ldots, X_b)^\sfT}$.  The notation $(\cdot)^+$ denotes the positive part operator, i.e., $(\cdot)^+ = \max(\cdot, 0)$ and $\mathbb{E}_{X}[ \cdot ]$ denotes the expectation with respect to the distribution of the random variable $X$. The logarithm function $\log$ is assumed to be base $2$. 







==> Mainmatter/Chapter1/introduction.tex <==
\section{Introduction} 
\label{sec:introduction}

%of such high data rates is \gls{MIMO}, in which a \gls{BS} is equipped with a large number of antennas and serves multiple single-antenna user equipments on the same time-frequency resource.

To keep up with the always increasing mobile user traffic, cellular communication systems have been driven by continuous innovation since the introduction of the first generation in 1979.
The attention is now turning from the fifth to the sixth generation, which some predict should be able to deliver data rates up to 1\:TB/s with high energy efficiency~\cite{roadmap_6G}.
A key enabler is to serve multiple single-antenna users on the same time-frequency resource using a \gls{BS} equipped with a large number of antennas.
However, optimal detection in such \gls{MIMO} systems is known to be NP-hard~\cite{10.1007_s10107-016-1036-0}, and approaches introduced in recent years suffers from unsatisfying performance or become impractical
%become inefficient or impractical on realistic correlated channels 
when the number of antennas or users is large.
Examples of recent approaches include the iterative algorithm AMP~\cite{AMP} or its extension to correlated channels OAMP~\cite{OAMP}.

Recently, advances in \gls{MIMO} detection have been made by using \gls{ML} in conjunction or in place of standard algorithms~\cite{Samsung, DetNet}.
A promising approach is to add trainable parameters to traditional iterative algorithms and interpret the whole structure as an \gls{NN}~\cite{OAMPNet}.
However, these schemes still either suffer from  a performance drop on correlated channels or from high complexity.
One of these approaches is the recently proposed MMNet~\cite{MMNet}, which achieves state-of-the-art performance on correlated channels.
However, it needs to be retrained on each channel realization, which makes its practical implementation challenging.

In this work, we alleviate this issue by leveraging the emerging idea of \emph{hypernetworks}~\cite{learnet,talking_heads}.
Applied to our setup, it consists in having a secondary \gls{NN}, referred to as the hypernetwork, that generates for a given channel matrix an optimized set of weights for an \gls{NN}-based detector.
This scheme, which we refer to as \emph{HyperMIMO}, is illustrated in Fig.~\ref{fig:HG_small}.
Used with the MMNet detector from~\cite{MMNet}, HyperMIMO replaces the training procedure that would be required for each channel realization by a single inference of the hypernetwork.

\begin{figure}
\centering
	\includegraphics[width=0.75\linewidth]{Chapter1/figs/HG_small.pdf}
	\caption{HyperMIMO: A hypernetwork generates the parameters of an NN-based detector (MMNet~\cite{MMNet} in this work) }
\label{fig:HG_small}
\end{figure} 
%
We have evaluated the proposed approach using exhaustive simulations on spatially correlated channels.
Our results show that HyperMIMO achieves a performance close to that of MMNet trained for each channel realization, and outperforms the recently proposed OAMPNet~\cite{OAMPNet}.
%Moreover, it outperforms the recently proposed OAMPNet~\cite{OAMPNet} and the well-known \gls{LMMSE} estimator.
Our results also reveal that HyperMIMO is robust to user mobility up to a certain point, which is encouraging for practical use.

%\textcolor{green}{
%The rest of this paper is organized as follows. 
%Section \ref{sec:Background} covers the background on both MIMO detection %schemes and HyperNetworks.
%Section \ref{sec:HyperMIMO} details the HyperMIMO structure.
%Section \ref{sec:Experiments} explains the channel model, the training %procedure, and presents simulation results.}

\textbf{Notations:} 
Matrices and column vectors are denoted by bold upper- and lower-case letters, respectively. 
$x_{i}$ is the $i^{\text{th}}$ element of the vector $\xv$, and $[X]_{i,j}$ the $(i,j)^{\text{th}}$ element of the matrix $\Xm$.
$\text{diag}(\xv)$ is the diagonal matrix composed of the elements of $\xv$, and $\Id_N$ the $N \times N$ identity matrix.
$||\Xm||_F$  is the Frobenius norm of $\Xm$, and $\Xm^H$ its conjugate transpose.


